A Cool Earth-sized Planet Candidate Transiting a Tenth Magnitude K-dwarf From K2

The transit method is currently one of our best means for the detection of potentially habitable "Earth-like" exoplanets. In principle, given sufficiently high photometric precision, cool Earth-sized exoplanets orbiting Sun-like stars could be discovered via single transit detections; however, this has not previously been achieved. In this work, we report a 10-hour long single transit event which occurred on the $V=10.1$ K-dwarf HD 137010 during K2 Campaign 15 in 2017. The transit is comparatively shallow ($225\pm10$ ppm), but is detected at high signal-to-noise thanks to the exceptionally high photometric precision achieved for the target. Our analysis of the K2 photometry, historical and new imaging observations, and archival radial velocities and astrometry strongly indicate that the event was astrophysical, occurred on-target, and can be best explained by a transiting planet candidate, which we designate HD 137010 b. The single observed transit implies a radius of $1.06^{+0.06}_{-0.05}$ $R_\oplus$, and assuming negligible orbital eccentricity we estimate an orbital period of $355^{+200}_{-59}$ days ($a=0.88^{+0.32}_{-0.10}$ AU), properties comparable to Earth. We project an incident flux of $0.29^{+0.11}_{-0.13}$ $I_\oplus$, which would place HD 137010 b near the outer edge of the habitable zone. This is the first planet candidate with Earth-like radius and orbital properties that transits a Sun-like star bright enough for substantial follow-up observations.

==> photometry_full.tex <==
\begin{deluxetable}{ccc}[ht!]
\label{tab:photometry}
\centering
\tablecaption{K2 photometry of \thisstar{}.}
\tablehead{\colhead{BJD - 2454833} & \colhead{Normalised flux} & \colhead{De-trended flux}}
\startdata
3157.8752 & 0.99945683 & 1.0000828  \\
3157.8956 & 0.99943504 & 1.0000273  \\
3157.9160 & 0.99941655 & 0.99997813 \\
3157.9365 & 0.99945957 & 0.99999344 \\
3157.9569 & 0.99948045 & 0.99998964 \\
3157.9773 & 0.99943664 & 0.99992387 \\
3157.9978 & 0.99945723 & 0.99992539 \\
3158.0182 & 0.99953923 & 0.99999049 \\
3158.2225 & 0.99968173 & 1.0000785  \\
3158.2430 & 0.99963269 & 1.0000327  \\
3158.2634 & 0.99963635 & 1.0000407  \\
3158.2838 & 0.99961781 & 1.0000275  \\
3158.3042 & 0.99958191 & 0.99999771 \\
3158.3247 & 0.99948166 & 0.99990457 \\
3158.3655 & 0.99964110 & 1.0000795  \\
3158.3860 & 0.99957721 & 1.0000241  \\
3158.4064 & 0.99956736 & 1.0000229  \\
3158.4268 & 0.99952351 & 0.99998800 \\
3158.4473 & 0.99952420 & 0.99999770 \\
3158.4677 & 0.99950944 & 0.99999164 \\
3158.4881 & 0.99944077 & 0.99993158 \\
3158.5086 & 0.99947306 & 0.99997230 \\
3158.5290 & 0.99941617 & 0.99992318 \\
3158.5494 & 0.99948348 & 0.99999774 \\
3158.5699 & 0.99941856 & 0.99993947 \\
3158.6312 & 0.99954451 & 1.0000801  \\
3158.6516 & 0.99951113 & 1.0000491  \\
3158.6720 & 0.99949487 & 1.0000347  \\
3158.6925 & 0.99950553 & 1.0000459  \\
3158.7129 & 0.99942104 & 0.99996092 \\
3158.7333 & 0.99946610 & 1.0000047  \\
3158.7538 & 0.99944507 & 0.99998126 \\
3158.7742 & 0.99943329 & 0.99996620 \\
3158.7946 & 0.99946396 & 0.99999294 \\
3158.8151 & 0.99946356 & 0.99998760 \\
3158.8559 & 0.99952354 & 1.0000356  \\
3158.8764 & 0.99952295 & 1.0000279  \\
3158.8968 & 0.99952107 & 1.0000183  \\
3158.9172 & 0.99951635 & 1.0000053  \\
3158.9376 & 0.99952419 & 1.0000042  \\
3158.9581 & 0.99950071 & 0.99997139 \\
3158.9785 & 0.99955581 & 1.0000167  \\
3158.9989 & 0.99961405 & 1.0000646  \\
3159.0194 & 0.99957893 & 1.0000187  \\
3159.0398 & 0.99961552 & 1.0000442  \\
3159.0602 & 0.99963061 & 1.0000479  \\
3159.1011 & 0.99959677 & 0.99999040 \\
3159.1215 & 0.99958542 & 0.99996688 \\
3159.1420 & 0.99957442 & 0.99994353 \\
3159.1624 & 0.99966120 & 1.0000181  \\
3159.1828 & 0.99961684 & 0.99996122 \\
3159.2033 & 0.99965114 & 0.99998295 \\
3159.2237 & 0.99965407 & 0.99997336 \\
3159.2441 & 0.99958119 & 0.99988812 \\
3159.2646 & 0.99958991 & 0.99988432 \\
3159.2850 & 0.99965971 & 0.99994192 \\
3159.3667 & 0.99976309 & 0.99999829 \\
3159.3872 & 0.99983004 & 1.0000543  \\
3159.4076 & 0.99982355 & 1.0000372  \\
3159.4280 & 0.99983639 & 1.0000396  \\
3159.4485 & 0.99982998 & 1.0000233  \\
3159.4689 & 0.99985408 & 1.0000378  \\
3159.4893 & 0.99983377 & 1.0000082  \\
3159.5098 & 0.99984361 & 1.0000091  \\
3159.5302 & 0.99983276 & 0.99998976 \\
3159.5506 & 0.99989799 & 1.0000467  \\
3159.5915 & 0.99987109 & 1.0000042  \\
3159.6119 & 0.99982880 & 0.99995468 \\
3159.6323 & 0.99982317 & 0.99994208 \\
3159.6528 & 0.99982485 & 0.99993702 \\
3159.6732 & 0.99984415 & 0.99995018 \\
3159.6936 & 0.99986570 & 0.99996566 \\
3159.7141 & 0.99985275 & 0.99994704 \\
3159.7345 & 0.99986576 & 0.99995469 \\
3159.7549 & 0.99997173 & 1.0000555  \\
3159.7754 & 0.99998325 & 1.0000624  \\
3159.7958 & 0.99998507 & 1.0000598  \\
3159.8367 & 0.99997136 & 1.0000379  \\
3159.8571 & 0.99998083 & 1.0000440  \\
3159.8775 & 0.99999278 & 1.0000527  \\
3159.8980 & 0.99999556 & 1.0000526  \\
3159.9184 & 0.99999770 & 1.0000518  \\
3159.9388 & 0.99998841 & 1.0000402  \\
3159.9593 & 0.99997921 & 1.0000289  \\
3159.9797 & 0.99999228 & 1.0000400  \\
3160.0206 & 1.0000211  & 1.0000660  \\
3160.0410 & 1.0000395  & 1.0000833  \\
3160.0819 & 0.99987305 & 0.99991561 \\
3160.1023 & 0.99989836 & 0.99994079 \\
3160.1227 & 0.99993231 & 0.99997475 \\
3160.1432 & 0.99993562 & 0.99997824 \\
3160.1636 & 0.99997843 & 1.0000216  \\
3160.1840 & 0.99999966 & 1.0000437  \\
3160.2045 & 0.99991442 & 0.99995942 \\
3160.2249 & 0.99996563 & 1.0000118  \\
3160.2453 & 0.99998115 & 1.0000288  \\
3160.2657 & 0.99993424 & 0.99998353 \\
3160.2862 & 0.99992643 & 0.99997757 \\
3160.3475 & 0.99992195 & 0.99997959 \\
3160.3679 & 0.99988302 & 0.99994322 \\
3160.3883 & 0.99994754 & 1.0000104  \\
3160.4088 & 0.99995866 & 1.0000245  \\
3160.4292 & 0.99994174 & 1.0000106  \\
3160.4496 & 0.99988726 & 0.99995926 \\
3160.4701 & 0.99990214 & 0.99997736 \\
3160.4905 & 0.99990991 & 0.99998835 \\
3160.5109 & 0.99986956 & 0.99995146 \\
3160.5314 & 0.99990081 & 0.99998635 \\
3160.5518 & 0.99991000 & 0.99999917 \\
3160.5722 & 0.99987442 & 0.99996728 \\
3160.5927 & 0.99984075 & 0.99993736 \\
3160.6131 & 0.99987149 & 0.99997192 \\
3160.6335 & 0.99987893 & 0.99998336 \\
3160.6540 & 0.99987307 & 0.99998137 \\
3160.6948 & 0.99989197 & 1.0000082  \\
3160.7153 & 0.99978813 & 0.99990846 \\
3160.7357 & 0.99982015 & 0.99994448 \\
3160.7561 & 0.99985390 & 0.99998223 \\
3160.7766 & 0.99989681 & 1.0000292  \\
3160.8174 & 0.99988390 & 1.0000243  \\
3160.8379 & 0.99984636 & 0.99999048 \\
3160.8583 & 0.99988614 & 1.0000343  \\
3160.8787 & 0.99982208 & 0.99997395 \\
3160.8991 & 0.99979984 & 0.99995558 \\
3160.9196 & 0.99985207 & 1.0000115  \\
3160.9400 & 0.99987227 & 1.0000354  \\
3160.9604 & 0.99985536 & 1.0000220  \\
3160.9809 & 0.99979297 & 0.99996308 \\
3161.0013 & 0.99985484 & 1.0000284  \\
3161.0217 & 0.99984645 & 1.0000231  \\
3161.0830 & 0.99985318 & 1.0000391  \\
3161.1035 & 0.99984333 & 1.0000319  \\
3161.1239 & 0.99988582 & 1.0000770  \\
3161.1443 & 0.99986342 & 1.0000571  \\
3161.1648 & 0.99988057 & 1.0000766  \\
3161.1852 & 0.99985538 & 1.0000538  \\
3161.2056 & 0.99982855 & 1.0000288  \\
3161.2261 & 0.99982528 & 1.0000274  \\
3161.2465 & 0.99983385 & 1.0000376  \\
3161.2669 & 0.99987300 & 1.0000782  \\
3161.2874 & 0.99978042 & 0.99998694 \\
3161.3282 & 0.99978121 & 0.99998959 \\
3161.3487 & 0.99981182 & 1.0000209  \\
3161.3691 & 0.99981566 & 1.0000251  \\
3161.3895 & 0.99976673 & 0.99997630 \\
3161.4100 & 0.99976148 & 0.99997092 \\
3161.4304 & 0.99972792 & 0.99993700 \\
3161.4508 & 0.99972004 & 0.99992858 \\
3161.4712 & 0.99980835 & 1.0000160  \\
3161.4917 & 0.99980134 & 1.0000080  \\
3161.5121 & 0.99980311 & 1.0000083  \\
3161.5530 & 0.99979934 & 1.0000009  \\
3161.5734 & 0.99980611 & 1.0000053  \\
3161.5938 & 0.99981336 & 1.0000100  \\
3161.6143 & 0.99978775 & 0.99998152 \\
3161.6347 & 0.99982379 & 1.0000142  \\
3161.6551 & 0.99978743 & 0.99997458 \\
3161.6756 & 0.99974375 & 0.99992690 \\
3161.6960 & 0.99978285 & 0.99996196 \\
3161.7164 & 0.99978786 & 0.99996243 \\
3161.7369 & 0.99979343 & 0.99996336 \\
3161.7573 & 0.99977764 & 0.99994262 \\
3161.7777 & 0.99981532 & 0.99997518 \\
3161.7982 & 0.99981502 & 0.99996933 \\
3161.8186 & 0.99982905 & 0.99997788 \\
3161.8390 & 0.99976465 & 0.99990757 \\
3161.8595 & 0.99976935 & 0.99990613 \\
3161.8799 & 0.99979936 & 0.99993007 \\
3161.9003 & 0.99998810 & 1.0001125  \\
3162.0434 & 0.99994932 & 1.0000265  \\
3162.0638 & 0.99999420 & 1.0000644  \\
3162.0842 & 0.99998973 & 1.0000529  \\
3162.1046 & 0.99999122 & 1.0000474  \\
3162.1251 & 0.99997782 & 1.0000271  \\
3162.1455 & 1.0000247  & 1.0000671  \\
3162.1659 & 1.0000297  & 1.0000653  \\
3162.1864 & 1.0000457  & 1.0000743  \\
3162.2068 & 1.0000153  & 1.0000372  \\
3162.2272 & 1.0000221  & 1.0000375  \\
3162.2477 & 1.0000519  & 1.0000607  \\
3162.3090 & 0.99998643 & 0.99997653 \\
3162.3294 & 0.99998485 & 0.99996887 \\
3162.3498 & 1.0000315  & 1.0000099  \\
3162.3703 & 0.99997614 & 0.99994896 \\
3162.3907 & 1.0000121  & 0.99997963 \\
3162.4111 & 0.99997234 & 0.99993479 \\
3162.4316 & 1.0000475  & 1.0000050  \\
3162.4520 & 1.0001003  & 1.0000535  \\
3162.4724 & 1.0001294  & 1.0000781  \\
3162.4929 & 1.0000553  & 0.99999961 \\
3162.5133 & 1.0000917  & 1.0000322  \\
3162.5337 & 1.0001375  & 1.0000740  \\
3162.5542 & 1.0000803  & 1.0000133  \\
3162.5746 & 1.0000660  & 0.99999583 \\
3162.5950 & 1.0000417  & 0.99996824 \\
3162.6155 & 1.0000612  & 0.99998495 \\
3162.6359 & 1.0000521  & 0.99997292 \\
3162.6563 & 1.0000604  & 0.99997859 \\
3162.6768 & 1.0000914  & 1.0000072  \\
3162.6972 & 1.0000925  & 1.0000062  \\
3162.7176 & 1.0000403  & 0.99995198 \\
3162.7380 & 1.0000540  & 0.99996384 \\
3162.7789 & 0.99995875 & 0.99986555 \\
3162.7993 & 0.99998828 & 0.99989363 \\
3162.8198 & 1.0000575  & 0.99996178 \\
3162.8402 & 1.0000322  & 0.99993545 \\
3162.8606 & 1.0000544  & 0.99995669 \\
3162.8811 & 1.0000299  & 0.99993145 \\
3162.9015 & 1.0000790  & 0.99998008 \\
3162.9219 & 1.0000762  & 0.99997674 \\
3162.9424 & 1.0000642  & 0.99996455 \\
3162.9628 & 1.0000797  & 0.99997976 \\
3162.9832 & 1.0001016  & 1.0000018  \\
3163.0037 & 1.0000778  & 0.99997815 \\
3163.0241 & 1.0001256  & 1.0000260  \\
3163.0445 & 1.0001902  & 1.0000910  \\
3163.0650 & 1.0001631  & 1.0000645  \\
3163.0854 & 1.0001900  & 1.0000919  \\
3163.1263 & 1.0002315  & 1.0001351  \\
3163.2693 & 1.0000583  & 0.99997010 \\
3163.2897 & 1.0000676  & 0.99998077 \\
3163.3101 & 1.0000995  & 1.0000142  \\
3163.3306 & 1.0000759  & 0.99999209 \\
3163.3714 & 1.0000777  & 0.99999699 \\
3163.3919 & 1.0000829  & 1.0000038  \\
3163.4123 & 1.0001293  & 1.0000516  \\
3163.4327 & 1.0000916  & 1.0000153  \\
3163.4532 & 1.0001530  & 1.0000783  \\
3163.4736 & 1.0001817  & 1.0001086  \\
3163.5145 & 1.0000872  & 1.0000168  \\
3163.5349 & 1.0000401  & 0.99997088 \\
3163.5553 & 1.0000546  & 0.99998682 \\
3163.5758 & 1.0000502  & 0.99998345 \\
3163.5962 & 1.0000411  & 0.99997532 \\
3163.6166 & 1.0000590  & 0.99999426 \\
3163.6371 & 1.0000256  & 0.99996158 \\
3163.6575 & 1.0000271  & 0.99996390 \\
3163.6779 & 1.0000093  & 0.99994687 \\
3163.6984 & 1.0000618  & 0.99999958 \\
3163.7188 & 1.0000233  & 0.99996156 \\
3163.7392 & 1.0000537  & 0.99999208 \\
3163.7597 & 1.0001001  & 1.0000385  \\
3163.7801 & 1.0000872  & 1.0000256  \\
3163.8005 & 1.0000655  & 1.0000034  \\
3163.8210 & 1.0000886  & 1.0000260  \\
3163.8414 & 1.0000514  & 0.99998807 \\
3163.8618 & 1.0000337  & 0.99996945 \\
3163.8822 & 1.0000734  & 1.0000079  \\
3163.9027 & 1.0000916  & 1.0000249  \\
3163.9231 & 1.0001036  & 1.0000353  \\
3163.9435 & 1.0000686  & 0.99999854 \\
3163.9640 & 1.0000393  & 0.99996714 \\
3163.9844 & 1.0001448  & 1.0000707  \\
3164.0048 & 1.0000662  & 0.99998952 \\
3164.0253 & 1.0000730  & 0.99999387 \\
3164.0457 & 1.0000811  & 0.99999947 \\
3164.0661 & 1.0000625  & 0.99997819 \\
3164.0866 & 1.0001304  & 1.0000431  \\
3164.1070 & 1.0000986  & 1.0000085  \\
3164.1274 & 1.0000475  & 0.99995438 \\
3164.1479 & 1.0000976  & 1.0000012  \\
3164.1683 & 1.0000826  & 0.99998316 \\
3164.1887 & 1.0001434  & 1.0000410  \\
3164.2092 & 1.0000846  & 0.99997889 \\
3164.2500 & 1.0001347  & 1.0000226  \\
3164.2705 & 1.0001005  & 0.99998524 \\
3164.2909 & 1.0000626  & 0.99994440 \\
3164.3113 & 1.0000953  & 0.99997391 \\
3164.3318 & 1.0001313  & 1.0000069  \\
3164.3522 & 1.0001323  & 1.0000052  \\
3164.3726 & 1.0001354  & 1.0000054  \\
3164.3931 & 1.0000820  & 0.99994942 \\
3164.4135 & 1.0001184  & 0.99998323 \\
3164.4339 & 1.0001018  & 0.99996424 \\
3164.4544 & 1.0000855  & 0.99994577 \\
3164.4952 & 1.0001325  & 0.99998902 \\
3164.5156 & 1.0001657  & 1.0000204  \\
3164.5361 & 1.0001488  & 1.0000022  \\
3164.5565 & 1.0001361  & 0.99998818 \\
3164.5769 & 1.0001236  & 0.99997467 \\
3164.5974 & 1.0001649  & 1.0000153  \\
3164.6178 & 1.0001540  & 1.0000041  \\
3164.6587 & 1.0001361  & 0.99998621 \\
3164.6791 & 1.0001475  & 0.99999815 \\
3164.6995 & 1.0001572  & 1.0000086  \\
3164.7200 & 1.0001613  & 1.0000140  \\
3164.7404 & 1.0001297  & 0.99998347 \\
3164.7608 & 1.0001297  & 0.99998514 \\
3164.7813 & 1.0001497  & 1.0000069  \\
3164.8017 & 1.0002437  & 1.0001031  \\
3164.8221 & 1.0001643  & 1.0000258  \\
3164.8426 & 1.0001882  & 1.0000522  \\
3164.8630 & 1.0001080  & 0.99997461 \\
3164.8834 & 1.0002008  & 1.0000700  \\
3164.9039 & 1.0001478  & 1.0000200  \\
3164.9243 & 1.0001272  & 1.0000023  \\
3164.9447 & 1.0001163  & 0.99999448 \\
3164.9652 & 1.0001444  & 1.0000258  \\
3164.9856 & 1.0001653  & 1.0000500  \\
3165.0060 & 1.0000595  & 0.99994746 \\
3165.0265 & 1.0000992  & 0.99999058 \\
3165.0469 & 1.0001099  & 1.0000048  \\
3165.0673 & 1.0001382  & 1.0000365  \\
3165.0877 & 1.0000581  & 0.99995977 \\
3165.1082 & 1.0001237  & 1.0000287  \\
3165.1286 & 1.0001083  & 1.0000167  \\
3165.1490 & 1.0000839  & 0.99999557 \\
3165.1695 & 1.0000771  & 0.99999218 \\
3165.1899 & 1.0000663  & 0.99998463 \\
3165.2103 & 1.0000392  & 0.99996051 \\
3165.2308 & 1.0000566  & 0.99998088 \\
3165.2512 & 1.0000793  & 1.0000065  \\
3165.2716 & 1.0000941  & 1.0000241  \\
3165.2921 & 1.0000970  & 1.0000295  \\
3165.3125 & 1.0000496  & 0.99998450 \\
3165.3329 & 1.0000704  & 1.0000072  \\
3165.3534 & 1.0000383  & 0.99997735 \\
3165.3738 & 1.0000073  & 0.99994820 \\
3165.3942 & 1.0000524  & 0.99999469 \\
3165.4147 & 1.0000079  & 0.99995152 \\
3165.4351 & 1.0000423  & 0.99998697 \\
3165.4555 & 1.0000478  & 0.99999328 \\
3165.4760 & 1.0000565  & 1.0000025  \\
3165.4964 & 1.0000127  & 0.99995910 \\
3165.5168 & 1.0000703  & 1.0000168  \\
3165.5373 & 1.0000156  & 0.99996193 \\
3165.5577 & 1.0000574  & 1.0000034  \\
3165.5781 & 1.0000144  & 0.99995990 \\
3165.5986 & 1.0001127  & 1.0000574  \\
3165.6190 & 1.0000568  & 1.0000005  \\
3165.6394 & 1.0000231  & 0.99996579 \\
3165.6598 & 1.0000429  & 0.99998418 \\
3165.6803 & 1.0000956  & 1.0000353  \\
3165.7211 & 1.0000493  & 0.99998554 \\
3165.7416 & 1.0000788  & 1.0000130  \\
3165.7620 & 1.0000859  & 1.0000178  \\
3165.7824 & 1.0001143  & 1.0000438  \\
3165.8029 & 1.0000863  & 1.0000133  \\
3165.8233 & 1.0000557  & 0.99998012 \\
3165.8437 & 1.0000850  & 1.0000067  \\
3165.8642 & 1.0000893  & 1.0000080  \\
3165.8846 & 1.0001094  & 1.0000250  \\
3165.9050 & 1.0000826  & 0.99999502 \\
3165.9255 & 1.0000942  & 1.0000035  \\
3165.9459 & 1.0001016  & 1.0000075  \\
3165.9663 & 1.0001039  & 1.0000063  \\
3165.9868 & 1.0001551  & 1.0000536  \\
3166.0072 & 1.0001002  & 0.99999504 \\
3166.0276 & 1.0000788  & 0.99997000 \\
3166.0481 & 1.0001149  & 1.0000020  \\
3166.0685 & 1.0001085  & 0.99999182 \\
3166.0889 & 1.0000918  & 0.99997100 \\
3166.1094 & 1.0001335  & 1.0000086  \\
3166.1298 & 1.0001610  & 1.0000319  \\
3166.1502 & 1.0001269  & 0.99999366 \\
3166.1707 & 1.0001107  & 0.99997315 \\
3166.2115 & 1.0002057  & 1.0000596  \\
3166.2319 & 1.0001962  & 1.0000456  \\
3166.2524 & 1.0001729  & 1.0000181  \\
3166.2728 & 1.0002438  & 1.0000844  \\
3166.2932 & 1.0001831  & 1.0000194  \\
3166.3137 & 1.0001412  & 0.99997302 \\
3166.3341 & 1.0002057  & 1.0000330  \\
3166.3545 & 1.0001957  & 1.0000187  \\
3166.3750 & 1.0001957  & 1.0000144  \\
3166.3954 & 1.0001704  & 0.99998456 \\
3166.4158 & 1.0001503  & 0.99996004 \\
3166.4363 & 1.0001717  & 0.99997727 \\
3166.4567 & 1.0001901  & 0.99999140 \\
3166.4771 & 1.0001302  & 0.99992721 \\
3166.4976 & 1.0001302  & 0.99992328 \\
3166.5180 & 1.0001348  & 0.99992378 \\
3166.5384 & 1.0001809  & 0.99996587 \\
3166.5589 & 1.0001478  & 0.99992880 \\
3166.5793 & 1.0001589  & 0.99993636 \\
3166.5997 & 1.0001948  & 0.99996829 \\
3166.6202 & 1.0002682  & 1.0000381  \\
3166.6406 & 1.0002601  & 1.0000266  \\
3166.6610 & 1.0002610  & 1.0000240  \\
3166.6815 & 1.0002721  & 1.0000320  \\
3166.7019 & 1.0002613  & 1.0000180  \\
3166.7836 & 1.0003147  & 1.0000607  \\
3166.8040 & 1.0002828  & 1.0000264  \\
3166.8245 & 1.0002583  & 0.99999962 \\
3166.8449 & 1.0002868  & 1.0000262  \\
3166.8653 & 1.0003083  & 1.0000459  \\
3166.8858 & 1.0002590  & 0.99999493 \\
3166.9062 & 1.0002447  & 0.99997932 \\
3166.9266 & 1.0002293  & 0.99996274 \\
3166.9471 & 1.0002389  & 0.99997139 \\
3166.9675 & 1.0002477  & 0.99997932 \\
3166.9879 & 1.0002604  & 0.99999157 \\
3167.0084 & 1.0002498  & 0.99998047 \\
3167.0288 & 1.0002475  & 0.99997798 \\
3167.0492 & 1.0002518  & 0.99998210 \\
3167.0697 & 1.0002618  & 0.99999227 \\
3167.0901 & 1.0002537  & 0.99998458 \\
3167.1105 & 1.0002719  & 1.0000030  \\
3167.1310 & 1.0002904  & 1.0000221  \\
3167.1514 & 1.0002580  & 0.99999039 \\
3167.1718 & 1.0002671  & 1.0000003  \\
3167.1923 & 1.0002932  & 1.0000271  \\
3167.2127 & 1.0002707  & 1.0000057  \\
3167.2331 & 1.0003100  & 1.0000460  \\
3167.2536 & 1.0002696  & 1.0000068  \\
3167.2740 & 1.0002837  & 1.0000223  \\
3167.2944 & 1.0002577  & 0.99999760 \\
3167.3148 & 1.0003068  & 1.0000480  \\
3167.3353 & 1.0002474  & 0.99999016 \\
3167.3557 & 1.0002752  & 1.0000193  \\
3167.3761 & 1.0002754  & 1.0000213  \\
3167.3966 & 1.0002381  & 0.99998552 \\
3167.4170 & 1.0002607  & 1.0000098  \\
3167.4374 & 1.0002779  & 1.0000285  \\
3167.4579 & 1.0002325  & 0.99998478 \\
3167.4783 & 1.0003020  & 1.0000561  \\
3167.4987 & 1.0002494  & 1.0000052  \\
3167.5192 & 1.0002904  & 1.0000479  \\
3167.5396 & 1.0002180  & 0.99997704 \\
3167.5600 & 1.0002419  & 1.0000027  \\
3167.5805 & 1.0002202  & 0.99998249 \\
3167.6009 & 1.0002353  & 0.99999923 \\
3167.6213 & 1.0002526  & 1.0000180  \\
3167.6418 & 1.0002536  & 1.0000204  \\
3167.6826 & 1.0002371  & 1.0000069  \\
3167.7031 & 1.0002244  & 0.99999532 \\
3167.7235 & 1.0002077  & 0.99997992 \\
3167.7439 & 1.0002522  & 1.0000256  \\
3167.7644 & 1.0002084  & 0.99998314 \\
3167.7848 & 1.0002002  & 0.99997587 \\
3167.8052 & 1.0002782  & 1.0000549  \\
3167.8257 & 1.0002127  & 0.99999036 \\
3167.8461 & 1.0001708  & 0.99994946 \\
3167.8665 & 1.0002539  & 1.0000336  \\
3167.8869 & 1.0001762  & 0.99995673 \\
3167.9074 & 1.0001841  & 0.99996559 \\
3167.9278 & 1.0001621  & 0.99994437 \\
3167.9482 & 1.0002374  & 1.0000207  \\
3167.9687 & 1.0001984  & 0.99998261 \\
3167.9891 & 1.0002141  & 0.99999900 \\
3168.0095 & 1.0001874  & 0.99997344 \\
3168.0300 & 1.0001335  & 0.99992038 \\
3168.0504 & 1.0002064  & 0.99999404 \\
3168.0708 & 1.0001676  & 0.99995623 \\
3168.0913 & 1.0001517  & 0.99994133 \\
3168.1117 & 1.0001636  & 0.99995415 \\
3168.1321 & 1.0002078  & 0.99999945 \\
3168.1730 & 1.0002131  & 1.0000069  \\
3168.1934 & 1.0002495  & 1.0000444  \\
3168.2139 & 1.0002822  & 1.0000782  \\
3168.2343 & 1.0002157  & 1.0000129  \\
3168.2547 & 1.0002615  & 1.0000599  \\
3168.2752 & 1.0002024  & 1.0000023  \\
3168.2956 & 1.0001847  & 0.99998570 \\
3168.3160 & 1.0002016  & 1.0000043  \\
3168.3365 & 1.0002084  & 1.0000126  \\
3168.3569 & 1.0001925  & 0.99999834 \\
3168.3773 & 1.0002205  & 1.0000280  \\
3168.3978 & 1.0001736  & 0.99998295 \\
3168.4182 & 1.0001798  & 0.99999095 \\
3168.4386 & 1.0001884  & 1.0000016  \\
3168.4590 & 1.0001949  & 1.0000101  \\
3168.4795 & 1.0001844  & 1.0000018  \\
3168.4999 & 1.0001622  & 0.99998169 \\
3168.5203 & 1.0001110  & 0.99993271 \\
3168.5408 & 1.0001462  & 0.99997025 \\
3168.5612 & 1.0001481  & 0.99997451 \\
3168.5816 & 1.0001502  & 0.99997898 \\
3168.6021 & 1.0001873  & 1.0000184  \\
3168.6225 & 1.0001984  & 1.0000321  \\
3168.6429 & 1.0002033  & 1.0000392  \\
3168.6634 & 1.0001509  & 0.99998933 \\
3168.6838 & 1.0001802  & 1.0000212  \\
3168.7042 & 1.0001628  & 1.0000062  \\
3168.7247 & 1.0002153  & 1.0000610  \\
3168.7655 & 1.0001680  & 1.0000185  \\
3168.7860 & 1.0001735  & 1.0000264  \\
3168.8064 & 1.0001321  & 0.99998713 \\
3168.8268 & 1.0001397  & 0.99999698 \\
3168.8473 & 1.0001554  & 1.0000148  \\
3168.8677 & 1.0001705  & 1.0000321  \\
3168.8881 & 1.0001650  & 1.0000284  \\
3168.9086 & 1.0001283  & 0.99999369 \\
3168.9290 & 1.0001482  & 1.0000154  \\
3168.9494 & 1.0001452  & 1.0000139  \\
3168.9698 & 1.0001609  & 1.0000313  \\
3168.9903 & 1.0001902  & 1.0000620  \\
3169.0107 & 1.0001783  & 1.0000515  \\
3169.0311 & 1.0001076  & 0.99998195 \\
3169.0516 & 1.0001113  & 0.99998677 \\
3169.0720 & 1.0000960  & 0.99997243 \\
3169.0924 & 1.0000461  & 0.99992329 \\
3169.1129 & 1.0001394  & 1.0000171  \\
3169.1333 & 1.0001146  & 0.99999264 \\
3169.1537 & 1.0000915  & 0.99996987 \\
3169.1742 & 1.0000830  & 0.99996152 \\
3169.1946 & 1.0000990  & 0.99997731 \\
3169.2150 & 1.0001045  & 0.99998228 \\
3169.2355 & 1.0000982  & 0.99997552 \\
3169.2559 & 1.0000577  & 0.99993444 \\
3169.2763 & 1.0001006  & 0.99997636 \\
3169.2968 & 1.0000824  & 0.99995737 \\
3169.3172 & 1.0002083  & 1.0000820  \\
3169.3581 & 1.0001632  & 1.0000346  \\
3169.3785 & 1.0000991  & 0.99996909 \\
3169.3989 & 1.0000867  & 0.99995499 \\
3169.4194 & 1.0001451  & 1.0000118  \\
3169.4398 & 1.0001299  & 0.99999491 \\
3169.4602 & 1.0001286  & 0.99999189 \\
3169.4806 & 1.0001586  & 1.0000202  \\
3169.5011 & 1.0001264  & 0.99998600 \\
3169.5215 & 1.0001394  & 0.99999711 \\
3169.5419 & 1.0001730  & 1.0000289  \\
3169.5624 & 1.0001942  & 1.0000480  \\
3169.5828 & 1.0001163  & 0.99996826 \\
3169.6032 & 1.0001631  & 1.0000131  \\
3169.6237 & 1.0001055  & 0.99995368 \\
3169.6441 & 1.0001921  & 1.0000382  \\
3169.6645 & 1.0002092  & 1.0000535  \\
3169.6850 & 1.0001818  & 1.0000242  \\
3169.7054 & 1.0001431  & 0.99998388 \\
3169.7258 & 1.0001663  & 1.0000052  \\
3169.7463 & 1.0001279  & 0.99996523 \\
3169.7667 & 1.0001817  & 1.0000174  \\
3169.7871 & 1.0001330  & 0.99996721 \\
3169.8076 & 1.0002121  & 1.0000449  \\
3169.8280 & 1.0001916  & 1.0000233  \\
3169.8484 & 1.0001338  & 0.99996427 \\
3169.8689 & 1.0002130  & 1.0000422  \\
3169.8893 & 1.0001432  & 0.99997158 \\
3169.9097 & 1.0000988  & 0.99992640 \\
3169.9302 & 1.0001902  & 1.0000174  \\
3169.9506 & 1.0001841  & 1.0000107  \\
3169.9710 & 1.0001275  & 0.99995366 \\
3169.9915 & 1.0001946  & 1.0000207  \\
3170.0119 & 1.0002123  & 1.0000384  \\
3170.0323 & 1.0001922  & 1.0000183  \\
3170.0527 & 1.0001572  & 0.99998365 \\
3170.0732 & 1.0001613  & 0.99998808 \\
3170.0936 & 1.0001980  & 1.0000250  \\
3170.1345 & 1.0001613  & 0.99998951 \\
3170.1549 & 1.0001394  & 0.99996842 \\
3170.1753 & 1.0001887  & 1.0000184  \\
3170.1958 & 1.0002040  & 1.0000348  \\
3170.2162 & 1.0001536  & 0.99998525 \\
3170.2366 & 1.0001751  & 1.0000079  \\
3170.2571 & 1.0001559  & 0.99998956 \\
3170.2775 & 1.0001507  & 0.99998561 \\
3170.2979 & 1.0001984  & 1.0000345  \\
3170.3184 & 1.0001660  & 1.0000033  \\
3170.6453 & 1.0001276  & 0.99998407 \\
3170.6657 & 1.0001365  & 0.99999395 \\
3170.6861 & 1.0001278  & 0.99998603 \\
3170.7066 & 1.0001384  & 0.99999728 \\
3170.7270 & 1.0000892  & 0.99994893 \\
3170.7474 & 1.0001312  & 0.99999134 \\
3170.7679 & 1.0001596  & 1.0000202  \\
3170.7883 & 1.0001400  & 1.0000010  \\
3170.8087 & 1.0001604  & 1.0000218  \\
3170.8292 & 1.0001497  & 1.0000112  \\
3170.8496 & 1.0001389  & 1.0000009  \\
3170.8700 & 1.0001512  & 1.0000130  \\
3170.8905 & 1.0001370  & 0.99999897 \\
3170.9109 & 1.0001255  & 0.99998744 \\
3170.9313 & 1.0001395  & 1.0000014  \\
3170.9518 & 1.0001371  & 0.99999889 \\
3170.9722 & 1.0001252  & 0.99998673 \\
3170.9926 & 1.0001479  & 1.0000092  \\
3171.0131 & 1.0001874  & 1.0000484  \\
3171.0335 & 1.0002181  & 1.0000786  \\
3171.0539 & 1.0000960  & 0.99995609 \\
3171.0743 & 1.0001338  & 0.99999350 \\
3171.0948 & 1.0000950  & 0.99995398 \\
3171.1152 & 1.0001306  & 0.99998894 \\
3171.1356 & 1.0001085  & 0.99996610 \\
3171.1561 & 1.0001522  & 1.0000091  \\
3171.1765 & 1.0001322  & 0.99998819 \\
3171.1969 & 1.0001162  & 0.99997140 \\
3171.2174 & 1.0001555  & 1.0000097  \\
3171.2378 & 1.0002141  & 1.0000674  \\
3171.2582 & 1.0001484  & 1.0000007  \\
3171.2787 & 1.0001531  & 1.0000043  \\
3171.2991 & 1.0001730  & 1.0000231  \\
3171.3195 & 1.0001645  & 1.0000132  \\
3171.3400 & 1.0001501  & 0.99999749 \\
3171.3604 & 1.0001551  & 1.0000014  \\
3171.3808 & 1.0001427  & 0.99998761 \\
3171.4013 & 1.0001606  & 1.0000040  \\
3171.4217 & 1.0001740  & 1.0000161  \\
3171.4421 & 1.0001712  & 1.0000115  \\
3171.4626 & 1.0001368  & 0.99997591 \\
3171.4830 & 1.0001680  & 1.0000057  \\
3171.5034 & 1.0001713  & 1.0000073  \\
3171.5239 & 1.0001590  & 0.99999337 \\
3171.5443 & 1.0001625  & 0.99999517 \\
3171.5647 & 1.0001307  & 0.99996165 \\
3171.6056 & 1.0001350  & 0.99996262 \\
3171.6260 & 1.0001602  & 0.99998620 \\
3171.6464 & 1.0001577  & 0.99998190 \\
3171.6669 & 1.0001139  & 0.99993643 \\
3171.6873 & 1.0001296  & 0.99995047 \\
3171.7077 & 1.0002171  & 1.0000364  \\
3171.7282 & 1.0001834  & 1.0000009  \\
3171.7486 & 1.0002186  & 1.0000344  \\
3171.7690 & 1.0002205  & 1.0000346  \\
3171.7895 & 1.0001886  & 1.0000012  \\
3171.8099 & 1.0002251  & 1.0000361  \\
3171.8303 & 1.0002457  & 1.0000551  \\
3171.8508 & 1.0001759  & 0.99998381 \\
3171.8712 & 1.0001979  & 1.0000043  \\
3171.8916 & 1.0001891  & 0.99999411 \\
3171.9121 & 1.0001840  & 0.99998763 \\
3171.9325 & 1.0001866  & 0.99998895 \\
3171.9529 & 1.0002038  & 1.0000049  \\
3171.9734 & 1.0002072  & 1.0000069  \\
3172.0142 & 1.0002194  & 1.0000171  \\
3172.0347 & 1.0002026  & 0.99999936 \\
3172.0551 & 1.0001985  & 0.99999419 \\
3172.1164 & 1.0002159  & 1.0000094  \\
3172.1368 & 1.0002357  & 1.0000287  \\
3172.1572 & 1.0002225  & 1.0000152  \\
3172.1777 & 1.0001939  & 0.99998617 \\
3172.1981 & 1.0002804  & 1.0000725  \\
3172.2185 & 1.0002111  & 1.0000030  \\
3172.2390 & 1.0001733  & 0.99996533 \\
3172.2594 & 1.0001826  & 0.99997462 \\
3172.2798 & 1.0002555  & 1.0000476  \\
3172.3003 & 1.0002122  & 1.0000044  \\
3172.3207 & 1.0001386  & 0.99993134 \\
3172.3411 & 1.0002341  & 1.0000270  \\
3172.3616 & 1.0001928  & 0.99998621 \\
3172.3820 & 1.0001887  & 0.99998264 \\
3172.4024 & 1.0001939  & 0.99998838 \\
3172.4229 & 1.0001992  & 0.99999425 \\
3172.4433 & 1.0002001  & 0.99999580 \\
3172.4637 & 1.0001903  & 0.99998680 \\
3172.4842 & 1.0001946  & 0.99999181 \\
3172.5046 & 1.0001929  & 0.99999101 \\
3172.5250 & 1.0002086  & 1.0000074  \\
3172.5455 & 1.0001889  & 0.99998849 \\
3172.5659 & 1.0002240  & 1.0000244  \\
3172.5863 & 1.0001784  & 0.99997978 \\
3172.6068 & 1.0001906  & 0.99999284 \\
3172.6272 & 1.0001353  & 0.99993849 \\
3172.6476 & 1.0001629  & 0.99996694 \\
3172.6680 & 1.0001838  & 0.99998851 \\
3172.6885 & 1.0001855  & 0.99999132 \\
3172.7089 & 1.0002155  & 1.0000220  \\
3172.7498 & 1.0002098  & 1.0000178  \\
3172.7702 & 1.0002008  & 1.0000097  \\
3172.7906 & 1.0001753  & 0.99998493 \\
3172.8315 & 1.0001981  & 1.0000087  \\
3172.8519 & 1.0002603  & 1.0000717  \\
3172.8724 & 1.0002057  & 1.0000176  \\
3172.8928 & 1.0002662  & 1.0000786  \\
3172.9132 & 1.0002269  & 1.0000396  \\
3172.9337 & 1.0001505  & 0.99996351 \\
3172.9541 & 1.0001955  & 1.0000088  \\
3172.9745 & 1.0001844  & 0.99999794 \\
3172.9950 & 1.0001817  & 0.99999513 \\
3173.0154 & 1.0001427  & 0.99995626 \\
3173.0358 & 1.0001870  & 1.0000005  \\
3173.0563 & 1.0001920  & 1.0000055  \\
3173.0767 & 1.0001151  & 0.99992835 \\
3173.0971 & 1.0001808  & 0.99999376 \\
3173.1176 & 1.0001857  & 0.99999846 \\
3173.1380 & 1.0001594  & 0.99997162 \\
3173.1584 & 1.0001750  & 0.99998691 \\
3173.1788 & 1.0002240  & 1.0000353  \\
3173.1993 & 1.0002557  & 1.0000664  \\
3173.2197 & 1.0001754  & 0.99998550 \\
3173.2401 & 1.0001864  & 0.99999595 \\
3173.2606 & 1.0001932  & 1.0000020  \\
3173.2810 & 1.0002067  & 1.0000146  \\
3173.3014 & 1.0001668  & 0.99997395 \\
3173.3219 & 1.0001610  & 0.99996745 \\
3173.3423 & 1.0001710  & 0.99997649 \\
3173.3627 & 1.0002257  & 1.0000300  \\
3173.3832 & 1.0002377  & 1.0000410  \\
3173.4036 & 1.0001742  & 0.99997658 \\
3173.4240 & 1.0002051  & 1.0000063  \\
3173.4445 & 1.0001834  & 0.99998345 \\
3173.4649 & 1.0002486  & 1.0000475  \\
3173.4853 & 1.0001811  & 0.99997873 \\
3173.5262 & 1.0002438  & 1.0000389  \\
3173.5466 & 1.0001831  & 0.99997675 \\
3173.5671 & 1.0002272  & 1.0000196  \\
3173.5875 & 1.0002422  & 1.0000332  \\
3173.6079 & 1.0002162  & 1.0000058  \\
3173.6284 & 1.0001998  & 0.99998787 \\
3173.6488 & 1.0002112  & 0.99999772 \\
3173.6692 & 1.0001960  & 0.99998102 \\
3173.6896 & 1.0001711  & 0.99995467 \\
3173.7101 & 1.0002120  & 0.99999394 \\
3173.7305 & 1.0002334  & 1.0000136  \\
3173.7509 & 1.0002039  & 0.99998275 \\
3173.7714 & 1.0002189  & 0.99999624 \\
3173.8122 & 1.0002156  & 0.99998953 \\
3173.8327 & 1.0001656  & 0.99993800 \\
3173.8531 & 1.0002913  & 1.0000619  \\
3173.8735 & 1.0002169  & 0.99998615 \\
3173.8940 & 1.0002290  & 0.99999658 \\
3173.9144 & 1.0002121  & 0.99997797 \\
3173.9348 & 1.0002507  & 1.0000150  \\
3173.9553 & 1.0002515  & 1.0000142  \\
3173.9757 & 1.0002476  & 1.0000088  \\
3173.9961 & 1.0002163  & 0.99997614 \\
3174.0166 & 1.0002615  & 1.0000199  \\
3174.0574 & 1.0003309  & 1.0000864  \\
3174.0779 & 1.0002266  & 0.99998080 \\
3174.0983 & 1.0002656  & 1.0000184  \\
3174.1187 & 1.0002283  & 0.99997989 \\
3174.1391 & 1.0002224  & 0.99997262 \\
3174.1596 & 1.0002683  & 1.0000173  \\
3174.1800 & 1.0002477  & 0.99999586 \\
3174.2004 & 1.0002481  & 0.99999504 \\
3174.2209 & 1.0002615  & 1.0000076  \\
3174.2413 & 1.0002488  & 0.99999406 \\
3174.2617 & 1.0002494  & 0.99999367 \\
3174.2822 & 1.0002461  & 0.99998984 \\
3174.3026 & 1.0003026  & 1.0000455  \\
3174.3230 & 1.0002556  & 0.99999808 \\
3174.3435 & 1.0002184  & 0.99996032 \\
3174.3639 & 1.0002348  & 0.99997648 \\
3174.3843 & 1.0002569  & 0.99999832 \\
3174.4048 & 1.0002212  & 0.99996243 \\
3174.4252 & 1.0002988  & 1.0000397  \\
3174.4456 & 1.0002633  & 1.0000043  \\
3174.5069 & 1.0002624  & 1.0000043  \\
3174.5478 & 1.0002831  & 1.0000257  \\
3174.5682 & 1.0002451  & 0.99998820 \\
3174.5887 & 1.0002505  & 0.99999429 \\
3174.6091 & 1.0002479  & 0.99999241 \\
3174.6295 & 1.0002613  & 1.0000064  \\
3174.6499 & 1.0002552  & 1.0000010  \\
3174.6704 & 1.0002007  & 0.99994734 \\
3174.6908 & 1.0002686  & 1.0000161  \\
3174.7112 & 1.0002736  & 1.0000220  \\
3174.7317 & 1.0002619  & 1.0000110  \\
3174.7521 & 1.0002292  & 0.99997912 \\
3174.7725 & 1.0002281  & 0.99997888 \\
3174.7930 & 1.0002185  & 0.99997006 \\
3174.8134 & 1.0002480  & 1.0000004  \\
3174.8338 & 1.0002638  & 1.0000169  \\
3174.8543 & 1.0002311  & 0.99998490 \\
3174.8747 & 1.0002179  & 0.99997254 \\
3174.8951 & 1.0002718  & 1.0000269  \\
3174.9156 & 1.0003006  & 1.0000564  \\
3174.9360 & 1.0002125  & 0.99996884 \\
3174.9564 & 1.0002837  & 1.0000405  \\
3174.9769 & 1.0002526  & 1.0000098  \\
3174.9973 & 1.0002253  & 0.99998286 \\
3175.0177 & 1.0002792  & 1.0000370  \\
3175.0382 & 1.0002644  & 1.0000223  \\
3175.0586 & 1.0002725  & 1.0000304  \\
3175.0790 & 1.0002203  & 0.99997816 \\
3175.0995 & 1.0002244  & 0.99998191 \\
3175.1199 & 1.0003152  & 1.0000724  \\
3175.1403 & 1.0001889  & 0.99994571 \\
3175.1607 & 1.0002605  & 1.0000167  \\
3175.1812 & 1.0002441  & 0.99999960 \\
3175.2016 & 1.0002304  & 0.99998479 \\
3175.2220 & 1.0003063  & 1.0000597  \\
3175.2425 & 1.0002296  & 0.99998184 \\
3175.2833 & 1.0001900  & 0.99993944 \\
3175.3038 & 1.0002700  & 1.0000178  \\
3175.3242 & 1.0002770  & 1.0000232  \\
3175.3446 & 1.0002010  & 0.99994555 \\
3175.3651 & 1.0002677  & 1.0000102  \\
3175.3855 & 1.0001696  & 0.99991026 \\
3175.4059 & 1.0002635  & 1.0000022  \\
3175.4264 & 1.0002583  & 0.99999501 \\
3175.4468 & 1.0002976  & 1.0000321  \\
3175.4672 & 1.0002694  & 1.0000017  \\
3175.4877 & 1.0002835  & 1.0000137  \\
3175.5081 & 1.0003267  & 1.0000547  \\
3175.5285 & 1.0002335  & 0.99995932 \\
3175.5490 & 1.0003217  & 1.0000451  \\
3175.5694 & 1.0003048  & 1.0000261  \\
3175.5898 & 1.0002791  & 0.99999811 \\
3175.6103 & 1.0002315  & 0.99994840 \\
3175.6307 & 1.0002441  & 0.99995868 \\
3175.6511 & 1.0002979  & 1.0000104  \\
3175.6715 & 1.0002871  & 0.99999763 \\
3175.6920 & 1.0002492  & 0.99995762 \\
3175.7328 & 1.0002634  & 0.99996798 \\
3175.7737 & 1.0002973  & 0.99999834 \\
3175.7941 & 1.0002962  & 0.99999552 \\
3175.8146 & 1.0003046  & 1.0000025  \\
3175.8350 & 1.0003039  & 1.0000006  \\
3175.8554 & 1.0003125  & 1.0000078  \\
3175.8759 & 1.0003047  & 0.99999889 \\
3175.8963 & 1.0003186  & 1.0000117  \\
3175.9167 & 1.0003275  & 1.0000198  \\
3175.9372 & 1.0003599  & 1.0000516  \\
3175.9576 & 1.0003266  & 1.0000178  \\
3175.9780 & 1.0003071  & 0.99999799 \\
3176.0189 & 1.0003053  & 0.99999607 \\
3176.0393 & 1.0003178  & 1.0000086  \\
3176.0598 & 1.0002930  & 0.99998410 \\
3176.0802 & 1.0002804  & 0.99997174 \\
3176.1006 & 1.0003492  & 1.0000413  \\
3176.1210 & 1.0003578  & 1.0000505  \\
3176.1415 & 1.0003270  & 1.0000205  \\
3176.1619 & 1.0002803  & 0.99997482 \\
3176.1823 & 1.0003523  & 1.0000476  \\
3176.2028 & 1.0002464  & 0.99994274 \\
3176.2232 & 1.0002689  & 0.99996635 \\
3176.2641 & 1.0002788  & 0.99997875 \\
3176.2845 & 1.0003261  & 1.0000276  \\
3176.3049 & 1.0003400  & 1.0000428  \\
3176.3254 & 1.0002873  & 0.99999152 \\
3176.3458 & 1.0002884  & 0.99999417 \\
3176.3662 & 1.0002800  & 0.99998738 \\
3176.3867 & 1.0002789  & 0.99998794 \\
3176.4071 & 1.0002028  & 0.99991335 \\
3176.4275 & 1.0002704  & 0.99998264 \\
3176.4480 & 1.0002942  & 1.0000081  \\
3176.4684 & 1.0002822  & 0.99999788 \\
3176.4888 & 1.0002720  & 0.99998925 \\
3176.5093 & 1.0002939  & 1.0000127  \\
3176.5297 & 1.0002719  & 0.99999233 \\
3176.5501 & 1.0002970  & 1.0000193  \\
3176.5706 & 1.0002760  & 0.99999989 \\
3176.5910 & 1.0002822  & 1.0000077  \\
3176.6114 & 1.0002398  & 0.99996673 \\
3176.6318 & 1.0003181  & 1.0000466  \\
3176.6523 & 1.0003194  & 1.0000491  \\
3176.6727 & 1.0002937  & 1.0000249  \\
3176.6931 & 1.0002731  & 1.0000056  \\
3176.7136 & 1.0002705  & 1.0000041  \\
3176.7544 & 1.0002581  & 0.99999422 \\
3176.7749 & 1.0002642  & 1.0000011  \\
3176.7953 & 1.0002688  & 1.0000069  \\
3176.8157 & 1.0002813  & 1.0000204  \\
3176.8362 & 1.0002633  & 1.0000032  \\
3176.8566 & 1.0002496  & 0.99999048 \\
3176.8770 & 1.0002662  & 1.0000079  \\
3176.8975 & 1.0002620  & 1.0000045  \\
3176.9179 & 1.0002821  & 1.0000253  \\
3176.9383 & 1.0001894  & 0.99993326 \\
3176.9588 & 1.0002332  & 0.99997790 \\
3176.9792 & 1.0002374  & 0.99998276 \\
3176.9996 & 1.0002622  & 1.0000083  \\
3177.0201 & 1.0001838  & 0.99993059 \\
3177.0405 & 1.0002971  & 1.0000445  \\
3177.0609 & 1.0002616  & 1.0000097  \\
3177.0814 & 1.0002876  & 1.0000364  \\
3177.1018 & 1.0002542  & 1.0000038  \\
3177.1222 & 1.0002159  & 0.99996602 \\
3177.1426 & 1.0002748  & 1.0000256  \\
3177.1631 & 1.0002463  & 0.99999794 \\
3177.1835 & 1.0002569  & 1.0000093  \\
3177.2039 & 1.0002644  & 1.0000176  \\
3177.2448 & 1.0002292  & 0.99998422 \\
3177.2652 & 1.0001985  & 0.99995437 \\
3177.2857 & 1.0002322  & 0.99998905 \\
3177.3061 & 1.0002498  & 1.0000076  \\
3177.3265 & 1.0002574  & 1.0000162  \\
3177.3470 & 1.0002099  & 0.99996980 \\
3177.3674 & 1.0002153  & 0.99997639 \\
3177.3878 & 1.0002236  & 0.99998604 \\
3177.4083 & 1.0002650  & 1.0000287  \\
3177.4287 & 1.0002155  & 0.99998071 \\
3177.4491 & 1.0002424  & 1.0000090  \\
3177.4696 & 1.0002270  & 0.99999507 \\
3177.4900 & 1.0001837  & 0.99995341 \\
3177.5104 & 1.0001997  & 0.99997120 \\
3177.5309 & 1.0002640  & 1.0000372  \\
3177.5513 & 1.0002293  & 1.0000043  \\
3177.5717 & 1.0002582  & 1.0000352  \\
3177.5921 & 1.0001986  & 0.99997760 \\
3177.6126 & 1.0002788  & 1.0000596  \\
3177.6330 & 1.0001751  & 0.99995810 \\
3177.6534 & 1.0002277  & 1.0000127  \\
3177.6739 & 1.0001862  & 0.99997349 \\
3177.6943 & 1.0002815  & 1.0000711  \\
3177.7352 & 1.0002067  & 1.0000008  \\
3177.7556 & 1.0001756  & 0.99997195 \\
3177.7760 & 1.0002377  & 1.0000364  \\
3177.7965 & 1.0002093  & 1.0000102  \\
3177.8169 & 1.0001849  & 0.99998809 \\
3177.8373 & 1.0002078  & 1.0000134  \\
3177.8578 & 1.0002387  & 1.0000467  \\
3177.8782 & 1.0002221  & 1.0000323  \\
3177.8986 & 1.0001815  & 0.99999423 \\
3177.9191 & 1.0001969  & 1.0000120  \\
3177.9395 & 1.0001757  & 0.99999323 \\
3177.9804 & 1.0001993  & 1.0000214  \\
3178.0008 & 1.0001474  & 0.99997191 \\
3178.0212 & 1.0001225  & 0.99994930 \\
3178.0417 & 1.0001818  & 1.0000109  \\
3178.0621 & 1.0001526  & 0.99998393 \\
3178.0825 & 1.0001678  & 1.0000014  \\
3178.1029 & 1.0001168  & 0.99995247 \\
3178.1234 & 1.0001676  & 1.0000055  \\
3178.1438 & 1.0001841  & 1.0000241  \\
3178.1642 & 1.0001378  & 0.99997971 \\
3178.1847 & 1.0001660  & 1.0000099  \\
3178.2051 & 1.0001776  & 1.0000236  \\
3178.2255 & 1.0001242  & 0.99997187 \\
3178.2460 & 1.0001567  & 1.0000062  \\
3178.2664 & 1.0001748  & 1.0000262  \\
3178.2868 & 1.0001490  & 1.0000020  \\
3178.3073 & 1.0001655  & 1.0000204  \\
3178.3277 & 1.0001040  & 0.99996045 \\
3178.3481 & 1.0001226  & 0.99998058 \\
3178.3890 & 1.0001428  & 1.0000036  \\
3178.4094 & 1.0001030  & 0.99996531 \\
3178.4299 & 1.0001319  & 0.99999575 \\
3178.4707 & 1.0001334  & 0.99999978 \\
3178.4912 & 1.0001520  & 1.0000196  \\
3178.5116 & 1.0001461  & 1.0000150  \\
3178.5320 & 1.0001119  & 0.99998180 \\
3178.5524 & 1.0001153  & 0.99998652 \\
3178.5729 & 1.0001099  & 0.99998221 \\
3178.5933 & 1.0001520  & 1.0000254  \\
3178.6137 & 1.0001301  & 1.0000045  \\
3178.6342 & 1.0001646  & 1.0000400  \\
3178.6546 & 1.0001244  & 1.0000008  \\
3178.6750 & 1.0001028  & 0.99997999 \\
3178.6955 & 1.0001294  & 1.0000075  \\
3178.7159 & 1.0001131  & 0.99999222 \\
3178.7363 & 1.0000745  & 0.99995442 \\
3178.7568 & 1.0001263  & 1.0000071  \\
3178.7772 & 1.0001546  & 1.0000363  \\
3178.7976 & 1.0001029  & 0.99998524 \\
3178.8181 & 1.0001350  & 1.0000180  \\
3178.8385 & 1.0001485  & 1.0000324  \\
3178.8589 & 1.0001767  & 1.0000612  \\
3178.8794 & 1.0000868  & 0.99997208 \\
3178.8998 & 1.0001250  & 1.0000110  \\
3178.9202 & 1.0000979  & 0.99998466 \\
3178.9611 & 1.0000552  & 0.99994330 \\
3178.9815 & 1.0001044  & 0.99999306 \\
3179.0019 & 1.0000894  & 0.99997851 \\
3179.0224 & 1.0000920  & 0.99998198 \\
3179.0428 & 1.0000758  & 0.99996640 \\
3179.0632 & 1.0000732  & 0.99996435 \\
3179.0837 & 1.0001372  & 1.0000290  \\
3179.1041 & 1.0000646  & 0.99995700 \\
3179.1450 & 1.0001196  & 1.0000131  \\
3179.1654 & 1.0001584  & 1.0000524  \\
3179.1858 & 1.0001150  & 1.0000095  \\
3179.2063 & 1.0001538  & 1.0000489  \\
3179.2267 & 1.0001477  & 1.0000433  \\
3179.2471 & 1.0001012  & 0.99999745 \\
3179.2676 & 1.0001041  & 1.0000008  \\
3179.2880 & 1.0000888  & 0.99998609 \\
3179.3084 & 1.0000724  & 0.99997025 \\
3179.3289 & 1.0001305  & 1.0000287  \\
3179.3493 & 1.0001425  & 1.0000413  \\
3179.3697 & 1.0001117  & 1.0000109  \\
3179.3902 & 1.0000889  & 0.99998861 \\
3179.4106 & 1.0000553  & 0.99995551 \\
3179.4310 & 1.0001591  & 1.0000598  \\
3179.4515 & 1.0001184  & 1.0000195  \\
3179.4719 & 1.0000653  & 0.99996693 \\
3179.4923 & 1.0000722  & 0.99997444 \\
3179.5127 & 1.0001100  & 1.0000127  \\
3179.5332 & 1.0000953  & 0.99999851 \\
3179.5740 & 1.0000744  & 0.99997864 \\
3179.5945 & 1.0000638  & 0.99996859 \\
3179.6353 & 1.0000671  & 0.99997297 \\
3179.6558 & 1.0001065  & 1.0000127  \\
3179.6966 & 1.0001158  & 1.0000231  \\
3179.7171 & 1.0001008  & 1.0000085  \\
3179.7375 & 1.0001329  & 1.0000411  \\
3179.7579 & 1.0000460  & 0.99995466 \\
3179.7784 & 1.0000854  & 0.99999483 \\
3179.7988 & 1.0000957  & 1.0000054  \\
3179.8192 & 1.0000323  & 0.99994271 \\
3179.8397 & 1.0000405  & 0.99995144 \\
3179.8601 & 1.0001036  & 1.0000150  \\
3179.8805 & 1.0000867  & 0.99999868 \\
3179.9010 & 1.0000941  & 1.0000067  \\
3179.9622 & 1.0000838  & 0.99999832 \\
3179.9827 & 1.0001054  & 1.0000204  \\
3180.0031 & 1.0000887  & 1.0000042  \\
3180.0235 & 1.0001210  & 1.0000372  \\
3180.0440 & 1.0001216  & 1.0000385  \\
3180.0644 & 1.0000944  & 1.0000119  \\
3180.0848 & 1.0000776  & 0.99999579 \\
3180.1053 & 1.0001150  & 1.0000339  \\
3180.1257 & 1.0000860  & 1.0000056  \\
3180.1461 & 1.0000678  & 0.99998818 \\
3180.1666 & 1.0001174  & 1.0000384  \\
3180.1870 & 1.0000873  & 1.0000091  \\
3180.2074 & 1.0000646  & 0.99998728 \\
3180.2279 & 1.0000747  & 0.99999819 \\
3180.2483 & 1.0000395  & 0.99996369 \\
3180.2687 & 1.0000144  & 0.99993938 \\
3180.2892 & 1.0000714  & 0.99999748 \\
3180.3096 & 1.0000764  & 1.0000032  \\
3180.3505 & 1.0000922  & 1.0000208  \\
3180.3709 & 1.0000436  & 0.99997312 \\
3180.3913 & 1.0000298  & 0.99996045 \\
3180.4117 & 1.0001049  & 1.0000365  \\
3180.4322 & 1.0000648  & 0.99999731 \\
3180.4526 & 1.0000366  & 0.99997022 \\
3180.4730 & 1.0000818  & 1.0000164  \\
3180.4935 & 1.0000436  & 0.99997923 \\
3180.5139 & 1.0000798  & 1.0000166  \\
3180.5343 & 1.0000386  & 0.99997659 \\
3180.5548 & 1.0000699  & 1.0000090  \\
3180.5752 & 1.0000843  & 1.0000244  \\
3180.5956 & 1.0000820  & 1.0000234  \\
3180.6161 & 1.0000645  & 1.0000071  \\
3180.6365 & 1.0000267  & 0.99997052 \\
3180.6774 & 1.0000586  & 1.0000049  \\
3180.6978 & 1.0000501  & 0.99999764 \\
3180.7182 & 1.0000608  & 1.0000095  \\
3180.7387 & 1.0000431  & 0.99999299 \\
3180.7591 & 1.0000526  & 1.0000037  \\
3180.7795 & 1.0000191  & 0.99997152 \\
3180.8000 & 1.0000982  & 1.0000520  \\
3180.8204 & 1.0000827  & 1.0000376  \\
3180.8408 & 1.0000098  & 0.99996588 \\
3180.8613 & 1.0000425  & 0.99999995 \\
3180.8817 & 1.0000431  & 1.0000017  \\
3180.9021 & 1.0000380  & 0.99999787 \\
3180.9225 & 1.0000327  & 0.99999397 \\
3180.9430 & 0.99998628 & 0.99994873 \\
3180.9634 & 0.99997919 & 0.99994259 \\
3180.9838 & 1.0001020  & 1.0000666  \\
3181.0043 & 1.0000481  & 1.0000139  \\
3181.0247 & 1.0001039  & 1.0000709  \\
3181.0451 & 1.0000507  & 1.0000188  \\
3181.0656 & 1.0000475  & 1.0000166  \\
3181.0860 & 1.0000791  & 1.0000493  \\
3181.1064 & 1.0000436  & 1.0000148  \\
3181.1269 & 1.0000319  & 1.0000043  \\
3181.1677 & 0.99995733 & 0.99993170 \\
3181.1882 & 0.99999696 & 0.99997229 \\
3181.2086 & 0.99999673 & 0.99997289 \\
3181.2290 & 1.0000102  & 0.99998729 \\
3181.2699 & 1.0000275  & 1.0000063  \\
3181.2903 & 0.99998477 & 0.99996439 \\
3181.3108 & 0.99997226 & 0.99995247 \\
3181.3312 & 1.0000044  & 0.99998548 \\
3181.3516 & 0.99998785 & 0.99996961 \\
3181.3720 & 1.0000139  & 0.99999625 \\
3181.3925 & 0.99998365 & 0.99996673 \\
3181.4129 & 0.99999306 & 0.99997684 \\
3181.4333 & 1.0000211  & 1.0000055  \\
3181.4538 & 1.0000268  & 1.0000119  \\
3181.4742 & 1.0000093  & 0.99999484 \\
3181.4946 & 1.0000173  & 1.0000036  \\
3181.5151 & 1.0000474  & 1.0000340  \\
3181.5355 & 1.0000311  & 1.0000184  \\
3181.5559 & 1.0000696  & 1.0000573  \\
3181.5764 & 1.0000708  & 1.0000592  \\
3181.5968 & 1.0000451  & 1.0000340  \\
3181.6172 & 1.0000459  & 1.0000353  \\
3181.6581 & 1.0000199  & 1.0000102  \\
3181.6785 & 0.99998732 & 0.99997838 \\
3181.6990 & 1.0000204  & 1.0000120  \\
3181.7194 & 0.99999341 & 0.99998530 \\
3181.7398 & 0.99996050 & 0.99995311 \\
3181.7603 & 0.99997032 & 0.99996340 \\
3181.7807 & 0.99999247 & 0.99998592 \\
3181.8011 & 1.0000047  & 0.99999879 \\
3181.8215 & 1.0000632  & 1.0000577  \\
3181.8420 & 0.99996230 & 0.99995754 \\
3181.8624 & 1.0000254  & 1.0000211  \\
3181.9033 & 1.0000132  & 1.0000100  \\
3181.9237 & 0.99999393 & 0.99999131 \\
3181.9441 & 0.99998910 & 0.99998707 \\
3181.9646 & 1.0000035  & 1.0000020  \\
3181.9850 & 1.0000243  & 1.0000235  \\
3182.0054 & 1.0000204  & 1.0000202  \\
3182.0259 & 1.0000123  & 1.0000128  \\
3182.0463 & 1.0000240  & 1.0000250  \\
3182.0667 & 0.99999045 & 0.99999230 \\
3182.0872 & 1.0000148  & 1.0000173  \\
3182.1076 & 0.99998940 & 0.99999262 \\
3182.1280 & 0.99999118 & 0.99999494 \\
3182.1485 & 0.99998151 & 0.99998598 \\
3182.1689 & 1.0000078  & 1.0000128  \\
3182.1893 & 0.99998420 & 0.99998987 \\
3182.2098 & 1.0000200  & 1.0000262  \\
3182.2302 & 0.99993486 & 0.99994183 \\
3182.2506 & 0.99997730 & 0.99998457 \\
3182.2915 & 0.99999383 & 1.0000022  \\
3182.3119 & 1.0000221  & 1.0000310  \\
3182.3323 & 0.99996653 & 0.99997571 \\
3182.3528 & 0.99995129 & 0.99996089 \\
3182.3732 & 1.0000275  & 1.0000375  \\
3182.3936 & 0.99995286 & 0.99996305 \\
3182.4141 & 0.99997275 & 0.99998330 \\
3182.4345 & 0.99994337 & 0.99995398 \\
3182.4549 & 0.99997127 & 0.99998205 \\
3182.4754 & 1.0000069  & 1.0000178  \\
3182.4958 & 0.99999505 & 1.0000060  \\
3182.5162 & 0.99997578 & 0.99998663 \\
3182.5367 & 1.0000096  & 1.0000203  \\
3182.5571 & 1.0000181  & 1.0000286  \\
3182.5775 & 0.99994801 & 0.99995832 \\
3182.5980 & 0.99997812 & 0.99998795 \\
3182.6388 & 1.0000158  & 1.0000249  \\
3182.6593 & 0.99995655 & 0.99996489 \\
3182.6797 & 1.0000616  & 1.0000692  \\
3182.7001 & 1.0000121  & 1.0000188  \\
3182.7205 & 0.99999163 & 0.99999765 \\
3182.7410 & 0.99995332 & 0.99995833 \\
3182.7614 & 0.99997803 & 0.99998202 \\
3182.7818 & 0.99999448 & 0.99999722 \\
3182.8023 & 0.99998640 & 0.99998795 \\
3182.8227 & 1.0000122  & 1.0000124  \\
3182.8431 & 1.0000110  & 1.0000097  \\
3182.8840 & 0.99997622 & 0.99997204 \\
3182.9044 & 1.0000132  & 1.0000074  \\
3182.9249 & 1.0000064  & 0.99999877 \\
3182.9453 & 0.99999438 & 0.99998508 \\
3182.9657 & 1.0000923  & 1.0000813  \\
3182.9862 & 1.0000843  & 1.0000713  \\
3183.0066 & 1.0000259  & 1.0000112  \\
3183.0270 & 1.0000626  & 1.0000459  \\
3183.0679 & 1.0000030  & 0.99998242 \\
3183.0883 & 1.0000038  & 0.99998119 \\
3183.1088 & 1.0000380  & 1.0000134  \\
3183.1292 & 1.0000141  & 0.99998742 \\
3183.1496 & 1.0000250  & 0.99999624 \\
3183.1700 & 1.0000572  & 1.0000263  \\
3183.1905 & 1.0000380  & 1.0000050  \\
3183.2109 & 1.0000286  & 0.99999338 \\
3183.2313 & 1.0000665  & 1.0000293  \\
3183.2518 & 1.0000336  & 0.99999414 \\
3183.2722 & 1.0000147  & 0.99997335 \\
3183.2926 & 0.99999095 & 0.99994744 \\
3183.3131 & 1.0000034  & 0.99995790 \\
3183.3335 & 1.0000265  & 0.99997893 \\
3183.3744 & 1.0000095  & 0.99995789 \\
3183.3948 & 1.0000287  & 0.99997522 \\
3183.4152 & 1.0000901  & 1.0000348  \\
3183.4357 & 1.0001274  & 1.0000700  \\
3183.4561 & 1.0000541  & 0.99999486 \\
3183.4765 & 1.0000640  & 1.0000030  \\
3183.4970 & 1.0000486  & 0.99998575 \\
3183.5174 & 1.0000671  & 1.0000028  \\
3183.5378 & 1.0000497  & 0.99998368 \\
3183.5583 & 1.0000885  & 1.0000209  \\
3183.5787 & 1.0000371  & 0.99996797 \\
3183.5991 & 1.0000445  & 0.99997378 \\
3183.6195 & 1.0000857  & 1.0000136  \\
3183.6400 & 1.0000442  & 0.99997069 \\
3183.6604 & 1.0000871  & 1.0000121  \\
3183.6808 & 1.0000837  & 1.0000075  \\
3183.7013 & 1.0000798  & 1.0000023  \\
3183.7217 & 1.0001322  & 1.0000535  \\
3183.7421 & 1.0000948  & 1.0000150  \\
3183.7626 & 1.0000726  & 0.99999167 \\
3183.7830 & 1.0000439  & 0.99996191 \\
3183.8034 & 1.0000958  & 1.0000128  \\
3183.8239 & 1.0001362  & 1.0000522  \\
3183.8852 & 1.0000690  & 0.99998211 \\
3183.9056 & 1.0001123  & 1.0000247  \\
3183.9260 & 1.0000471  & 0.99995887 \\
3183.9465 & 1.0001118  & 1.0000227  \\
3183.9873 & 1.0000821  & 0.99999178 \\
3184.0078 & 1.0000544  & 0.99996345 \\
3184.0282 & 1.0000546  & 0.99996304 \\
3184.0486 & 1.0000353  & 0.99994323 \\
3184.0690 & 1.0000956  & 1.0000031  \\
3184.0895 & 1.0001878  & 1.0000949  \\
3184.1099 & 1.0001265  & 1.0000331  \\
3184.1303 & 1.0000698  & 0.99997603 \\
3184.1508 & 1.0001084  & 1.0000144  \\
3184.1712 & 1.0000952  & 1.0000009  \\
3184.1916 & 1.0000835  & 0.99998887 \\
3184.2121 & 1.0000883  & 0.99999370 \\
3184.2325 & 1.0001045  & 1.0000097  \\
3184.2529 & 1.0001197  & 1.0000247  \\
3184.2734 & 1.0000636  & 0.99996855 \\
3184.2938 & 1.0000927  & 0.99999745 \\
3184.3142 & 1.0000762  & 0.99998109 \\
3184.3551 & 1.0000802  & 0.99998493 \\
3184.3755 & 1.0001019  & 1.0000067  \\
3184.3960 & 1.0001274  & 1.0000322  \\
3184.4164 & 1.0001122  & 1.0000171  \\
3184.4368 & 1.0001626  & 1.0000675  \\
3184.4573 & 1.0000817  & 0.99998676 \\
3184.4777 & 1.0000917  & 0.99999683 \\
3184.4981 & 1.0001070  & 1.0000123  \\
3184.5185 & 1.0001094  & 1.0000148  \\
3184.5390 & 1.0000824  & 0.99998786 \\
3184.5594 & 1.0000923  & 0.99999780 \\
3184.5798 & 1.0000426  & 0.99994808 \\
3184.6003 & 1.0000688  & 0.99997441 \\
3184.6207 & 1.0001028  & 1.0000084  \\
3184.6411 & 1.0000986  & 1.0000042  \\
3184.6616 & 1.0000901  & 0.99999570 \\
3184.6820 & 1.0000204  & 0.99992608 \\
3184.7024 & 1.0000922  & 0.99999774 \\
3184.7229 & 1.0000966  & 1.0000021  \\
3184.7433 & 1.0001016  & 1.0000068  \\
3184.7637 & 1.0000949  & 1.0000000  \\
3184.7842 & 1.0001177  & 1.0000227  \\
3184.8046 & 1.0000875  & 0.99999230 \\
3184.8455 & 1.0000779  & 0.99998218 \\
3184.8659 & 1.0000582  & 0.99996183 \\
3184.8863 & 1.0000870  & 0.99999028 \\
3184.9068 & 1.0001069  & 1.0000098  \\
3184.9272 & 1.0001533  & 1.0000556  \\
3184.9476 & 1.0001394  & 1.0000412  \\
3184.9680 & 1.0001160  & 1.0000171  \\
3184.9885 & 1.0001553  & 1.0000557  \\
3185.0089 & 1.0001096  & 1.0000094  \\
3185.0293 & 1.0001247  & 1.0000235  \\
3185.0498 & 1.0001010  & 0.99999898 \\
3185.0702 & 1.0000684  & 0.99996528 \\
3185.0906 & 1.0000975  & 0.99999327 \\
3185.1111 & 1.0000559  & 0.99995072 \\
3185.1315 & 1.0000669  & 0.99996060 \\
3185.1519 & 1.0001083  & 1.0000009  \\
3185.1724 & 1.0001371  & 1.0000286  \\
3185.1928 & 1.0001037  & 0.99999412 \\
3185.2132 & 1.0001375  & 1.0000266  \\
3185.2337 & 1.0000727  & 0.99996073 \\
3185.2541 & 1.0000876  & 0.99997436 \\
3185.2745 & 1.0001193  & 1.0000048  \\
3185.2950 & 1.0001271  & 1.0000115  \\
3185.3358 & 1.0001306  & 1.0000125  \\
3185.3563 & 1.0001018  & 0.99998246 \\
3185.3767 & 1.0001169  & 0.99999639 \\
3185.3971 & 1.0000882  & 0.99996652 \\
3185.4175 & 1.0001842  & 1.0000612  \\
3185.4380 & 1.0001564  & 1.0000325  \\
3185.4584 & 1.0001234  & 0.99999836 \\
3185.4788 & 1.0001468  & 1.0000207  \\
3185.4993 & 1.0000901  & 0.99996291 \\
3185.5197 & 1.0001564  & 1.0000282  \\
3185.5401 & 1.0001659  & 1.0000368  \\
3185.5606 & 1.0001394  & 1.0000095  \\
3185.5810 & 1.0001443  & 1.0000137  \\
3185.6014 & 1.0001615  & 1.0000300  \\
3185.6219 & 1.0000919  & 0.99995955 \\
3185.6423 & 1.0001041  & 0.99997135 \\
3185.6627 & 1.0001144  & 0.99998084 \\
3185.6832 & 1.0001246  & 0.99999075 \\
3185.7036 & 1.0001164  & 0.99998204 \\
3185.7240 & 1.0001227  & 0.99998811 \\
3185.7445 & 1.0001351  & 1.0000003  \\
3185.7649 & 1.0000981  & 0.99996316 \\
3185.7853 & 1.0001102  & 0.99997527 \\
3185.8262 & 1.0001438  & 1.0000089  \\
3185.8466 & 1.0001031  & 0.99996826 \\
3185.8670 & 1.0001265  & 0.99999204 \\
3185.8875 & 1.0001351  & 1.0000010  \\
3185.9079 & 1.0001323  & 0.99999832 \\
3185.9283 & 1.0001718  & 1.0000383  \\
3185.9488 & 1.0001722  & 1.0000392  \\
3185.9692 & 1.0001108  & 0.99997814 \\
3185.9896 & 1.0001199  & 0.99998785 \\
3186.0101 & 1.0000696  & 0.99993799 \\
3186.0305 & 1.0001529  & 1.0000219  \\
3186.0714 & 1.0001886  & 1.0000588  \\
3186.0918 & 1.0001670  & 1.0000378  \\
3186.1122 & 1.0000854  & 0.99995682 \\
3186.1327 & 1.0001106  & 0.99998244 \\
3186.1531 & 1.0001357  & 1.0000083  \\
3186.1735 & 1.0001170  & 0.99999008 \\
3186.1940 & 1.0001713  & 1.0000450  \\
3186.2144 & 1.0001125  & 0.99998675 \\
3186.2348 & 1.0001230  & 0.99999785 \\
3186.2553 & 1.0001157  & 0.99999113 \\
3186.2757 & 1.0001263  & 1.0000024  \\
3186.2961 & 1.0001495  & 1.0000260  \\
3186.3165 & 1.0001152  & 0.99999210 \\
3186.3370 & 1.0001320  & 1.0000094  \\
3186.3574 & 1.0001467  & 1.0000245  \\
3186.3778 & 1.0001509  & 1.0000289  \\
3186.3983 & 1.0001499  & 1.0000281  \\
3186.4187 & 1.0000747  & 0.99995316 \\
3186.4391 & 1.0001233  & 1.0000018  \\
3186.4596 & 1.0001785  & 1.0000570  \\
3186.4800 & 1.0001422  & 1.0000208  \\
3186.5004 & 1.0001540  & 1.0000325  \\
3186.5209 & 1.0001192  & 0.99999760 \\
3186.5617 & 1.0001285  & 1.0000063  \\
3186.5822 & 1.0000733  & 0.99995065 \\
3186.6026 & 1.0001707  & 1.0000478  \\
3186.6230 & 1.0001026  & 0.99997924 \\
3186.6435 & 1.0001375  & 1.0000134  \\
3186.6639 & 1.0001199  & 0.99999530 \\
3186.6843 & 1.0001120  & 0.99998686 \\
3186.7048 & 1.0001308  & 1.0000050  \\
3186.7252 & 1.0001183  & 0.99999182 \\
3186.7456 & 1.0001402  & 1.0000131  \\
3186.7660 & 1.0000896  & 0.99996158 \\
3186.7865 & 1.0001044  & 0.99997561 \\
3186.8069 & 1.0000990  & 0.99996946 \\
3186.8273 & 1.0001342  & 1.0000037  \\
3186.8478 & 1.0001223  & 0.99999117 \\
3186.8682 & 1.0001483  & 1.0000162  \\
3186.8886 & 1.0001146  & 0.99998159 \\
3186.9091 & 1.0000982  & 0.99996432 \\
3186.9295 & 1.0001164  & 0.99998170 \\
3186.9499 & 1.0001316  & 0.99999611 \\
3186.9704 & 1.0001270  & 0.99999051 \\
3186.9908 & 1.0001247  & 0.99998737 \\
3187.0112 & 1.0001260  & 0.99998785 \\
3187.0317 & 1.0001233  & 0.99998438 \\
3187.0521 & 1.0001499  & 1.0000102  \\
3187.0725 & 1.0001176  & 0.99997706 \\
3187.0930 & 1.0001282  & 0.99998698 \\
3187.1338 & 1.0001337  & 0.99999103 \\
3187.1543 & 1.0000756  & 0.99993229 \\
3187.1747 & 1.0001265  & 0.99998255 \\
3187.1951 & 1.0001332  & 0.99998877 \\
3187.2155 & 1.0001213  & 0.99997633 \\
3187.2360 & 1.0002125  & 1.0000669  \\
3187.2973 & 1.0001446  & 0.99999784 \\
3187.3177 & 1.0001786  & 1.0000317  \\
3187.3381 & 1.0001285  & 0.99998124 \\
3187.3586 & 1.0001609  & 1.0000136  \\
3187.3790 & 1.0001680  & 1.0000205  \\
3187.3994 & 1.0002011  & 1.0000534  \\
3187.4199 & 1.0001584  & 1.0000104  \\
3187.4403 & 1.0001184  & 0.99997075 \\
3187.4607 & 1.0001311  & 0.99998312 \\
3187.4812 & 1.0002288  & 1.0000808  \\
3187.5016 & 1.0001461  & 0.99999801 \\
3187.5220 & 1.0002190  & 1.0000709  \\
3187.5425 & 1.0001411  & 0.99999319 \\
3187.5629 & 1.0001711  & 1.0000231  \\
3187.5833 & 1.0001513  & 1.0000034  \\
3187.6037 & 1.0001647  & 1.0000168  \\
3187.6242 & 1.0001294  & 0.99998160 \\
3187.6446 & 1.0002077  & 1.0000600  \\
3187.6650 & 1.0001688  & 1.0000210  \\
3187.6855 & 1.0001442  & 0.99999650 \\
3187.7059 & 1.0001883  & 1.0000409  \\
3187.7263 & 1.0001758  & 1.0000282  \\
3187.7468 & 1.0001661  & 1.0000187  \\
3187.8081 & 1.0000992  & 0.99995158 \\
3187.8285 & 1.0001240  & 0.99997632 \\
3187.8489 & 1.0000981  & 0.99995043 \\
3187.8694 & 1.0001448  & 0.99999703 \\
3187.8898 & 1.0001138  & 0.99996570 \\
3187.9102 & 1.0001239  & 0.99997568 \\
3187.9307 & 1.0000716  & 0.99992323 \\
3187.9511 & 1.0001317  & 0.99998301 \\
3187.9920 & 1.0001460  & 0.99999655 \\
3188.0328 & 1.0001188  & 0.99996871 \\
3188.0532 & 1.0001746  & 1.0000240  \\
3188.0737 & 1.0001576  & 1.0000066  \\
3188.0941 & 1.0001606  & 1.0000092  \\
3188.1145 & 1.0001485  & 0.99999653 \\
3188.1554 & 1.0002025  & 1.0000493  \\
3188.1758 & 1.0002058  & 1.0000521  \\
3188.1963 & 1.0001332  & 0.99997885 \\
3188.2167 & 1.0001449  & 0.99998990 \\
3188.2371 & 1.0001825  & 1.0000269  \\
3188.2576 & 1.0000956  & 0.99993949 \\
3188.2780 & 1.0001664  & 1.0000095  \\
3188.2984 & 1.0001664  & 1.0000090  \\
3188.3189 & 1.0001759  & 1.0000178  \\
3188.3393 & 1.0001319  & 0.99997352 \\
3188.3597 & 1.0001728  & 1.0000138  \\
3188.3802 & 1.0001646  & 1.0000051  \\
3188.4006 & 1.0001639  & 1.0000038  \\
3188.4210 & 1.0001585  & 0.99999805 \\
3188.4415 & 1.0000995  & 0.99993860 \\
3188.4619 & 1.0001539  & 0.99999245 \\
3188.4823 & 1.0001659  & 1.0000042  \\
3188.5232 & 1.0001364  & 0.99997406 \\
3188.5436 & 1.0001851  & 1.0000226  \\
3188.5640 & 1.0001340  & 0.99997127 \\
3188.5845 & 1.0001718  & 1.0000090  \\
3188.6049 & 1.0001739  & 1.0000110  \\
3188.6253 & 1.0001456  & 0.99998275 \\
3188.6458 & 1.0001296  & 0.99996690 \\
3188.6662 & 1.0001707  & 1.0000081  \\
3188.6866 & 1.0001590  & 0.99999663 \\
3188.7071 & 1.0001807  & 1.0000187  \\
3188.7275 & 1.0001618  & 1.0000002  \\
3188.7479 & 1.0001974  & 1.0000364  \\
3188.7684 & 1.0002144  & 1.0000538  \\
3188.7888 & 1.0001730  & 1.0000131  \\
3188.8092 & 1.0001655  & 1.0000064  \\
3188.8297 & 1.0001633  & 1.0000050  \\
3188.8501 & 1.0001751  & 1.0000176  \\
3188.8705 & 1.0001487  & 0.99999220 \\
3188.8910 & 1.0001690  & 1.0000137  \\
3188.9114 & 1.0001730  & 1.0000185  \\
3188.9318 & 1.0001460  & 0.99999272 \\
3188.9522 & 1.0001401  & 0.99998791 \\
3188.9727 & 1.0001422  & 0.99999139 \\
3189.0135 & 1.0001599  & 1.0000116  \\
3189.0340 & 1.0001393  & 0.99999244 \\
3189.0544 & 1.0001113  & 0.99996574 \\
3189.0748 & 1.0001232  & 0.99997913 \\
3189.0953 & 1.0001796  & 1.0000371  \\
3189.1157 & 1.0001014  & 0.99996021 \\
3189.1361 & 1.0001544  & 1.0000147  \\
3189.1566 & 1.0001722  & 1.0000341  \\
3189.1770 & 1.0001111  & 0.99997434 \\
3189.1974 & 1.0001325  & 0.99999744 \\
3189.2179 & 1.0001643  & 1.0000308  \\
3189.2383 & 1.0001518  & 1.0000197  \\
3189.2587 & 1.0000972  & 0.99996669 \\
3189.2792 & 1.0001812  & 1.0000523  \\
3189.2996 & 1.0000966  & 0.99996929 \\
3189.3200 & 1.0000770  & 0.99995126 \\
3189.3404 & 1.0001431  & 1.0000187  \\
3189.3609 & 1.0001116  & 0.99998883 \\
3189.3813 & 1.0000729  & 0.99995155 \\
3189.4017 & 1.0000878  & 0.99996786 \\
3189.4222 & 1.0001364  & 1.0000179  \\
3189.4426 & 1.0001089  & 0.99999186 \\
3189.4630 & 1.0001249  & 1.0000092  \\
3189.5039 & 1.0001309  & 1.0000177  \\
3189.5243 & 1.0001178  & 1.0000057  \\
3189.5448 & 1.0001114  & 1.0000004  \\
3189.5652 & 1.0001610  & 1.0000512  \\
3189.5856 & 1.0000967  & 0.99998810 \\
3189.6061 & 1.0000929  & 0.99998537 \\
3189.6265 & 1.0000907  & 0.99998424 \\
3189.6469 & 1.0001000  & 0.99999442 \\
3189.6674 & 1.0000670  & 0.99996238 \\
3189.6878 & 1.0000703  & 0.99996669 \\
3189.7082 & 1.0000675  & 0.99996490 \\
3189.7695 & 1.0000950  & 0.99999509 \\
3189.7899 & 1.0001435  & 1.0000444  \\
3189.8104 & 1.0001452  & 1.0000470  \\
3189.8308 & 1.0000864  & 0.99998909 \\
3189.8512 & 1.0001333  & 1.0000368  \\
3189.8717 & 1.0001266  & 1.0000310  \\
3189.8921 & 1.0001152  & 1.0000206  \\
3189.9125 & 1.0001100  & 1.0000161  \\
3189.9330 & 1.0001114  & 1.0000184  \\
3189.9534 & 1.0000885  & 0.99999643 \\
3189.9943 & 1.0000842  & 0.99999369 \\
3190.0147 & 1.0000627  & 0.99997344 \\
3190.0351 & 1.0000980  & 1.0000095  \\
3190.0556 & 1.0000962  & 1.0000087  \\
3190.0760 & 1.0001182  & 1.0000317  \\
3190.0964 & 1.0000811  & 0.99999565 \\
3190.1169 & 1.0001129  & 1.0000284  \\
3190.1373 & 1.0000716  & 0.99998818 \\
3190.1577 & 1.0001142  & 1.0000318  \\
3190.1782 & 1.0001069  & 1.0000257  \\
3190.1986 & 1.0000658  & 0.99998568 \\
3190.2190 & 1.0000478  & 0.99996886 \\
3190.2394 & 1.0000708  & 0.99999321 \\
3190.2599 & 1.0000453  & 0.99996890 \\
3190.2803 & 1.0000809  & 1.0000058  \\
3190.3007 & 1.0000380  & 0.99996436 \\
3190.3212 & 1.0000469  & 0.99997449 \\
3190.3416 & 1.0000523  & 0.99998159 \\
3190.3620 & 1.0000244  & 0.99995502 \\
3190.3825 & 1.0000740  & 1.0000061  \\
3190.4029 & 1.0000316  & 0.99996519 \\
3190.4233 & 1.0000638  & 0.99999891 \\
3190.4438 & 1.0000601  & 0.99999691 \\
3190.4846 & 1.0000533  & 0.99999343 \\
3190.5051 & 1.0000666  & 1.0000084  \\
3190.5255 & 1.0000428  & 0.99998619 \\
3190.5459 & 1.0000530  & 0.99999820 \\
3190.5664 & 0.99997580 & 0.99992264 \\
3190.5868 & 1.0000698  & 1.0000184  \\
3190.6072 & 1.0000862  & 1.0000366  \\
3190.6276 & 1.0000802  & 1.0000323  \\
3190.6481 & 1.0000399  & 0.99999387 \\
3190.6685 & 1.0000313  & 0.99998712 \\
3190.6889 & 1.0000074  & 0.99996483 \\
3190.7094 & 1.0000369  & 0.99999623 \\
3190.7298 & 1.0000653  & 1.0000264  \\
3190.7502 & 1.0000448  & 1.0000078  \\
3190.7707 & 1.0000605  & 1.0000252  \\
3190.7911 & 1.0000209  & 0.99998729 \\
3190.8115 & 1.0000733  & 1.0000416  \\
3190.8320 & 1.0000814  & 1.0000515  \\
3190.8524 & 1.0000838  & 1.0000557  \\
3190.8728 & 1.0000418  & 1.0000155  \\
3190.8933 & 1.0000401  & 1.0000156  \\
3190.9137 & 1.0000525  & 1.0000298  \\
3190.9341 & 1.0000579  & 1.0000368  \\
3190.9750 & 1.0000336  & 1.0000160  \\
3190.9954 & 1.0000332  & 1.0000172  \\
3191.0159 & 1.0000360  & 1.0000220  \\
3191.0363 & 0.99994394 & 0.99993142 \\
3191.0567 & 0.99997537 & 0.99996452 \\
3191.0771 & 1.0000412  & 1.0000319  \\
3191.0976 & 1.0000319  & 1.0000243  \\
3191.1180 & 1.0000330  & 1.0000270  \\
3191.1384 & 0.99995011 & 0.99994570 \\
3191.1589 & 0.99994975 & 0.99994677 \\
3191.1793 & 1.0000180  & 1.0000166  \\
3191.1997 & 0.99999653 & 0.99999653 \\
3191.2202 & 1.0000078  & 1.0000093  \\
3191.2406 & 0.99997279 & 0.99997571 \\
3191.2610 & 0.99995953 & 0.99996394 \\
3191.2815 & 1.0000118  & 1.0000175  \\
3191.3019 & 1.0000042  & 1.0000113  \\
3191.3223 & 0.99997343 & 0.99998201 \\
3191.3428 & 1.0000012  & 1.0000111  \\
3191.3632 & 0.99995531 & 0.99996652 \\
3191.3836 & 0.99996489 & 0.99997740 \\
3191.4041 & 0.99997863 & 0.99999234 \\
3191.4245 & 0.99998616 & 1.0000012  \\
3191.4653 & 0.99999538 & 1.0000128  \\
3191.4858 & 0.99995505 & 0.99997365 \\
3191.5062 & 0.99994552 & 0.99996531 \\
3191.5266 & 0.99998600 & 1.0000069  \\
3191.5471 & 0.99993454 & 0.99995653 \\
3191.5675 & 0.99992256 & 0.99994569 \\
3191.6084 & 0.99996599 & 0.99999108 \\
3191.6288 & 0.99996158 & 0.99998769 \\
3191.6492 & 0.99997885 & 1.0000060  \\
3191.6697 & 1.0000267  & 1.0000547  \\
3191.7105 & 0.99998812 & 1.0000179  \\
3191.7310 & 0.99992952 & 0.99996021 \\
3191.7514 & 0.99997044 & 1.0000021  \\
3191.7718 & 0.99994797 & 0.99998033 \\
3191.7923 & 0.99999418 & 1.0000273  \\
3191.8127 & 0.99996610 & 1.0000001  \\
3191.8331 & 0.99996139 & 0.99999608 \\
3191.8536 & 0.99999429 & 1.0000297  \\
3191.8740 & 0.99998156 & 1.0000176  \\
3191.8944 & 0.99996584 & 1.0000027  \\
3191.9353 & 0.99993002 & 0.99996810 \\
3191.9557 & 0.99995834 & 0.99999703 \\
3191.9761 & 0.99995622 & 0.99999556 \\
3191.9966 & 0.99996405 & 1.0000041  \\
3192.0170 & 1.0000155  & 1.0000560  \\
3192.0374 & 0.99996885 & 1.0000099  \\
3192.0579 & 0.99997728 & 1.0000189  \\
3192.0783 & 0.99995810 & 1.0000004  \\
3192.0987 & 0.99998162 & 1.0000243  \\
3192.1192 & 1.0000019  & 1.0000452  \\
3192.1396 & 0.99994817 & 0.99999198 \\
3192.1600 & 0.99997788 & 1.0000223  \\
3192.2009 & 0.99994157 & 0.99998705 \\
3192.2213 & 0.99991970 & 0.99996553 \\
3192.2418 & 0.99997064 & 1.0000170  \\
3192.2622 & 0.99996728 & 1.0000143  \\
3192.2826 & 1.0000437  & 1.0000913  \\
3192.3235 & 0.99995341 & 1.0000018  \\
3192.3439 & 0.99995942 & 1.0000084  \\
3192.3643 & 0.99995572 & 1.0000053  \\
3192.3848 & 0.99995053 & 1.0000007  \\
3192.4052 & 0.99993583 & 0.99998649 \\
3192.4461 & 0.99994859 & 1.0000004  \\
3192.4665 & 0.99992956 & 0.99998201 \\
3192.4869 & 0.99998093 & 1.0000339  \\
3192.5074 & 0.99992535 & 0.99997888 \\
3192.5278 & 0.99992955 & 0.99998373 \\
3192.5482 & 0.99996788 & 1.0000227  \\
3192.5687 & 0.99991860 & 0.99997415 \\
3192.5891 & 0.99990719 & 0.99996328 \\
3192.6095 & 0.99995396 & 1.0000106  \\
3192.6300 & 0.99987507 & 0.99993252 \\
3192.6504 & 0.99989030 & 0.99994835 \\
3192.6708 & 0.99991640 & 0.99997523 \\
3192.6913 & 0.99993254 & 0.99999190 \\
3192.7117 & 0.99995320 & 1.0000133  \\
3192.7321 & 0.99994164 & 1.0000025  \\
3192.7525 & 0.99993821 & 0.99999961 \\
3192.7730 & 0.99994441 & 1.0000065  \\
3192.7934 & 0.99994334 & 1.0000061  \\
3192.8138 & 0.99992194 & 0.99998536 \\
3192.8343 & 0.99992927 & 0.99999317 \\
3192.8547 & 0.99993434 & 0.99999901 \\
3192.8751 & 0.99997374 & 1.0000389  \\
3192.8956 & 0.99990385 & 0.99996977 \\
3192.9364 & 0.99991359 & 0.99998065 \\
3192.9569 & 0.99992457 & 0.99999222 \\
3192.9773 & 0.99995688 & 1.0000251  \\
3192.9977 & 0.99993128 & 1.0000000  \\
3193.0182 & 0.99991286 & 0.99998188 \\
3193.0386 & 0.99991435 & 0.99998408 \\
3193.0590 & 0.99993628 & 1.0000064  \\
3193.0795 & 0.99996302 & 1.0000335  \\
3193.0999 & 0.99999386 & 1.0000647  \\
3193.1203 & 0.99992294 & 0.99999429 \\
3193.1408 & 0.99993871 & 1.0000104  \\
3193.1612 & 0.99988768 & 0.99995980 \\
3193.1816 & 0.99992729 & 0.99999953 \\
3193.2020 & 0.99993239 & 1.0000049  \\
3193.2225 & 0.99994796 & 1.0000207  \\
3193.2429 & 0.99995478 & 1.0000276  \\
3193.2633 & 0.99987539 & 0.99994834 \\
3193.2838 & 0.99989885 & 0.99997199 \\
3193.3042 & 0.99989970 & 0.99997295 \\
3193.3246 & 0.99991363 & 0.99998682 \\
3193.3451 & 0.99993448 & 1.0000079  \\
3193.3655 & 0.99989094 & 0.99996413 \\
3193.3859 & 0.99999060 & 1.0000639  \\
3193.4268 & 0.99993467 & 1.0000080  \\
3193.4472 & 0.99991854 & 0.99999191 \\
3193.4677 & 0.99992330 & 0.99999655 \\
3193.4881 & 0.99990236 & 0.99997567 \\
3193.5085 & 0.99990330 & 0.99997667 \\
3193.5290 & 0.99992500 & 0.99999832 \\
3193.5494 & 0.99995922 & 1.0000327  \\
3193.5698 & 0.99993209 & 1.0000058  \\
3193.5902 & 0.99996349 & 1.0000373  \\
3193.6107 & 0.99988037 & 0.99995428 \\
3193.6311 & 0.99994766 & 1.0000219  \\
3193.6924 & 0.99995082 & 1.0000263  \\
3193.7128 & 0.99995491 & 1.0000309  \\
3193.7333 & 0.99997439 & 1.0000509  \\
3193.7537 & 0.99992448 & 1.0000015  \\
3193.7741 & 0.99992774 & 1.0000057  \\
3193.7946 & 0.99992189 & 1.0000006  \\
3193.8150 & 0.99988636 & 0.99996605 \\
3193.8354 & 0.99993794 & 1.0000186  \\
3193.8559 & 0.99989433 & 0.99997634 \\
3193.8763 & 0.99998592 & 1.0000691  \\
3193.8967 & 0.99985583 & 0.99994028 \\
3193.9172 & 0.99992846 & 1.0000144  \\
3193.9376 & 0.99992709 & 1.0000146  \\
3193.9580 & 0.99992623 & 1.0000155  \\
3193.9785 & 0.99986073 & 0.99995180 \\
3193.9989 & 0.99992518 & 1.0000183  \\
3194.0193 & 0.99991975 & 1.0000150  \\
3194.0397 & 0.99988578 & 0.99998329 \\
3194.0602 & 0.99989281 & 0.99999276 \\
3194.0806 & 0.99995522 & 1.0000576  \\
3194.1010 & 0.99993451 & 1.0000395  \\
3194.1215 & 0.99988825 & 0.99999601 \\
3194.1623 & 0.99986656 & 0.99997993 \\
3194.1828 & 0.99986098 & 0.99997739 \\
3194.2032 & 0.99987417 & 0.99999373 \\
3194.2236 & 0.99988512 & 1.0000077  \\
3194.2441 & 0.99985125 & 0.99997695 \\
3194.2645 & 0.99987599 & 1.0000049  \\
3194.2849 & 0.99985121 & 0.99998329 \\
3194.3054 & 0.99990716 & 1.0000425  \\
3194.3258 & 0.99986160 & 1.0000002  \\
3194.3462 & 0.99985428 & 0.99999614 \\
3194.3667 & 0.99987322 & 1.0000183  \\
3194.3871 & 0.99980948 & 0.99995777 \\
3194.4075 & 0.99983173 & 0.99998324 \\
3194.4279 & 0.99982353 & 0.99997814 \\
3194.4484 & 0.99977912 & 0.99993700 \\
3194.4688 & 0.99983346 & 0.99999433 \\
3194.4892 & 0.99977211 & 0.99993613 \\
3194.5097 & 0.99983375 & 1.0000009  \\
3194.5301 & 0.99982783 & 0.99999788 \\
3194.5505 & 0.99981652 & 0.99998925 \\
3194.5710 & 0.99981114 & 0.99998656 \\
3194.5914 & 0.99983243 & 1.0000106  \\
3194.6118 & 0.99984914 & 1.0000299  \\
3194.6527 & 0.99979910 & 0.99998453 \\
3194.6731 & 0.99978687 & 0.99997438 \\
3194.6936 & 0.99978889 & 0.99997855 \\
3194.7140 & 0.99977765 & 0.99996915 \\
3194.7344 & 0.99977149 & 0.99996466 \\
3194.7549 & 0.99977267 & 0.99996751 \\
3194.7753 & 0.99976883 & 0.99996480 \\
3194.7957 & 0.99979527 & 0.99999256 \\
3194.8162 & 0.99987333 & 1.0000717  \\
3194.8366 & 0.99982490 & 1.0000241  \\
3194.8570 & 0.99981030 & 1.0000103  \\
3194.8774 & 0.99986990 & 1.0000704  \\
3194.8979 & 0.99980240 & 1.0000034  \\
3194.9183 & 0.99986657 & 1.0000678  \\
3194.9387 & 0.99982934 & 1.0000308  \\
3194.9592 & 0.99981203 & 1.0000136  \\
3194.9796 & 0.99982839 & 1.0000299  \\
3195.0000 & 0.99981349 & 1.0000148  \\
3195.0205 & 0.99978911 & 0.99999021 \\
3195.0409 & 0.99976189 & 0.99996264 \\
3195.0613 & 0.99983080 & 1.0000311  \\
3195.0818 & 0.99978959 & 0.99998932 \\
3195.1431 & 0.99981303 & 1.0000109  \\
3195.1635 & 0.99977880 & 0.99997573 \\
3195.1839 & 0.99981982 & 1.0000159  \\
3195.2044 & 0.99979717 & 0.99999226 \\
3195.2248 & 0.99981710 & 1.0000113  \\
3195.2452 & 0.99984706 & 1.0000403  \\
3195.2656 & 0.99986806 & 1.0000602  \\
3195.2861 & 0.99981878 & 1.0000100  \\
3195.3065 & 0.99977301 & 0.99996308 \\
3195.3269 & 0.99983911 & 1.0000282  \\
3195.3474 & 0.99981495 & 1.0000029  \\
3195.3678 & 0.99984186 & 1.0000289  \\
3195.3882 & 0.99982089 & 1.0000067  \\
3195.4087 & 0.99976044 & 0.99994532 \\
3195.4291 & 0.99978419 & 0.99996800 \\
3195.4700 & 0.99980318 & 0.99998503 \\
3195.4904 & 0.99981739 & 0.99999835 \\
3195.5313 & 0.99979036 & 0.99996947 \\
3195.5517 & 0.99981190 & 0.99999035 \\
3195.5721 & 0.99981519 & 0.99999293 \\
3195.5926 & 0.99975806 & 0.99993501 \\
3195.6334 & 0.99979869 & 0.99997446 \\
3195.6539 & 0.99985242 & 1.0000277  \\
3195.6743 & 0.99991774 & 1.0000926  \\
3195.6947 & 0.99984810 & 1.0000225  \\
3195.7151 & 0.99986089 & 1.0000350  \\
3195.7356 & 0.99976607 & 0.99993993 \\
3195.7560 & 0.99981828 & 0.99999191 \\
3195.7764 & 0.99979879 & 0.99997224 \\
3195.7969 & 0.99983018 & 1.0000036  \\
3195.8173 & 0.99988027 & 1.0000536  \\
3195.8377 & 0.99981263 & 0.99998602 \\
3195.8582 & 0.99981296 & 0.99998653 \\
3195.8786 & 0.99975666 & 0.99993034 \\
3195.8990 & 0.99980886 & 0.99998290 \\
3195.9195 & 0.99984848 & 1.0000228  \\
3195.9399 & 0.99990474 & 1.0000794  \\
3196.0012 & 0.99981096 & 0.99998745 \\
3196.0216 & 0.99980755 & 0.99998475 \\
3196.0421 & 0.99981444 & 0.99999260 \\
3196.0625 & 0.99979978 & 0.99997871 \\
3196.0829 & 0.99984090 & 1.0000209  \\
3196.1033 & 0.99982727 & 1.0000082  \\
3196.1238 & 0.99979559 & 0.99997768 \\
3196.1442 & 0.99977855 & 0.99996207 \\
3196.1646 & 0.99977091 & 0.99995579 \\
3196.1851 & 0.99976377 & 0.99994997 \\
3196.2055 & 0.99977891 & 0.99996660 \\
3196.2259 & 0.99976237 & 0.99995185 \\
3196.2464 & 0.99978614 & 0.99997729 \\
3196.2668 & 0.99979516 & 0.99998815 \\
3196.2872 & 0.99983519 & 1.0000301  \\
3196.3077 & 0.99986450 & 1.0000614  \\
3196.3281 & 0.99981240 & 1.0000114  \\
3196.3690 & 0.99978950 & 0.99999287 \\
3196.3894 & 0.99979079 & 0.99999643 \\
3196.4098 & 0.99980005 & 1.0000080  \\
3196.4303 & 0.99979599 & 1.0000062  \\
3196.4507 & 0.99979683 & 1.0000095  \\
3196.4711 & 0.99979925 & 1.0000142  \\
3196.4915 & 0.99978288 & 1.0000002  \\
3196.5120 & 0.99978829 & 1.0000079  \\
3196.5324 & 0.99983436 & 1.0000565  \\
3196.5528 & 0.99975314 & 0.99997749 \\
3196.5733 & 0.99977300 & 0.99999955 \\
3196.5937 & 0.99981618 & 1.0000451  \\
3196.6141 & 0.99979364 & 1.0000246  \\
3196.6346 & 0.99976975 & 1.0000030  \\
3196.6550 & 0.99975756 & 0.99999288 \\
3196.6754 & 0.99978661 & 1.0000238  \\
3196.6959 & 0.99978719 & 1.0000263  \\
3196.7163 & 0.99973790 & 0.99997875 \\
3196.7367 & 0.99977963 & 1.0000223  \\
3196.7572 & 0.99974308 & 0.99998722 \\
3196.7776 & 0.99978081 & 1.0000264  \\
3196.7980 & 0.99975694 & 1.0000037  \\
3196.8185 & 0.99976913 & 1.0000170  \\
3196.8389 & 0.99973111 & 0.99998007 \\
3196.8593 & 0.99977199 & 1.0000217  \\
3196.8798 & 0.99978428 & 1.0000346  \\
3196.9002 & 0.99977888 & 1.0000298  \\
3196.9206 & 0.99972320 & 0.99997431 \\
3196.9410 & 0.99976531 & 1.0000165  \\
3196.9615 & 0.99974850 & 0.99999961 \\
3196.9819 & 0.99975814 & 1.0000088  \\
3197.0023 & 0.99976184 & 1.0000121  \\
3197.0228 & 0.99971872 & 0.99996810 \\
3197.0432 & 0.99978289 & 1.0000312  \\
3197.0636 & 0.99977971 & 1.0000268  \\
3197.1045 & 0.99973176 & 0.99997560 \\
3197.1249 & 0.99976977 & 1.0000117  \\
3197.1454 & 0.99973460 & 0.99997456 \\
3197.1658 & 0.99977672 & 1.0000145  \\
3197.1862 & 0.99971307 & 0.99994844 \\
3197.2067 & 0.99976114 & 0.99999401 \\
3197.2271 & 0.99973879 & 0.99996898 \\
3197.2475 & 0.99976997 & 0.99999736 \\
3197.2680 & 0.99974850 & 0.99997315 \\
3197.2884 & 0.99977898 & 1.0000006  \\
3197.3088 & 0.99979699 & 1.0000156  \\
3197.3292 & 0.99977096 & 0.99998654 \\
3197.3497 & 0.99972945 & 0.99994193 \\
3197.3701 & 0.99977998 & 0.99998937 \\
3197.3905 & 0.99980306 & 1.0000092  \\
3197.4110 & 0.99977942 & 0.99998237 \\
3197.4314 & 0.99980112 & 1.0000008  \\
3197.4518 & 0.99979081 & 0.99998715 \\
3197.4723 & 0.99978639 & 0.99997951 \\
3197.4927 & 0.99984888 & 1.0000390  \\
3197.5131 & 0.99977891 & 0.99996582 \\
3197.5336 & 0.99979450 & 0.99997838 \\
3197.5949 & 0.99981796 & 0.99999290 \\
3197.6153 & 0.99982026 & 0.99999257 \\
3197.6357 & 0.99986466 & 1.0000342  \\
3197.6562 & 0.99981158 & 0.99997865 \\
3197.6766 & 0.99979029 & 0.99995497 \\
3197.6970 & 0.99978090 & 0.99994326 \\
3197.7175 & 0.99980605 & 0.99996632 \\
3197.7379 & 0.99981012 & 0.99996861 \\
3197.7583 & 0.99988246 & 1.0000392  \\
3197.7787 & 0.99982480 & 0.99998007 \\
3197.7992 & 0.99986670 & 1.0000206  \\
3197.8196 & 0.99985049 & 1.0000033  \\
3197.8400 & 0.99983577 & 0.99998758 \\
3197.8605 & 0.99984803 & 0.99999906 \\
3197.8809 & 0.99992374 & 1.0000741  \\
3197.9013 & 0.99989733 & 1.0000473  \\
3197.9218 & 0.99985231 & 1.0000020  \\
3197.9422 & 0.99986074 & 1.0000101  \\
3197.9626 & 0.99984121 & 0.99999058 \\
3197.9831 & 0.99985101 & 1.0000005  \\
3198.0035 & 0.99985834 & 1.0000081  \\
3198.0239 & 0.99985078 & 1.0000007  \\
3198.0444 & 0.99985530 & 1.0000057  \\
3198.0648 & 0.99989794 & 1.0000489  \\
3198.0852 & 0.99981340 & 0.99996491 \\
3198.1057 & 0.99985073 & 1.0000030  \\
3198.1261 & 0.99984736 & 1.0000003  \\
3198.1669 & 0.99987272 & 1.0000272  \\
3198.1874 & 0.99991057 & 1.0000661  \\
3198.2078 & 0.99983326 & 0.99998966 \\
3198.2282 & 0.99982849 & 0.99998596 \\
3198.2487 & 0.99987979 & 1.0000382  \\
3198.2691 & 0.99989113 & 1.0000506  \\
3198.2895 & 0.99985832 & 1.0000188  \\
3198.3100 & 0.99985079 & 1.0000124  \\
3198.3304 & 0.99980171 & 0.99996443 \\
3198.3508 & 0.99986755 & 1.0000313  \\
3198.3713 & 0.99983576 & 1.0000004  \\
3198.3917 & 0.99984492 & 1.0000106  \\
3198.4121 & 0.99985836 & 1.0000250  \\
3198.4326 & 0.99983989 & 1.0000074  \\
3198.4530 & 0.99982256 & 0.99999100 \\
3198.4734 & 0.99985066 & 1.0000199  \\
3198.4939 & 0.99984172 & 1.0000117  \\
3198.5143 & 0.99982768 & 0.99999827 \\
3198.5347 & 0.99987132 & 1.0000425  \\
3198.5756 & 0.99984388 & 1.0000161  \\
3198.5960 & 0.99978930 & 0.99996185 \\
3198.6164 & 0.99983803 & 1.0000109  \\
3198.6369 & 0.99985211 & 1.0000251  \\
3198.6573 & 0.99980981 & 0.99998296 \\
3198.6777 & 0.99980428 & 0.99997754 \\
3198.6982 & 0.99981378 & 0.99998711 \\
3198.7186 & 0.99976024 & 0.99993356 \\
3198.7595 & 0.99980702 & 0.99998011 \\
3198.7799 & 0.99982621 & 0.99999924 \\
3198.8003 & 0.99982428 & 0.99999720 \\
3198.8208 & 0.99981576 & 0.99998831 \\
3198.8412 & 0.99976790 & 0.99994015 \\
3198.8616 & 0.99977314 & 0.99994521 \\
3198.8821 & 0.99977135 & 0.99994295 \\
3198.9025 & 0.99984453 & 1.0000158  \\
3198.9229 & 0.99980794 & 0.99997877 \\
3198.9434 & 0.99981084 & 0.99998125 \\
3198.9638 & 0.99980700 & 0.99997705 \\
3198.9842 & 0.99981949 & 0.99998912 \\
3199.0046 & 0.99985722 & 1.0000263  \\
3199.0251 & 0.99978043 & 0.99994899 \\
3199.0455 & 0.99983995 & 1.0000080  \\
3199.0659 & 0.99980635 & 0.99997384 \\
3199.0864 & 0.99981131 & 0.99997832 \\
3199.1068 & 0.99982287 & 0.99998946 \\
3199.1272 & 0.99982311 & 0.99998928 \\
3199.1477 & 0.99985928 & 1.0000248  \\
3199.1681 & 0.99986173 & 1.0000268  \\
3199.1885 & 0.99981657 & 0.99998114 \\
3199.2090 & 0.99984855 & 1.0000127  \\
3199.2294 & 0.99985083 & 1.0000144  \\
3199.2498 & 0.99985812 & 1.0000214  \\
3199.2703 & 0.99984120 & 1.0000041  \\
3199.2907 & 0.99983574 & 0.99999828 \\
3199.3111 & 0.99983365 & 0.99999584 \\
3199.3520 & 0.99985263 & 1.0000140  \\
3199.3724 & 0.99981579 & 0.99997701 \\
3199.3928 & 0.99987746 & 1.0000385  \\
3199.4133 & 0.99983467 & 0.99999536 \\
3199.4337 & 0.99982635 & 0.99998680 \\
3199.4541 & 0.99989037 & 1.0000506  \\
3199.4746 & 0.99980903 & 0.99996912 \\
3199.4950 & 0.99982753 & 0.99998733 \\
3199.5154 & 0.99985194 & 1.0000115  \\
3199.5563 & 0.99986374 & 1.0000230  \\
3199.5767 & 0.99988084 & 1.0000399  \\
3199.5972 & 0.99988010 & 1.0000389  \\
3199.6176 & 0.99985683 & 1.0000156  \\
3199.6380 & 0.99980890 & 0.99996744 \\
3199.6585 & 0.99988010 & 1.0000386  \\
3199.6789 & 0.99983349 & 0.99999168 \\
3199.6993 & 0.99988521 & 1.0000431  \\
3199.7198 & 0.99989811 & 1.0000559  \\
3199.7402 & 0.99987943 & 1.0000370  \\
3199.7606 & 0.99985312 & 1.0000105  \\
3199.7810 & 0.99987846 & 1.0000357  \\
3199.8015 & 0.99983835 & 0.99999517 \\
3199.8219 & 0.99986308 & 1.0000197  \\
3199.8423 & 0.99984857 & 1.0000049  \\
3199.8628 & 0.99983972 & 0.99999582 \\
3199.8832 & 0.99980324 & 0.99995886 \\
3199.9036 & 0.99983620 & 0.99999159 \\
3199.9241 & 0.99983883 & 0.99999392 \\
3199.9445 & 0.99986568 & 1.0000204  \\
3199.9649 & 0.99986333 & 1.0000175  \\
3199.9854 & 0.99985054 & 1.0000042  \\
3200.0058 & 0.99983857 & 0.99999188 \\
3200.0467 & 0.99984756 & 0.99999979 \\
3200.0671 & 0.99983752 & 0.99998910 \\
3200.0875 & 0.99982979 & 0.99998089 \\
3200.1080 & 0.99987625 & 1.0000267  \\
3200.1284 & 0.99981581 & 0.99996565 \\
3200.1693 & 0.99982928 & 0.99997770 \\
3200.1897 & 0.99984346 & 0.99999086 \\
3200.2101 & 0.99983937 & 0.99998600 \\
3200.2305 & 0.99984288 & 0.99998867 \\
3200.2510 & 0.99983537 & 0.99998033 \\
3200.2714 & 0.99984994 & 0.99999383 \\
3200.2918 & 0.99983677 & 0.99997958 \\
3200.3123 & 0.99981128 & 0.99995314 \\
3200.3327 & 0.99985884 & 0.99999951 \\
3200.3531 & 0.99975217 & 0.99989169 \\
3200.3736 & 0.99979058 & 0.99992892 \\
3200.3940 & 0.99981623 & 0.99995326 \\
3200.4144 & 0.99983584 & 0.99997161 \\
3200.4349 & 0.99985385 & 0.99998819 \\
3200.4553 & 0.99985794 & 0.99999092 \\
3200.4757 & 0.99991452 & 1.0000461  \\
3200.4962 & 0.99995183 & 1.0000818  \\
3200.5370 & 0.99989485 & 1.0000214  \\
3200.5575 & 0.99987039 & 0.99999532 \\
3200.5779 & 0.99987317 & 0.99999619 \\
3200.5983 & 0.99990890 & 1.0000302  \\
3200.6187 & 0.99987685 & 0.99999635 \\
3200.6392 & 0.99993097 & 1.0000483  \\
3200.6596 & 0.99986437 & 0.99997971 \\
3200.6800 & 0.99987092 & 0.99998417 \\
3200.7005 & 0.99985783 & 0.99996887 \\
3200.7209 & 0.99991633 & 1.0000252  \\
3200.7413 & 0.99992821 & 1.0000347  \\
3200.7618 & 0.99990723 & 1.0000114  \\
3200.7822 & 0.99993052 & 1.0000322  \\
3200.8026 & 0.99995398 & 1.0000531  \\
3200.8231 & 0.99993136 & 1.0000278  \\
3200.8435 & 0.99990836 & 1.0000021  \\
3200.8639 & 0.99992698 & 1.0000181  \\
3200.8844 & 0.99989983 & 0.99998805 \\
3200.9048 & 0.99995942 & 1.0000448  \\
3200.9252 & 0.99994667 & 1.0000292  \\
3200.9457 & 0.99994718 & 1.0000268  \\
3200.9661 & 0.99992441 & 1.0000010  \\
3200.9865 & 0.99993626 & 1.0000099  \\
3201.0069 & 0.99988850 & 0.99995913 \\
3201.0274 & 0.99994821 & 1.0000157  \\
3201.0478 & 0.99989946 & 0.99996390 \\
3201.0682 & 0.99991737 & 0.99997871 \\
3201.0887 & 0.99990447 & 0.99996276 \\
3201.1091 & 0.99992230 & 0.99997731 \\
3201.1295 & 0.99994985 & 1.0000017  \\
3201.1500 & 0.99995378 & 1.0000026  \\
3201.1704 & 0.99996967 & 1.0000153  \\
3201.1908 & 0.99994801 & 0.99999063 \\
3201.2113 & 0.99992372 & 0.99996318 \\
3201.2317 & 0.99995832 & 0.99999474 \\
3201.2521 & 0.99995176 & 0.99998514 \\
3201.2726 & 0.99997765 & 1.0000079  \\
3201.2930 & 0.99997407 & 1.0000014  \\
3201.3134 & 1.0000140  & 1.0000382  \\
3201.3339 & 0.99998125 & 1.0000026  \\
3201.3543 & 0.99999260 & 1.0000111  \\
3201.3747 & 1.0000055  & 1.0000211  \\
3201.3951 & 0.99997133 & 0.99998408 \\
3201.4156 & 0.99996005 & 0.99997000 \\
3201.4360 & 0.99995246 & 0.99995985 \\
3201.4564 & 0.99999705 & 1.0000017  \\
3201.4769 & 1.0000145  & 1.0000167  \\
3201.5177 & 0.99997612 & 0.99997337 \\
3201.5382 & 1.0000267  & 1.0000217  \\
3201.5790 & 1.0000456  & 1.0000361  \\
3201.6403 & 1.0000186  & 1.0000032  \\
3201.6608 & 0.99993627 & 0.99991898 \\
3201.6812 & 0.99994600 & 0.99992705 \\
3201.7016 & 0.99994315 & 0.99992241 \\
3201.7221 & 0.99993831 & 0.99991602 \\
3201.8038 & 1.0000952  & 1.0000673  \\
3201.8242 & 1.0000489  & 1.0000197  \\
3201.8446 & 1.0001170  & 1.0000870  \\
3201.8651 & 1.0000946  & 1.0000633  \\
3201.8855 & 1.0000607  & 1.0000286  \\
3201.9059 & 1.0000851  & 1.0000521  \\
3201.9468 & 1.0000702  & 1.0000358  \\
3201.9672 & 1.0000678  & 1.0000327  \\
3201.9877 & 1.0000236  & 0.99998785 \\
3202.0081 & 1.0000004  & 0.99996429 \\
3202.0285 & 1.0000569  & 1.0000205  \\
3202.0490 & 1.0000546  & 1.0000178  \\
3202.0694 & 1.0000414  & 1.0000043  \\
3202.1103 & 1.0000422  & 1.0000050  \\
3202.1307 & 1.0000215  & 0.99998416 \\
3202.1511 & 1.0000214  & 0.99998410 \\
3202.1716 & 1.0000374  & 1.0000003  \\
3202.1920 & 1.0000787  & 1.0000420  \\
3202.2124 & 1.0000200  & 0.99998356 \\
3202.2328 & 1.0000245  & 0.99998839 \\
3202.2533 & 1.0000257  & 0.99999006 \\
3202.2737 & 1.0000220  & 0.99998692 \\
3202.2941 & 1.0000441  & 1.0000098  \\
3202.3146 & 1.0000749  & 1.0000413  \\
3202.3350 & 1.0000535  & 1.0000205  \\
3202.3554 & 1.0000465  & 1.0000143  \\
3202.3759 & 1.0000258  & 0.99999460 \\
3202.3963 & 0.99999992 & 0.99996977 \\
3202.4167 & 1.0000296  & 1.0000004  \\
3202.4372 & 1.0000229  & 0.99999481 \\
3202.4576 & 1.0000374  & 1.0000104  \\
3202.4780 & 1.0000421  & 1.0000163  \\
3202.4985 & 1.0000398  & 1.0000151  \\
3202.5189 & 1.0000362  & 1.0000128  \\
3202.5393 & 0.99998532 & 0.99996326 \\
3202.5598 & 0.99996310 & 0.99994224 \\
3202.5802 & 0.99998857 & 0.99996914 \\
3202.6006 & 1.0000448  & 1.0000267  \\
3202.6210 & 0.99997250 & 0.99995581 \\
3202.6415 & 0.99998484 & 0.99996946 \\
3202.6619 & 0.99995717 & 0.99994310 \\
3202.6823 & 0.99998954 & 0.99997703 \\
3202.7232 & 1.0000140  & 1.0000040  \\
3202.7436 & 1.0000091  & 1.0000007  \\
3202.7845 & 1.0000223  & 1.0000165  \\
3202.8049 & 0.99998882 & 0.99998429 \\
3202.8254 & 0.99999927 & 0.99999606 \\
3202.8458 & 1.0000109  & 1.0000089  \\
3202.8662 & 1.0000192  & 1.0000185  \\
3202.8867 & 0.99999414 & 0.99999461 \\
3202.9071 & 1.0000000  & 1.0000016  \\
3202.9275 & 0.99996809 & 0.99997083 \\
3202.9480 & 1.0000311  & 1.0000350  \\
3202.9888 & 0.99999408 & 0.99999992 \\
3203.0093 & 1.0000195  & 1.0000262  \\
3203.0297 & 0.99994372 & 0.99995128 \\
3203.0501 & 0.99998529 & 0.99999363 \\
3203.0705 & 0.99994465 & 0.99995371 \\
3203.0910 & 0.99997048 & 0.99998008 \\
3203.1114 & 0.99996588 & 0.99997619 \\
3203.1318 & 0.99998882 & 0.99999967 \\
3203.1523 & 1.0000077  & 1.0000189  \\
3203.1727 & 1.0000134  & 1.0000250  \\
3203.1931 & 1.0000215  & 1.0000337  \\
3203.2136 & 0.99998834 & 1.0000007  \\
3203.2340 & 0.99999169 & 1.0000047  \\
3203.2544 & 0.99998937 & 1.0000026  \\
3203.2749 & 1.0000272  & 1.0000408  \\
3203.2953 & 1.0000111  & 1.0000250  \\
3203.3157 & 0.99998841 & 1.0000024  \\
3203.3362 & 0.99999186 & 1.0000061  \\
3203.3566 & 1.0000099  & 1.0000244  \\
3203.3770 & 1.0000465  & 1.0000613  \\
3203.3975 & 1.0000042  & 1.0000191  \\
3203.4179 & 0.99996742 & 0.99998268 \\
3203.4383 & 0.99999502 & 1.0000105  \\
3203.4792 & 1.0000162  & 1.0000322  \\
3203.4996 & 1.0000011  & 1.0000175  \\
3203.5200 & 0.99998459 & 1.0000013  \\
3203.5405 & 1.0000085  & 1.0000256  \\
3203.5609 & 0.99998126 & 0.99999884 \\
3203.5813 & 1.0000349  & 1.0000529  \\
3203.6018 & 0.99992963 & 0.99994811 \\
3203.6222 & 0.99993508 & 0.99995409 \\
3203.6426 & 0.99993791 & 0.99995752 \\
3203.6631 & 0.99998373 & 1.0000040  \\
3203.6835 & 0.99996347 & 0.99998445 \\
3203.7039 & 1.0000426  & 1.0000643  \\
3203.7244 & 0.99999741 & 1.0000201  \\
3203.7448 & 0.99997382 & 0.99999731 \\
3203.7652 & 0.99996790 & 0.99999234 \\
3203.7857 & 0.99994177 & 0.99996728 \\
3203.8061 & 0.99998910 & 1.0000159  \\
3203.8265 & 0.99992695 & 0.99995490 \\
3203.8469 & 0.99996761 & 0.99999675 \\
3203.8674 & 0.99996573 & 0.99999625 \\
3203.8878 & 0.99988723 & 0.99991924 \\
3203.9082 & 0.99999377 & 1.0000272  \\
3203.9287 & 0.99999324 & 1.0000282  \\
3203.9491 & 0.99992446 & 0.99996117 \\
3203.9695 & 0.99992673 & 0.99996512 \\
3203.9900 & 0.99992645 & 0.99996651 \\
3204.0104 & 0.99994302 & 0.99998492 \\
3204.0308 & 0.99993462 & 0.99997819 \\
3204.0513 & 0.99994375 & 0.99998923 \\
3204.0717 & 0.99998934 & 1.0000365  \\
3204.0921 & 0.99997727 & 1.0000264  \\
3204.1126 & 0.99993276 & 0.99998372 \\
3204.1330 & 0.99999153 & 1.0000445  \\
3204.1534 & 0.99996243 & 1.0000172  \\
3204.1739 & 0.99993728 & 0.99999396 \\
3204.1943 & 0.99994483 & 1.0000034  \\
3204.2147 & 0.99992130 & 0.99998180 \\
3204.2351 & 0.99991371 & 0.99997635 \\
3204.2760 & 0.99992971 & 0.99999593 \\
3204.2964 & 0.99997916 & 1.0000472  \\
3204.3169 & 0.99992885 & 0.99999883 \\
3204.3373 & 0.99992030 & 0.99999201 \\
3204.3577 & 0.99989779 & 0.99997128 \\
3204.3782 & 0.99992822 & 1.0000034  \\
3204.3986 & 0.99988801 & 0.99996490 \\
3204.4190 & 0.99995201 & 1.0000305  \\
3204.4395 & 0.99993380 & 1.0000139  \\
3204.4599 & 0.99990825 & 0.99998996 \\
3204.4803 & 0.99990232 & 0.99998541 \\
3204.5008 & 0.99993871 & 1.0000232  \\
3204.5212 & 0.99996710 & 1.0000529  \\
3204.5416 & 0.99992865 & 1.0000157  \\
3204.5621 & 0.99990520 & 0.99999353 \\
3204.5825 & 0.99997340 & 1.0000628  \\
3204.6029 & 0.99993916 & 1.0000296  \\
3204.6233 & 0.99987517 & 0.99996660 \\
3204.6438 & 0.99988657 & 0.99997896 \\
3204.6642 & 0.99989816 & 0.99999145 \\
3204.6846 & 0.99992102 & 1.0000150  \\
3204.7051 & 0.99988113 & 0.99997602 \\
3204.7255 & 0.99991747 & 1.0000131  \\
3204.7459 & 0.99992544 & 1.0000218  \\
3204.7664 & 0.99987486 & 0.99997196 \\
3204.7868 & 0.99989102 & 0.99998871 \\
3204.8072 & 0.99992529 & 1.0000236  \\
3204.8277 & 0.99982750 & 0.99992644 \\
3204.8481 & 0.99990703 & 1.0000067  \\
3204.8685 & 0.99987785 & 0.99997810 \\
3204.8890 & 0.99990676 & 1.0000076  \\
3204.9094 & 0.99990305 & 1.0000046  \\
3204.9503 & 0.99991743 & 1.0000201  \\
3204.9707 & 0.99990075 & 1.0000042  \\
3204.9911 & 0.99987463 & 0.99997864 \\
3205.0116 & 0.99989537 & 1.0000003  \\
3205.0320 & 0.99988571 & 0.99999138 \\
3205.0524 & 0.99984575 & 0.99995214 \\
3205.0728 & 0.99991781 & 1.0000250  \\
3205.0933 & 0.99985829 & 0.99996641 \\
3205.1137 & 0.99995273 & 1.0000618  \\
3205.1341 & 0.99995957 & 1.0000697  \\
3205.1546 & 0.99988863 & 0.99999986 \\
3205.1750 & 0.99990245 & 1.0000148  \\
3205.1954 & 0.99986691 & 0.99998051 \\
3205.2159 & 0.99985071 & 0.99996538 \\
3205.2363 & 0.99984510 & 0.99996114 \\
3205.2567 & 0.99988886 & 1.0000065  \\
3205.2772 & 0.99989459 & 1.0000137  \\
3205.2976 & 0.99985621 & 0.99997702 \\
3205.3180 & 0.99983256 & 0.99995510 \\
3205.3385 & 0.99990705 & 1.0000313  \\
3205.3589 & 0.99991409 & 1.0000403  \\
3205.3793 & 0.99987471 & 1.0000029  \\
3205.3998 & 0.99989542 & 1.0000256  \\
3205.4406 & 0.99985130 & 0.99998582 \\
3205.4815 & 0.99983970 & 0.99997863 \\
3205.5019 & 0.99984845 & 0.99998977 \\
3205.5223 & 0.99983070 & 0.99997434 \\
3205.5428 & 0.99986185 & 1.0000079  \\
3205.5632 & 0.99987737 & 1.0000258  \\
3205.5836 & 0.99986641 & 1.0000174  \\
3205.6041 & 0.99984358 & 0.99999677 \\
3205.6245 & 0.99979681 & 0.99995267 \\
3205.6449 & 0.99984112 & 0.99999937 \\
3205.6654 & 0.99981921 & 0.99997978 \\
3205.6858 & 0.99984820 & 1.0000112  \\
3205.7062 & 0.99989843 & 1.0000637  \\
3205.7267 & 0.99983345 & 1.0000012  \\
3205.7471 & 0.99988020 & 1.0000502  \\
3205.7675 & 0.99980048 & 0.99997286 \\
3205.7880 & 0.99983250 & 1.0000070  \\
3205.8084 & 0.99983444 & 1.0000111  \\
3205.8288 & 0.99979974 & 0.99997867 \\
3205.8492 & 0.99982497 & 1.0000059  \\
3205.8697 & 0.99980031 & 0.99998306 \\
3205.8901 & 0.99984263 & 1.0000275  \\
3205.9105 & 0.99979186 & 0.99997847 \\
3205.9310 & 0.99982132 & 1.0000098  \\
3205.9514 & 0.99986720 & 1.0000572  \\
3205.9718 & 0.99980773 & 0.99999918 \\
3205.9923 & 0.99979469 & 0.99998762 \\
3206.0127 & 0.99979086 & 0.99998505 \\
3206.0331 & 0.99980528 & 1.0000007  \\
3206.0536 & 0.99976492 & 0.99996143 \\
3206.0740 & 0.99975425 & 0.99995171 \\
3206.0944 & 0.99981758 & 1.0000158  \\
3206.1149 & 0.99982292 & 1.0000219  \\
3206.1353 & 0.99977156 & 0.99997099 \\
3206.1557 & 0.99977071 & 0.99997085 \\
3206.1762 & 0.99979651 & 0.99999702 \\
3206.1966 & 0.99976496 & 0.99996589 \\
3206.2170 & 0.99979073 & 0.99999195 \\
3206.2374 & 0.99980922 & 1.0000107  \\
3206.2579 & 0.99979423 & 0.99999599 \\
3206.2783 & 0.99978086 & 0.99998273 \\
3206.2987 & 0.99980716 & 1.0000092  \\
3206.3192 & 0.99977167 & 0.99997378 \\
3206.3396 & 0.99981519 & 1.0000175  \\
3206.3600 & 0.99983043 & 1.0000329  \\
3206.3805 & 0.99977282 & 0.99997541 \\
3206.4009 & 0.99981133 & 1.0000141  \\
3206.4213 & 0.99983703 & 1.0000399  \\
3206.4418 & 0.99983328 & 1.0000364  \\
3206.4622 & 0.99984226 & 1.0000456  \\
3206.4826 & 0.99978962 & 0.99999316 \\
3206.5031 & 0.99982757 & 1.0000315  \\
3206.5235 & 0.99983796 & 1.0000422  \\
3206.5439 & 0.99978828 & 0.99999314 \\
3206.5644 & 0.99974873 & 0.99995418 \\
3206.5848 & 0.99977931 & 0.99998554 \\
3206.6052 & 0.99977586 & 0.99998257 \\
3206.6257 & 0.99976347 & 0.99997113 \\
3206.6461 & 0.99977530 & 0.99998409 \\
3206.6665 & 0.99978678 & 0.99999658 \\
3206.6869 & 0.99979792 & 1.0000090  \\
3206.7074 & 0.99976162 & 0.99997422 \\
3206.7278 & 0.99981574 & 1.0000298  \\
3206.7482 & 0.99981006 & 1.0000259  \\
3206.7687 & 0.99977424 & 0.99999191 \\
3206.7891 & 0.99981565 & 1.0000356  \\
3206.8095 & 0.99984938 & 1.0000716  \\
3206.8300 & 0.99977146 & 0.99999599 \\
3206.8504 & 0.99975226 & 0.99997947 \\
3206.8708 & 0.99970516 & 0.99993522 \\
3206.8913 & 0.99978324 & 1.0000163  \\
3206.9117 & 0.99980499 & 1.0000411  \\
3206.9321 & 0.99977098 & 1.0000104  \\
3206.9526 & 0.99970322 & 0.99994622 \\
3206.9730 & 0.99970046 & 0.99994709 \\
3206.9934 & 0.99974673 & 0.99999701 \\
3207.0139 & 0.99975439 & 1.0000087  \\
3207.0343 & 0.99976464 & 1.0000227  \\
3207.0547 & 0.99972073 & 0.99998298 \\
3207.0751 & 0.99972017 & 0.99998677 \\
3207.0956 & 0.99968606 & 0.99995695 \\
3207.1569 & 0.99969561 & 0.99998033 \\
3207.1773 & 0.99973762 & 1.0000270  \\
3207.1977 & 0.99972538 & 1.0000196  \\
3207.2182 & 0.99970159 & 1.0000008  \\
3207.2386 & 0.99965499 & 0.99995908 \\
3207.2590 & 0.99970662 & 1.0000158  \\
3207.2795 & 0.99973200 & 1.0000462  \\
3207.2999 & 0.99967093 & 0.99999047 \\
3207.3203 & 0.99973884 & 1.0000635  \\
3207.3408 & 0.99969756 & 1.0000274  \\
3207.3612 & 0.99968976 & 1.0000249  \\
3207.4021 & 0.99964874 & 0.99999438 \\
3207.4225 & 0.99966153 & 1.0000125  \\
3207.4633 & 0.99957182 & 0.99993360 \\
3207.4838 & 0.99959096 & 0.99995805 \\
3207.5042 & 0.99959596 & 0.99996835 \\
3207.5246 & 0.99959808 & 0.99997585 \\
3207.5451 & 0.99960922 & 0.99999212 \\
3207.5655 & 0.99958131 & 0.99996951 \\
3207.5859 & 0.99960912 & 1.0000027  \\
3207.6064 & 0.99959846 & 0.99999716 \\
3207.6268 & 0.99957948 & 0.99998359 \\
3207.6472 & 0.99957567 & 0.99998479 \\
3207.6677 & 0.99956982 & 0.99998401 \\
3207.6881 & 0.99963214 & 1.0000515  \\
3207.7085 & 0.99961063 & 1.0000351  \\
3207.7290 & 0.99955883 & 0.99998822 \\
3207.7494 & 0.99956619 & 1.0000005  \\
3207.7698 & 0.99960345 & 1.0000426  \\
3207.7903 & 0.99955244 & 0.99999644 \\
3207.8107 & 0.99957109 & 1.0000198  \\
3207.8311 & 0.99951983 & 0.99997329 \\
3207.8515 & 0.99956876 & 1.0000268  \\
3207.8720 & 0.99951712 & 0.99997982 \\
3207.8924 & 0.99954745 & 1.0000146  \\
3207.9128 & 0.99950144 & 0.99997302 \\
3207.9333 & 0.99956602 & 1.0000420  \\
3207.9537 & 0.99949851 & 0.99997873 \\
3207.9741 & 0.99956573 & 1.0000501  \\
3207.9946 & 0.99946813 & 0.99995663 \\
3208.0150 & 0.99952737 & 1.0000200  \\
3208.0559 & 0.99950200 & 1.0000023  \\
3208.0763 & 0.99950775 & 1.0000118  \\
3208.0967 & 0.99952338 & 1.0000311  \\
3208.1172 & 0.99947314 & 0.99998418 \\
3208.1376 & 0.99944871 & 0.99996320 \\
3208.1580 & 0.99949984 & 1.0000178  \\
3208.1785 & 0.99949551 & 1.0000165  \\
3208.1989 & 0.99950796 & 1.0000322  \\
3208.2193 & 0.99944891 & 0.99997598 \\
3208.2397 & 0.99948383 & 1.0000137  \\
3208.2602 & 0.99946248 & 0.99999523 \\
3208.2806 & 0.99948365 & 1.0000190  \\
3208.3010 & 0.99947899 & 1.0000167  \\
3208.3215 & 0.99948028 & 1.0000204  \\
3208.3419 & 0.99945420 & 0.99999648 \\
3208.3623 & 0.99944665 & 0.99999090 \\
3208.3828 & 0.99948169 & 1.0000280  \\
3208.4032 & 0.99943953 & 0.99998765 \\
3208.4236 & 0.99947128 & 1.0000213  \\
3208.4441 & 0.99944927 & 1.0000008  \\
3208.4645 & 0.99942913 & 0.99998207 \\
3208.4849 & 0.99944788 & 1.0000024  \\
3208.5054 & 0.99942969 & 0.99998555 \\
3208.5258 & 0.99945128 & 1.0000085  \\
3208.5462 & 0.99940037 & 0.99995872 \\
3208.5667 & 0.99941652 & 0.99997601 \\
3208.5871 & 0.99942744 & 0.99998790 \\
3208.6075 & 0.99944549 & 1.0000070  \\
3208.6280 & 0.99943259 & 0.99999508 \\
3208.6484 & 0.99936680 & 0.99993003 \\
3208.6688 & 0.99939823 & 0.99996219 \\
3208.6892 & 0.99942068 & 0.99998543 \\
3208.7097 & 0.99942915 & 0.99999462 \\
3208.7301 & 0.99940572 & 0.99997195 \\
3208.7505 & 0.99944143 & 1.0000082  \\
3208.7710 & 0.99942314 & 0.99999045 \\
3208.7914 & 0.99943135 & 0.99999920 \\
3208.8118 & 0.99946225 & 1.0000306  \\
3208.8323 & 0.99937635 & 0.99994519 \\
3208.8731 & 0.99944200 & 1.0000119  \\
3208.8936 & 0.99941886 & 0.99998939 \\
3208.9140 & 0.99945934 & 1.0000302  \\
3208.9344 & 0.99942708 & 0.99999857 \\
3208.9549 & 0.99942873 & 1.0000006  \\
3208.9753 & 0.99943628 & 1.0000087  \\
3208.9957 & 0.99945715 & 1.0000300  \\
3209.0162 & 0.99947984 & 1.0000533  \\
3209.0366 & 0.99946227 & 1.0000364  \\
3209.0570 & 0.99944298 & 1.0000176  \\
3209.0774 & 0.99942187 & 0.99999723 \\
3209.0979 & 0.99945287 & 1.0000289  \\
3209.1183 & 0.99944397 & 1.0000207  \\
3209.1387 & 0.99937953 & 0.99995708 \\
3209.1592 & 0.99942404 & 1.0000021  \\
3209.1796 & 0.99941032 & 0.99998925 \\
3209.2000 & 0.99941385 & 0.99999362 \\
3209.2205 & 0.99938422 & 0.99996474 \\
3209.2409 & 0.99942500 & 1.0000064  \\
3209.2613 & 0.99941538 & 0.99999766 \\
3209.2818 & 0.99941410 & 0.99999721 \\
3209.3022 & 0.99944110 & 1.0000251  \\
3209.3226 & 0.99942258 & 1.0000075  \\
3209.3635 & 0.99943881 & 1.0000255  \\
3209.3839 & 0.99952632 & 1.0001140  \\
3209.4044 & 0.99945018 & 1.0000386  \\
3209.4248 & 0.99937661 & 0.99996596 \\
3209.4452 & 0.99939335 & 0.99998361 \\
3209.4656 & 0.99941615 & 1.0000073  \\
3209.4861 & 0.99937432 & 0.99996629 \\
3209.5065 & 0.99934062 & 0.99993341 \\
3209.5269 & 0.99937746 & 0.99997117 \\
3209.5474 & 0.99935554 & 0.99995007 \\
3209.5678 & 0.99946017 & 1.0000555  \\
3209.5882 & 0.99938470 & 0.99998091 \\
3209.6087 & 0.99937771 & 0.99997464 \\
3209.6291 & 0.99939531 & 0.99999291 \\
3209.6495 & 0.99944810 & 1.0000465  \\
3209.6700 & 0.99936997 & 0.99996910 \\
3209.6904 & 0.99943706 & 1.0000369  \\
3209.7108 & 0.99936223 & 0.99996267 \\
3209.7313 & 0.99940499 & 1.0000062  \\
3209.7517 & 0.99937023 & 0.99997187 \\
3209.7721 & 0.99935238 & 0.99995460 \\
3209.7926 & 0.99939363 & 0.99999641 \\
3209.8130 & 0.99940354 & 1.0000067  \\
3209.8538 & 0.99938898 & 0.99999300 \\
3209.8743 & 0.99940633 & 1.0000105  \\
3209.8947 & 0.99940809 & 1.0000127  \\
3209.9356 & 0.99942375 & 1.0000289  \\
3209.9560 & 0.99935556 & 0.99996100 \\
3209.9764 & 0.99935367 & 0.99995940 \\
3209.9969 & 0.99936900 & 0.99997486 \\
3210.0173 & 0.99939825 & 1.0000044  \\
3210.0377 & 0.99940788 & 1.0000144  \\
3210.0582 & 0.99938920 & 0.99999585 \\
3210.0786 & 0.99940055 & 1.0000074  \\
3210.0990 & 0.99941283 & 1.0000200  \\
3210.1195 & 0.99940122 & 1.0000087  \\
3210.1399 & 0.99941104 & 1.0000188  \\
3210.1603 & 0.99942502 & 1.0000331  \\
3210.1808 & 0.99940664 & 1.0000151  \\
3210.2012 & 0.99942483 & 1.0000337  \\
3210.2216 & 0.99940660 & 1.0000159  \\
3210.2420 & 0.99944675 & 1.0000566  \\
3210.2625 & 0.99936901 & 0.99997929 \\
3210.2829 & 0.99939599 & 1.0000068  \\
3210.3033 & 0.99937361 & 0.99998508 \\
3210.3238 & 0.99939754 & 1.0000096  \\
3210.3442 & 0.99941079 & 1.0000237  \\
3210.3646 & 0.99942648 & 1.0000403  \\
3210.3851 & 0.99940153 & 1.0000161  \\
3210.4055 & 0.99940188 & 1.0000175  \\
3210.4259 & 0.99937775 & 0.99999436 \\
3210.4464 & 0.99935022 & 0.99996794 \\
3210.4668 & 0.99933150 & 0.99995052 \\
3210.4872 & 0.99935306 & 0.99997335 \\
3210.5077 & 0.99933723 & 0.99995888 \\
3210.5281 & 0.99938288 & 1.0000062  \\
3210.5485 & 0.99930922 & 0.99993407 \\
3210.5894 & 0.99936727 & 0.99999580 \\
3210.6098 & 0.99936962 & 1.0000000  \\
3210.6302 & 0.99938446 & 1.0000168  \\
3210.6507 & 0.99933923 & 0.99997370 \\
3210.6711 & 0.99940737 & 1.0000442  \\
3210.6915 & 0.99939256 & 1.0000316  \\
3210.7120 & 0.99939435 & 1.0000357  \\
3210.7324 & 0.99935088 & 0.99999460 \\
3210.7528 & 0.99940509 & 1.0000514  \\
3210.7733 & 0.99932873 & 0.99997751 \\
3210.7937 & 0.99933489 & 0.99998612 \\
3210.8346 & 0.99931496 & 0.99997148 \\
3210.8550 & 0.99927462 & 0.99993362 \\
3210.8754 & 0.99932253 & 0.99998426 \\
3210.8959 & 0.99932634 & 0.99999063 \\
3210.9163 & 0.99932716 & 0.99999401 \\
3210.9367 & 0.99936743 & 1.0000370  \\
3210.9572 & 0.99933371 & 1.0000058  \\
3210.9776 & 0.99927646 & 0.99995109 \\
3210.9980 & 0.99930840 & 0.99998568 \\
3211.0185 & 0.99934756 & 1.0000273  \\
3211.0389 & 0.99936323 & 1.0000456  \\
3211.0593 & 0.99932084 & 1.0000054  \\
3211.0797 & 0.99932941 & 1.0000164  \\
3211.1002 & 0.99932023 & 1.0000096  \\
3211.1206 & 0.99929769 & 0.99998921 \\
3211.1410 & 0.99934686 & 1.0000404  \\
3211.1615 & 0.99927139 & 0.99996713 \\
3211.1819 & 0.99930984 & 1.0000075  \\
3211.2023 & 0.99927286 & 0.99997236 \\
3211.2228 & 0.99926997 & 0.99997120 \\
3211.2432 & 0.99928005 & 0.99998296 \\
3211.2636 & 0.99927801 & 0.99998258 \\
3211.2841 & 0.99930322 & 1.0000090  \\
3211.3454 & 0.99924051 & 0.99994971 \\
3211.3658 & 0.99930029 & 1.0000104  \\
3211.3862 & 0.99929368 & 1.0000045  \\
3211.4067 & 0.99930118 & 1.0000127  \\
3211.4271 & 0.99928993 & 1.0000019  \\
3211.4475 & 0.99929310 & 1.0000055  \\
3211.4679 & 0.99928504 & 0.99999791 \\
3211.4884 & 0.99930949 & 1.0000226  \\
3211.5088 & 0.99932667 & 1.0000401  \\
3211.5292 & 0.99929309 & 1.0000067  \\
3211.5497 & 0.99931096 & 1.0000247  \\
3211.5701 & 0.99923729 & 0.99995108 \\
3211.5905 & 0.99933975 & 1.0000537  \\
3211.6110 & 0.99931070 & 1.0000247  \\
3211.6314 & 0.99930834 & 1.0000223  \\
3211.6518 & 0.99932719 & 1.0000413  \\
3211.6723 & 0.99931512 & 1.0000294  \\
3211.6927 & 0.99925212 & 0.99996646 \\
3211.7131 & 0.99929989 & 1.0000144  \\
3211.7336 & 0.99930120 & 1.0000161  \\
3211.7540 & 0.99924422 & 0.99995939 \\
3211.7744 & 0.99923740 & 0.99995280 \\
3211.8153 & 0.99928469 & 1.0000010  \\
3211.8357 & 0.99927241 & 0.99998926 \\
3211.8561 & 0.99927290 & 0.99999042 \\
3211.8766 & 0.99928298 & 1.0000013  \\
3211.8970 & 0.99925688 & 0.99997611 \\
3211.9174 & 0.99926062 & 0.99998087 \\
3211.9379 & 0.99927353 & 0.99999492 \\
3211.9583 & 0.99930241 & 1.0000251  \\
3211.9787 & 0.99922783 & 0.99995212 \\
3211.9992 & 0.99931716 & 1.0000432  \\
3212.0196 & 0.99926486 & 0.99999257 \\
3212.0605 & 0.99921019 & 0.99994209 \\
3212.0809 & 0.99925054 & 0.99998510 \\
3212.1013 & 0.99925490 & 0.99999203 \\
3212.1218 & 0.99924734 & 0.99998726 \\
3212.1422 & 0.99925781 & 1.0000007  \\
3212.1626 & 0.99925087 & 0.99999706 \\
3212.1831 & 0.99923648 & 0.99998600 \\
3212.2035 & 0.99925800 & 1.0000111  \\
3212.2239 & 0.99921695 & 0.99997355 \\
3212.2443 & 0.99925227 & 1.0000127  \\
3212.2648 & 0.99925398 & 1.0000184  \\
3212.2852 & 0.99926215 & 1.0000305  \\
3212.3056 & 0.99922866 & 1.0000010  \\
3212.3261 & 0.99924101 & 1.0000178  \\
3212.3465 & 0.99919353 & 0.99997451 \\
3212.3669 & 0.99926147 & 1.0000470  \\
3212.3874 & 0.99926010 & 1.0000500  \\
3212.4078 & 0.99923001 & 1.0000243  \\
3212.4282 & 0.99925412 & 1.0000532  \\
3212.4487 & 0.99921874 & 1.0000225  \\
3212.4691 & 0.99924606 & 1.0000544  \\
3212.4895 & 0.99927572 & 1.0000888  \\
3212.5100 & 0.99917685 & 0.99999450 \\
3212.5508 & 0.99910415 & 0.99993129 \\
3212.5713 & 0.99915271 & 0.99998460 \\
3212.5917 & 0.99917302 & 1.0000096  \\
3212.6121 & 0.99913778 & 0.99997903 \\
3212.6325 & 0.99911890 & 0.99996466 \\
3212.6530 & 0.99912941 & 0.99997989 \\
3212.6734 & 0.99916748 & 1.0000225  \\
3212.6938 & 0.99901871 & 0.99987810 \\
3212.7143 & 0.99908354 & 0.99994728 \\
3212.7347 & 0.99907052 & 0.99993854 \\
3212.7551 & 0.99913748 & 1.0000099  \\
3212.7960 & 0.99904221 & 0.99992250 \\
3212.8164 & 0.99911966 & 1.0000040  \\
3212.8369 & 0.99911153 & 0.99999958 \\
3212.8573 & 0.99913667 & 1.0000283  \\
3212.8777 & 0.99904135 & 0.99993644 \\
3212.8982 & 0.99908057 & 0.99997903 \\
3212.9186 & 0.99910504 & 1.0000068  \\
3212.9390 & 0.99905620 & 0.99996108 \\
3212.9799 & 0.99905939 & 0.99997030 \\
3213.0003 & 0.99908192 & 0.99999583 \\
3213.0412 & 0.99918358 & 1.0001029  \\
3213.0616 & 0.99917387 & 1.0000958  \\
3213.0820 & 0.99916769 & 1.0000921  \\
3213.1025 & 0.99912545 & 1.0000523  \\
3213.1229 & 0.99908531 & 1.0000143  \\
3213.1433 & 0.99910354 & 1.0000349  \\
3213.1638 & 0.99907630 & 1.0000099  \\
3213.1842 & 0.99903599 & 0.99997152 \\
3213.2046 & 0.99907001 & 1.0000078  \\
3213.2251 & 0.99904386 & 0.99998357 \\
3213.2455 & 0.99901625 & 0.99995791 \\
3213.3068 & 0.99905998 & 1.0000072  \\
3213.3272 & 0.99907335 & 1.0000224  \\
3213.3477 & 0.99909730 & 1.0000482  \\
3213.3681 & 0.99907218 & 1.0000247  \\
3213.3885 & 0.99905103 & 1.0000052  \\
3213.4090 & 0.99900897 & 0.99996481 \\
3213.4294 & 0.99903269 & 0.99999011 \\
3213.4498 & 0.99899721 & 0.99995627 \\
3213.4702 & 0.99901460 & 0.99997529 \\
3213.4907 & 0.99902072 & 0.99998296 \\
3213.5315 & 0.99902630 & 0.99999176 \\
3213.5520 & 0.99903513 & 1.0000022  \\
3213.5724 & 0.99907318 & 1.0000419  \\
3213.5928 & 0.99903359 & 1.0000038  \\
3213.6133 & 0.99903981 & 1.0000116  \\
3213.6337 & 0.99904160 & 1.0000151  \\
3213.6541 & 0.99905207 & 1.0000272  \\
3213.6746 & 0.99897566 & 0.99995242 \\
3213.6950 & 0.99899365 & 0.99997209 \\
3213.7154 & 0.99909157 & 1.0000719  \\
3213.7359 & 0.99905157 & 1.0000334  \\
3213.7767 & 0.99900474 & 0.99999012 \\
3213.7972 & 0.99897866 & 0.99996580 \\
3213.8176 & 0.99900118 & 0.99999025 \\
3213.8380 & 0.99900506 & 0.99999599 \\
3213.8584 & 0.99901963 & 1.0000125  \\
3213.8789 & 0.99901648 & 1.0000112  \\
3213.8993 & 0.99898554 & 0.99998217 \\
3213.9197 & 0.99893934 & 0.99993807 \\
3213.9402 & 0.99899991 & 1.0000009  \\
3213.9606 & 0.99892808 & 0.99993092 \\
3213.9810 & 0.99895143 & 0.99995650 \\
3214.0219 & 0.99892633 & 0.99993609 \\
3214.0423 & 0.99899105 & 1.0000031  \\
3214.0628 & 0.99897602 & 0.99999048 \\
3214.0832 & 0.99899501 & 1.0000119  \\
3214.1036 & 0.99901960 & 1.0000391  \\
3214.1241 & 0.99896052 & 0.99998260 \\
3214.1445 & 0.99895728 & 0.99998204 \\
3214.1649 & 0.99900214 & 1.0000297  \\
3214.1854 & 0.99899695 & 1.0000274  \\
3214.2058 & 0.99897256 & 1.0000058  \\
3214.2262 & 0.99895683 & 0.99999317 \\
3214.2466 & 0.99896147 & 1.0000007  \\
3214.2671 & 0.99897086 & 1.0000132  \\
3214.2875 & 0.99899244 & 1.0000382  \\
3214.3079 & 0.99897319 & 1.0000221  \\
3214.3284 & 0.99895248 & 1.0000049  \\
3214.3488 & 0.99892777 & 0.99998365 \\
3214.3692 & 0.99896772 & 1.0000272  \\
3214.3897 & 0.99894196 & 1.0000051  \\
3214.4101 & 0.99887422 & 0.99994096 \\
3214.4305 & 0.99896826 & 1.0000389  \\
3214.4510 & 0.99890027 & 0.99997449 \\
3214.4714 & 0.99893503 & 1.0000133  \\
3214.5123 & 0.99897533 & 1.0000612  \\
3214.5327 & 0.99889651 & 0.99998619 \\
3214.5531 & 0.99889375 & 0.99998736 \\
3214.5736 & 0.99892174 & 1.0000191  \\
3214.5940 & 0.99890561 & 1.0000068  \\
3214.6144 & 0.99889295 & 0.99999784 \\
3214.6348 & 0.99879175 & 0.99990016 \\
3214.6553 & 0.99886460 & 0.99997680 \\
3214.6757 & 0.99887684 & 0.99999263 \\
3214.6961 & 0.99886128 & 0.99998075 \\
3214.7166 & 0.99886642 & 0.99998918 \\
3214.7574 & 0.99887305 & 1.0000024  \\
3214.7779 & 0.99886777 & 1.0000001  \\
3214.7983 & 0.99885671 & 0.99999205 \\
3214.8187 & 0.99888612 & 1.0000245  \\
3214.8392 & 0.99894299 & 1.0000841  \\
3214.8596 & 0.99882956 & 0.99997322 \\
3214.8800 & 0.99888697 & 1.0000329  \\
3214.9005 & 0.99887058 & 1.0000187  \\
3214.9209 & 0.99889936 & 1.0000497  \\
3214.9413 & 0.99884237 & 0.99999435 \\
3214.9618 & 0.99887537 & 1.0000291  \\
3214.9822 & 0.99883538 & 0.99999045 \\
3215.0026 & 0.99885415 & 1.0000105  \\
3215.0230 & 0.99885988 & 1.0000173  \\
3215.0435 & 0.99890799 & 1.0000662  \\
3215.0639 & 0.99887918 & 1.0000378  \\
3215.0843 & 0.99883526 & 0.99999415 \\
3215.1048 & 0.99885112 & 1.0000100  \\
3215.1252 & 0.99886645 & 1.0000251  \\
3215.1456 & 0.99883658 & 0.99999469 \\
3215.1661 & 0.99878986 & 0.99994720 \\
3215.2069 & 0.99888244 & 1.0000380  \\
3215.2478 & 0.99885712 & 1.0000101  \\
3215.2682 & 0.99881231 & 0.99996365 \\
3215.2887 & 0.99889947 & 1.0000494  \\
3215.3091 & 0.99883194 & 0.99998002 \\
3215.3295 & 0.99885045 & 0.99999676 \\
3215.3500 & 0.99881200 & 0.99995642 \\
3215.3704 & 0.99882968 & 0.99997227 \\
3215.3908 & 0.99882027 & 0.99996094 \\
3215.4113 & 0.99883350 & 0.99997216 \\
3215.4317 & 0.99879946 & 0.99993611 \\
3215.4521 & 0.99885231 & 0.99998711 \\
3215.4725 & 0.99886587 & 0.99999877 \\
3215.4930 & 0.99883326 & 0.99996428 \\
3215.5134 & 0.99885976 & 0.99998883 \\
3215.5338 & 0.99887064 & 0.99999806 \\
3215.5543 & 0.99886149 & 0.99998723 \\
3215.5747 & 0.99880499 & 0.99992918 \\
3215.5951 & 0.99885553 & 0.99997833 \\
3215.6156 & 0.99884779 & 0.99996934 \\
3215.6360 & 0.99886188 & 0.99998219 \\
3215.6564 & 0.99882506 & 0.99994443 \\
3215.6769 & 0.99876033 & 0.99987867 \\
3215.6973 & 0.99888602 & 1.0000039  \\
3215.7382 & 0.99888898 & 1.0000063  \\
3215.7586 & 0.99893007 & 1.0000474  \\
3215.7790 & 0.99890090 & 1.0000186  \\
3215.7995 & 0.99892052 & 1.0000389  \\
3215.8199 & 0.99890373 & 1.0000230  \\
3215.8403 & 0.99891978 & 1.0000402  \\
3215.8607 & 0.99892278 & 1.0000447  \\
3215.8812 & 0.99887675 & 1.0000004  \\
3215.9016 & 0.99894465 & 1.0000704  \\
3215.9220 & 0.99894388 & 1.0000719  \\
3215.9425 & 0.99892885 & 1.0000594  \\
3215.9833 & 0.99889643 & 1.0000327  \\
3216.0038 & 0.99892843 & 1.0000679  \\
3216.0446 & 0.99884903 & 0.99999516 \\
3216.0651 & 0.99888193 & 1.0000319  \\
3216.0855 & 0.99891855 & 1.0000722  \\
3216.1059 & 0.99886707 & 1.0000245  \\
3216.1264 & 0.99883566 & 0.99999699 \\
3216.1468 & 0.99883696 & 1.0000024  \\
3216.1672 & 0.99887353 & 1.0000431  \\
3216.1877 & 0.99885639 & 1.0000300  \\
3216.2285 & 0.99879578 & 0.99997778 \\
3216.2489 & 0.99875341 & 0.99993947 \\
3216.2694 & 0.99873157 & 0.99992185 \\
3216.2898 & 0.99872841 & 0.99992285 \\
3216.3102 & 0.99876341 & 0.99996201 \\
3216.3307 & 0.99876644 & 0.99996916 \\
3216.3511 & 0.99874997 & 0.99995679 \\
3216.3715 & 0.99876610 & 0.99997670 \\
3216.3920 & 0.99874307 & 0.99995740 \\
3216.4124 & 0.99875698 & 0.99997509 \\
3216.4328 & 0.99874797 & 0.99996953 \\
3216.4533 & 0.99874654 & 0.99997150 \\
3216.4737 & 0.99873307 & 0.99996111 \\
3216.4941 & 0.99873667 & 0.99996783 \\
3216.5146 & 0.99882670 & 1.0000606  \\
3216.5350 & 0.99874918 & 0.99998566 \\
3216.5554 & 0.99878754 & 1.0000265  \\
3216.5759 & 0.99884256 & 1.0000837  \\
3216.5963 & 0.99873021 & 0.99997299 \\
3216.6167 & 0.99879764 & 1.0000421  \\
3216.6371 & 0.99877088 & 1.0000168  \\
3216.6780 & 0.99880127 & 1.0000491  \\
3216.7189 & 0.99877670 & 1.0000256  \\
3216.7393 & 0.99873456 & 0.99998349 \\
3216.7597 & 0.99873778 & 0.99998678 \\
3216.7802 & 0.99874046 & 0.99998928 \\
3216.8006 & 0.99876007 & 1.0000084  \\
3216.8210 & 0.99877302 & 1.0000207  \\
3216.8415 & 0.99876132 & 1.0000084  \\
3216.8619 & 0.99879057 & 1.0000368  \\
3216.8823 & 0.99879184 & 1.0000369  \\
3216.9028 & 0.99880699 & 1.0000508  \\
3216.9641 & 0.99868341 & 0.99992237 \\
3216.9845 & 0.99870304 & 0.99994018 \\
3217.0049 & 0.99874969 & 0.99998498 \\
3217.0254 & 0.99879144 & 1.0000248  \\
3217.0458 & 0.99880536 & 1.0000365  \\
3217.0662 & 0.99879246 & 1.0000214  \\
3217.0866 & 0.99875278 & 0.99997930 \\
3217.1071 & 0.99877858 & 1.0000026  \\
3217.1275 & 0.99879861 & 1.0000202  \\
3217.1479 & 0.99880366 & 1.0000225  \\
3217.1684 & 0.99881438 & 1.0000308  \\
3217.2092 & 0.99871905 & 0.99992995 \\
3217.2297 & 0.99873102 & 0.99993901 \\
3217.2501 & 0.99881585 & 1.0000213  \\
3217.2705 & 0.99880359 & 1.0000061  \\
3217.2910 & 0.99875793 & 0.99995742 \\
3217.3114 & 0.99874168 & 0.99993841 \\
3217.3318 & 0.99876473 & 0.99995850 \\
3217.3523 & 0.99879877 & 0.99998966 \\
3217.3727 & 0.99881397 & 1.0000021  \\
3217.3931 & 0.99878252 & 0.99996766 \\
3217.4136 & 0.99876235 & 0.99994472 \\
3217.4340 & 0.99882075 & 1.0000002  \\
3217.4544 & 0.99882074 & 0.99999745 \\
3217.4748 & 0.99887333 & 1.0000472  \\
3217.4953 & 0.99881181 & 0.99998278 \\
3217.5157 & 0.99882552 & 0.99999358 \\
3217.5361 & 0.99885190 & 1.0000171  \\
3217.5566 & 0.99886313 & 1.0000255  \\
3217.5770 & 0.99884786 & 1.0000075  \\
3217.5974 & 0.99888777 & 1.0000447  \\
3217.6179 & 0.99888256 & 1.0000366  \\
3217.6383 & 0.99888174 & 1.0000329  \\
3217.6587 & 0.99890561 & 1.0000541  \\
3217.6996 & 0.99894013 & 1.0000831  \\
3217.7200 & 0.99885485 & 0.99999496 \\
3217.7405 & 0.99885599 & 0.99999336 \\
3217.7609 & 0.99887616 & 1.0000108  \\
3217.7813 & 0.99889716 & 1.0000290  \\
3217.8018 & 0.99888370 & 1.0000128  \\
3217.8222 & 0.99891037 & 1.0000368  \\
3217.8426 & 0.99892370 & 1.0000474  \\
3217.8630 & 0.99889461 & 1.0000155  \\
3217.8835 & 0.99890311 & 1.0000214  \\
3217.9039 & 0.99885262 & 0.99996814 \\
3217.9243 & 0.99888559 & 0.99999847 \\
3217.9448 & 0.99886244 & 0.99997261 \\
3217.9652 & 0.99884690 & 0.99995454 \\
3217.9856 & 0.99890288 & 1.0000078  \\
3218.0061 & 0.99887680 & 0.99997911 \\
3218.0265 & 0.99885092 & 0.99995051 \\
3218.0469 & 0.99886700 & 0.99996416 \\
3218.0674 & 0.99884251 & 0.99993708 \\
3218.0878 & 0.99887044 & 0.99996236 \\
3218.1082 & 0.99885917 & 0.99994845 \\
3218.1287 & 0.99889317 & 0.99997986 \\
3218.1491 & 0.99887960 & 0.99996389 \\
3218.1900 & 0.99887349 & 0.99995288 \\
3218.2104 & 0.99889022 & 0.99996706 \\
3218.2308 & 0.99891912 & 0.99999337 \\
3218.2512 & 0.99885269 & 0.99992448 \\
3218.2717 & 0.99895493 & 1.0000244  \\
3218.2921 & 0.99896444 & 1.0000316  \\
3218.3125 & 0.99896865 & 1.0000334  \\
3218.3330 & 0.99897374 & 1.0000361  \\
3218.3534 & 0.99897619 & 1.0000362  \\
3218.3738 & 0.99895467 & 1.0000124  \\
3218.3943 & 0.99895632 & 1.0000116  \\
3218.4351 & 0.99892060 & 0.99997140 \\
3218.4556 & 0.99895220 & 1.0000007  \\
3218.4760 & 0.99901976 & 1.0000662  \\
3218.4964 & 0.99897244 & 1.0000165  \\
3218.5373 & 0.99902528 & 1.0000652  \\
3218.5577 & 0.99899108 & 1.0000288  \\
3218.5782 & 0.99897051 & 1.0000061  \\
3218.5986 & 0.99899525 & 1.0000288  \\
3218.6190 & 0.99897826 & 1.0000097  \\
3218.6394 & 0.99903098 & 1.0000605  \\
3218.6599 & 0.99896949 & 0.99999701 \\
3218.6803 & 0.99899547 & 1.0000209  \\
3218.7007 & 0.99898218 & 1.0000056  \\
3218.7212 & 0.99897368 & 0.99999530 \\
3218.7416 & 0.99897144 & 0.99999115 \\
3218.7620 & 0.99897650 & 0.99999430 \\
3218.7825 & 0.99902191 & 1.0000380  \\
3218.8029 & 0.99899903 & 1.0000134  \\
3218.8438 & 0.99900376 & 1.0000146  \\
3218.8642 & 0.99898048 & 0.99998952 \\
3218.8846 & 0.99895187 & 0.99995939 \\
3218.9255 & 0.99898946 & 0.99999361 \\
3218.9459 & 0.99898084 & 0.99998338 \\
3218.9664 & 0.99899449 & 0.99999549 \\
3218.9868 & 0.99899563 & 0.99999514 \\
3219.0072 & 0.99898821 & 0.99998622 \\
3219.0277 & 0.99893190 & 0.99992835 \\
3219.0481 & 0.99901063 & 1.0000058  \\
3219.0685 & 0.99894404 & 0.99993765 \\
3219.0889 & 0.99896385 & 0.99995605 \\
3219.1094 & 0.99896354 & 0.99995442 \\
3219.1707 & 0.99895074 & 0.99993755 \\
3219.1911 & 0.99906161 & 1.0000472  \\
3219.2115 & 0.99905497 & 1.0000393  \\
3219.2320 & 0.99902581 & 1.0000088  \\
3219.2524 & 0.99901497 & 0.99999678 \\
3219.2728 & 0.99901319 & 0.99999380 \\
3219.2933 & 0.99898242 & 0.99996174 \\
3219.3137 & 0.99901231 & 0.99999041 \\
3219.3341 & 0.99903218 & 1.0000091  \\
3219.3546 & 0.99906425 & 1.0000401  \\
3219.3750 & 0.99904495 & 1.0000196  \\
3219.3954 & 0.99905489 & 1.0000283  \\
3219.4159 & 0.99901426 & 0.99998652 \\
3219.4363 & 0.99903715 & 1.0000083  \\
3219.4567 & 0.99905761 & 1.0000277  \\
3219.4771 & 0.99901220 & 0.99998117 \\
3219.4976 & 0.99902032 & 0.99998816 \\
3219.5180 & 0.99898855 & 0.99995529 \\
3219.5384 & 0.99905157 & 1.0000173  \\
3219.5589 & 0.99902498 & 0.99998967 \\
3219.5793 & 0.99902233 & 0.99998582 \\
3219.5997 & 0.99906575 & 1.0000283  \\
3219.6202 & 0.99906876 & 1.0000302  \\
3219.6610 & 0.99908259 & 1.0000418  \\
3219.6815 & 0.99908815 & 1.0000463  \\
3219.7019 & 0.99903113 & 0.99998819 \\
3219.7223 & 0.99902587 & 0.99998173 \\
3219.7428 & 0.99906817 & 1.0000231  \\
3219.7632 & 0.99901236 & 0.99996618 \\
3219.7836 & 0.99901933 & 0.99997190 \\
3219.8041 & 0.99906366 & 1.0000152  \\
3219.8245 & 0.99904280 & 0.99999319 \\
3219.8449 & 0.99906786 & 1.0000171  \\
3219.8653 & 0.99904832 & 0.99999645 \\
3219.9062 & 0.99911378 & 1.0000595  \\
3219.9266 & 0.99907156 & 1.0000159  \\
3219.9471 & 0.99906381 & 1.0000069  \\
3219.9675 & 0.99904310 & 0.99998490 \\
3219.9879 & 0.99902607 & 0.99996654 \\
3220.0084 & 0.99902058 & 0.99995961 \\
3220.0288 & 0.99910624 & 1.0000439  \\
3220.0492 & 0.99902849 & 0.99996472 \\
3220.0697 & 0.99905159 & 0.99998636 \\
3220.0901 & 0.99908975 & 1.0000230  \\
3220.1105 & 0.99904332 & 0.99997498 \\
3220.1514 & 0.99905940 & 0.99998791 \\
3220.1718 & 0.99906878 & 0.99999557 \\
3220.1923 & 0.99905164 & 0.99997680 \\
3220.2127 & 0.99906212 & 0.99998550 \\
3220.2331 & 0.99911093 & 1.0000326  \\
3220.2535 & 0.99912000 & 1.0000397  \\
3220.2740 & 0.99915612 & 1.0000739  \\
3220.2944 & 0.99907411 & 0.99998981 \\
3220.3148 & 0.99908370 & 0.99999744 \\
3220.3353 & 0.99909509 & 1.0000066  \\
3220.3557 & 0.99904522 & 0.99995469 \\
3220.3761 & 0.99910479 & 1.0000121  \\
3220.3966 & 0.99910301 & 1.0000081  \\
3220.4170 & 0.99907152 & 0.99997415 \\
3220.4374 & 0.99909041 & 0.99999073 \\
3220.4579 & 0.99908393 & 0.99998174 \\
3220.4783 & 0.99909086 & 0.99998629 \\
3220.4987 & 0.99912552 & 1.0000184  \\
3220.5192 & 0.99914269 & 1.0000332  \\
3220.5396 & 0.99913355 & 1.0000214  \\
3220.5600 & 0.99909858 & 0.99998393 \\
3220.5805 & 0.99911252 & 0.99999544 \\
3220.6009 & 0.99907841 & 0.99995880 \\
3220.6418 & 0.99911364 & 0.99998904 \\
3220.6622 & 0.99908357 & 0.99995638 \\
3220.6826 & 0.99911779 & 0.99998819 \\
3220.7030 & 0.99910222 & 0.99997028 \\
3220.7235 & 0.99912504 & 0.99999067 \\
3220.7439 & 0.99917136 & 1.0000345  \\
3220.7643 & 0.99917907 & 1.0000399  \\
3220.7848 & 0.99916415 & 1.0000228  \\
3220.8052 & 0.99914956 & 1.0000059  \\
3220.8869 & 0.99918378 & 1.0000320  \\
3220.9074 & 0.99914364 & 0.99998972 \\
3220.9278 & 0.99916444 & 1.0000089  \\
3220.9482 & 0.99916435 & 1.0000071  \\
3220.9687 & 0.99914382 & 0.99998495 \\
3220.9891 & 0.99911678 & 0.99995634 \\
3221.0095 & 0.99915209 & 0.99999007 \\
3221.0300 & 0.99911789 & 0.99995452 \\
3221.0504 & 0.99920628 & 1.0000419  \\
3221.0708 & 0.99925857 & 1.0000931  \\
3221.0912 & 0.99916543 & 0.99999900 \\
3221.1525 & 0.99911857 & 0.99995001 \\
3221.1730 & 0.99913360 & 0.99996458 \\
3221.1934 & 0.99915782 & 0.99998852 \\
3221.2138 & 0.99915137 & 0.99998170 \\
3221.2343 & 0.99917246 & 1.0000027  \\
3221.2547 & 0.99915793 & 0.99998804 \\
3221.2751 & 0.99919640 & 1.0000264  \\
3221.2956 & 0.99920701 & 1.0000371  \\
3221.3160 & 0.99920857 & 1.0000386  \\
3221.3364 & 0.99919787 & 1.0000279  \\
3221.3773 & 0.99915503 & 0.99998525 \\
3221.3977 & 0.99919123 & 1.0000217  \\
3221.4182 & 0.99915895 & 0.99998954 \\
3221.4386 & 0.99914795 & 0.99997864 \\
3221.4590 & 0.99914589 & 0.99997670 \\
3221.4794 & 0.99918806 & 1.0000190  \\
3221.4999 & 0.99916226 & 0.99999333 \\
3221.5203 & 0.99913873 & 0.99996966 \\
3221.5407 & 0.99916446 & 0.99999540 \\
3221.5612 & 0.99916010 & 0.99999092 \\
3221.5816 & 0.99914236 & 0.99997305 \\
3221.6225 & 0.99914201 & 0.99997210 \\
3221.6429 & 0.99919967 & 1.0000293  \\
3221.6633 & 0.99916704 & 0.99999614 \\
3221.6838 & 0.99917824 & 1.0000068  \\
3221.7042 & 0.99915012 & 0.99997783 \\
3221.7246 & 0.99918571 & 1.0000126  \\
3221.7451 & 0.99918351 & 1.0000092  \\
3221.7655 & 0.99922081 & 1.0000455  \\
3221.7859 & 0.99917661 & 0.99999993 \\
3221.8268 & 0.99917560 & 0.99999575 \\
3221.8881 & 0.99920024 & 1.0000143  \\
3221.9085 & 0.99903422 & 0.99984567 \\
3221.9289 & 0.99903294 & 0.99984182 \\
3221.9494 & 0.99903002 & 0.99983628 \\
3221.9698 & 0.99900905 & 0.99981243 \\
3221.9902 & 0.99897547 & 0.99977584 \\
3222.0107 & 0.99898671 & 0.99978393 \\
3222.0311 & 0.99898968 & 0.99978391 \\
3222.0515 & 0.99900124 & 0.99979226 \\
3222.1128 & 0.99897540 & 0.99975597 \\
3222.1333 & 0.99903010 & 0.99980714 \\
3222.1537 & 0.99905321 & 0.99982650 \\
3222.1741 & 0.99903087 & 0.99980063 \\
3222.1946 & 0.99900119 & 0.99976722 \\
3222.2150 & 0.99903021 & 0.99979251 \\
3222.2354 & 0.99904595 & 0.99980463 \\
3222.2559 & 0.99901975 & 0.99977478 \\
3222.2763 & 0.99906422 & 0.99981551 \\
3222.2967 & 0.99921064 & 0.99995829 \\
3222.3171 & 0.99925468 & 0.99999884 \\
3222.3580 & 0.99920795 & 0.99994498 \\
3222.3784 & 0.99926529 & 0.99999896 \\
3222.3989 & 0.99927073 & 1.0000009  \\
3222.4193 & 0.99920584 & 0.99993273 \\
3222.4397 & 0.99923971 & 0.99996334 \\
3222.4602 & 0.99938191 & 1.0001025  \\
3222.4806 & 0.99929214 & 1.0000098  \\
3222.5010 & 0.99930441 & 1.0000192  \\
3222.5215 & 0.99928295 & 0.99999504 \\
3222.5419 & 0.99925319 & 0.99996270 \\
3222.5623 & 0.99935354 & 1.0000607  \\
3222.6032 & 0.99924602 & 0.99994884 \\
3222.6236 & 0.99924624 & 0.99994722 \\
3222.6441 & 0.99928441 & 0.99998374 \\
3222.6645 & 0.99928111 & 0.99997888 \\
3222.6849 & 0.99933309 & 1.0000297  \\
3222.7053 & 0.99932679 & 1.0000220  \\
3222.7258 & 0.99926562 & 0.99995980 \\
3222.7462 & 0.99930060 & 0.99999392 \\
3222.7666 & 0.99929821 & 0.99999063 \\
3222.8075 & 0.99935532 & 1.0000467  \\
3222.8484 & 0.99931340 & 1.0000040  \\
3222.8688 & 0.99926972 & 0.99996021 \\
3222.8892 & 0.99929035 & 0.99998074 \\
3222.9097 & 0.99929103 & 0.99998154 \\
3222.9301 & 0.99934392 & 1.0000345  \\
3222.9505 & 0.99928936 & 0.99998005 \\
3222.9710 & 0.99935711 & 1.0000480  \\
3222.9914 & 0.99935323 & 1.0000444  \\
3223.0118 & 0.99931946 & 1.0000108  \\
3223.0323 & 0.99933373 & 1.0000256  \\
3223.0527 & 0.99930466 & 0.99999685 \\
3223.0935 & 0.99934260 & 1.0000356  \\
3223.1140 & 0.99932985 & 1.0000235  \\
3223.1344 & 0.99934376 & 1.0000379  \\
3223.1548 & 0.99930445 & 0.99999903 \\
3223.1753 & 0.99927362 & 0.99996870 \\
3223.1957 & 0.99929922 & 0.99999487 \\
3223.2161 & 0.99932068 & 1.0000168  \\
3223.2366 & 0.99933008 & 1.0000265  \\
3223.2570 & 0.99936674 & 1.0000637  \\
3223.2774 & 0.99938725 & 1.0000846  \\
3223.2979 & 0.99927627 & 0.99997387 \\
3223.3387 & 0.99925747 & 0.99995553 \\
3223.3592 & 0.99930630 & 1.0000046  \\
3223.3796 & 0.99931641 & 1.0000148  \\
3223.4000 & 0.99927603 & 0.99997422 \\
3223.4205 & 0.99923696 & 0.99993519 \\
3223.4409 & 0.99927679 & 0.99997498 \\
3223.4613 & 0.99925573 & 0.99995379 \\
3223.4818 & 0.99928852 & 0.99998642 \\
3223.5022 & 0.99938078 & 1.0000784  \\
3223.5226 & 0.99928640 & 0.99998365 \\
3223.5430 & 0.99928294 & 0.99997988 \\
3223.5839 & 0.99930063 & 0.99999687 \\
3223.6043 & 0.99928323 & 0.99997892 \\
3223.6248 & 0.99931704 & 1.0000125  \\
3223.6452 & 0.99924818 & 0.99994313 \\
3223.6656 & 0.99926863 & 0.99996312 \\
3223.6861 & 0.99934521 & 1.0000393  \\
3223.7065 & 0.99933044 & 1.0000240  \\
3223.7269 & 0.99933870 & 1.0000319  \\
3223.7474 & 0.99934058 & 1.0000331  \\
3223.7678 & 0.99931339 & 1.0000056  \\
3223.7882 & 0.99929346 & 0.99998516 \\
3223.8291 & 0.99927333 & 0.99996413 \\
3223.8495 & 0.99929211 & 0.99998262 \\
3223.8700 & 0.99930029 & 0.99999044 \\
3223.8904 & 0.99925750 & 0.99994721 \\
3223.9108 & 0.99927673 & 0.99996616 \\
3223.9517 & 0.99921958 & 0.99990849 \\
3223.9721 & 0.99929622 & 0.99998494 \\
3223.9925 & 0.99929384 & 0.99998256 \\
3224.0130 & 0.99928597 & 0.99997463 \\
3224.0334 & 0.99934724 & 1.0000360  \\
3224.0743 & 0.99932663 & 1.0000156  \\
3224.0947 & 0.99929330 & 0.99998238 \\
3224.1151 & 0.99931022 & 0.99999961 \\
3224.1356 & 0.99936512 & 1.0000548  \\
3224.1560 & 0.99934707 & 1.0000373  \\
3224.1764 & 0.99934136 & 1.0000321  \\
3224.1969 & 0.99928376 & 0.99997510 \\
3224.2173 & 0.99929189 & 0.99998383 \\
3224.2377 & 0.99931582 & 1.0000084  \\
3224.2582 & 0.99928001 & 0.99997331 \\
3224.2786 & 0.99934416 & 1.0000383  \\
3224.3195 & 0.99938704 & 1.0000830  \\
3224.3399 & 0.99930007 & 0.99999690 \\
3224.3603 & 0.99929978 & 0.99999763 \\
3224.3807 & 0.99923629 & 0.99993511 \\
3224.4012 & 0.99928499 & 0.99998480 \\
3224.4216 & 0.99929875 & 0.99999964 \\
3224.4420 & 0.99932338 & 1.0000254  \\
3224.4625 & 0.99928717 & 0.99999014 \\
3224.4829 & 0.99933760 & 1.0000417  \\
3224.5033 & 0.99930103 & 1.0000063  \\
3224.5646 & 0.99928937 & 0.99999795 \\
3224.5851 & 0.99932260 & 1.0000321  \\
3224.6055 & 0.99932438 & 1.0000349  \\
3224.6259 & 0.99928555 & 0.99999711 \\
3224.6464 & 0.99936285 & 1.0000755  \\
3224.6668 & 0.99929417 & 1.0000078  \\
3224.6872 & 0.99929573 & 1.0000104  \\
3224.7077 & 0.99930774 & 1.0000234  \\
3224.7281 & 0.99929916 & 1.0000157  \\
3224.7485 & 0.99933215 & 1.0000496  \\
3224.7689 & 0.99928480 & 1.0000030  \\
3224.8098 & 0.99927644 & 0.99999634 \\
3224.8302 & 0.99924232 & 0.99996268 \\
3224.8507 & 0.99931655 & 1.0000377  \\
3224.8711 & 0.99930687 & 1.0000286  \\
3224.8915 & 0.99928894 & 1.0000113  \\
3224.9120 & 0.99922329 & 0.99994596 \\
3224.9324 & 0.99927978 & 1.0000030  \\
3224.9528 & 0.99926992 & 0.99999334 \\
3224.9733 & 0.99920195 & 0.99992567 \\
3225.0141 & 0.99925249 & 0.99997667 \\
3225.0754 & 0.99925922 & 0.99998394 \\
3225.0959 & 0.99920989 & 0.99993470 \\
3225.1163 & 0.99923088 & 0.99995588 \\
3225.1367 & 0.99924523 & 0.99997036 \\
3225.1571 & 0.99928090 & 1.0000062  \\
3225.1776 & 0.99923929 & 0.99996454 \\
3225.1980 & 0.99922956 & 0.99995485 \\
3225.2184 & 0.99927530 & 1.0000007  \\
3225.2389 & 0.99930812 & 1.0000337  \\
3225.2593 & 0.99929510 & 1.0000207  \\
3225.3002 & 0.99929777 & 1.0000236  \\
3225.3206 & 0.99927816 & 1.0000041  \\
3225.3410 & 0.99927440 & 1.0000006  \\
3225.3615 & 0.99926494 & 0.99999140 \\
3225.3819 & 0.99928238 & 1.0000090  \\
3225.4023 & 0.99925560 & 0.99998241 \\
3225.4432 & 0.99923970 & 0.99996709 \\
3225.4636 & 0.99925791 & 0.99998574 \\
3225.4841 & 0.99924864 & 0.99997717 \\
3225.5045 & 0.99923679 & 0.99996561 \\
3225.5454 & 0.99929164 & 1.0000217  \\
3225.5658 & 0.99930289 & 1.0000337  \\
3225.5862 & 0.99925016 & 0.99998180 \\
3225.6066 & 0.99926935 & 1.0000018  \\
3225.6271 & 0.99927661 & 1.0000099  \\
3225.6475 & 0.99931341 & 1.0000479  \\
3225.6679 & 0.99929530 & 1.0000308  \\
3225.6884 & 0.99927212 & 1.0000088  \\
3225.7088 & 0.99923086 & 0.99996862 \\
3225.7292 & 0.99924069 & 0.99997977 \\
3225.7497 & 0.99922573 & 0.99996617 \\
3225.7905 & 0.99927103 & 1.0000142  \\
3225.8110 & 0.99925574 & 1.0000004  \\
3225.8314 & 0.99933505 & 1.0000812  \\
3225.8518 & 0.99925724 & 1.0000050  \\
3225.8723 & 0.99928753 & 1.0000368  \\
3225.8927 & 0.99928532 & 1.0000362  \\
3225.9131 & 0.99921914 & 0.99997162 \\
3225.9336 & 0.99923387 & 0.99998792 \\
3225.9540 & 0.99925354 & 1.0000093  \\
3225.9744 & 0.99922917 & 0.99998656 \\
3225.9948 & 0.99926672 & 1.0000258  \\
3226.0357 & 0.99923059 & 0.99999275 \\
3226.0561 & 0.99924035 & 1.0000042  \\
3226.0766 & 0.99923108 & 0.99999652 \\
3226.0970 & 0.99919703 & 0.99996406 \\
3226.1174 & 0.99923507 & 1.0000036  \\
3226.1379 & 0.99925212 & 1.0000222  \\
3226.1583 & 0.99923763 & 1.0000093  \\
3226.1787 & 0.99920385 & 0.99997690 \\
3226.1992 & 0.99926544 & 1.0000401  \\
3226.2196 & 0.99926825 & 1.0000442  \\
3226.2400 & 0.99923010 & 1.0000074  \\
3226.3013 & 0.99923828 & 1.0000190  \\
3226.3218 & 0.99922698 & 1.0000088  \\
3226.3422 & 0.99922528 & 1.0000081  \\
3226.3626 & 0.99925160 & 1.0000354  \\
3226.3830 & 0.99919204 & 0.99997672 \\
3226.4035 & 0.99919602 & 0.99998136 \\
3226.4239 & 0.99924634 & 1.0000325  \\
3226.4443 & 0.99924142 & 1.0000281  \\
3226.4648 & 0.99917155 & 0.99995878 \\
3226.4852 & 0.99920800 & 0.99999579 \\
3226.5261 & 0.99918348 & 0.99997197 \\
3226.5465 & 0.99921242 & 1.0000012  \\
3226.5669 & 0.99917399 & 0.99996307 \\
3226.5874 & 0.99920691 & 0.99999625 \\
3226.6078 & 0.99920713 & 0.99999683 \\
3226.6282 & 0.99914520 & 0.99993485 \\
3226.6487 & 0.99914830 & 0.99993819 \\
3226.6691 & 0.99918831 & 0.99997835 \\
3226.7100 & 0.99918085 & 0.99997101 \\
3226.7713 & 0.99923024 & 1.0000205  \\
3226.7917 & 0.99920219 & 0.99999248 \\
3226.8121 & 0.99922063 & 1.0000109  \\
3226.8325 & 0.99917148 & 0.99996175 \\
3226.8530 & 0.99921976 & 1.0000101  \\
3226.8734 & 0.99922080 & 1.0000112  \\
3226.8938 & 0.99916004 & 0.99995036 \\
3226.9143 & 0.99922690 & 1.0000175  \\
3226.9347 & 0.99915985 & 0.99995034 \\
3226.9551 & 0.99917657 & 0.99996720 \\
3226.9756 & 0.99920564 & 0.99999641 \\
3227.0164 & 0.99927866 & 1.0000698  \\
3227.0369 & 0.99926989 & 1.0000614  \\
3227.0573 & 0.99921864 & 1.0000104  \\
3227.0777 & 0.99921776 & 1.0000100  \\
3227.0982 & 0.99925168 & 1.0000443  \\
3227.1186 & 0.99919135 & 0.99998444 \\
3227.1390 & 0.99919914 & 0.99999265 \\
3227.1595 & 0.99923022 & 1.0000244  \\
3227.1799 & 0.99924466 & 1.0000394  \\
3227.2003 & 0.99927403 & 1.0000695  \\
3227.2207 & 0.99921164 & 1.0000077  \\
3227.2616 & 0.99918598 & 0.99998372 \\
3227.2820 & 0.99918022 & 0.99997855 \\
3227.3025 & 0.99921567 & 1.0000150  \\
3227.3229 & 0.99920463 & 1.0000047  \\
3227.3433 & 0.99916321 & 0.99996397 \\
3227.3638 & 0.99926977 & 1.0000717  \\
3227.3842 & 0.99922559 & 1.0000283  \\
3227.4046 & 0.99916600 & 0.99996938 \\
3227.4251 & 0.99914693 & 0.99995120 \\
3227.4659 & 0.99922369 & 1.0000298  \\
3227.5068 & 0.99919759 & 1.0000051  \\
3227.5272 & 0.99921856 & 1.0000269  \\
3227.5477 & 0.99917595 & 0.99998496 \\
3227.5681 & 0.99918093 & 0.99999059 \\
3227.5885 & 0.99919977 & 1.0000100  \\
3227.6090 & 0.99919667 & 1.0000075  \\
3227.6294 & 0.99915765 & 0.99996914 \\
3227.6498 & 0.99919172 & 1.0000037  \\
3227.6702 & 0.99919679 & 1.0000092  \\
3227.6907 & 0.99915500 & 0.99996780 \\
3227.7111 & 0.99913905 & 0.99995208 \\
3227.7520 & 0.99914806 & 0.99996139 \\
3227.7724 & 0.99917086 & 0.99998427 \\
3227.7928 & 0.99917144 & 0.99998485 \\
3227.8133 & 0.99915169 & 0.99996479 \\
3227.8337 & 0.99913544 & 0.99994847 \\
3227.8541 & 0.99916339 & 0.99997602 \\
3227.8746 & 0.99910323 & 0.99991551 \\
3227.8950 & 0.99913377 & 0.99994548 \\
3227.9154 & 0.99923235 & 1.0000434  \\
3227.9359 & 0.99920473 & 1.0000150  \\
3227.9563 & 0.99921118 & 1.0000207  \\
3227.9972 & 0.99924075 & 1.0000483  \\
3228.0380 & 0.99918828 & 0.99999341 \\
3228.0584 & 0.99925762 & 1.0000615  \\
3228.0789 & 0.99924457 & 1.0000471  \\
3228.0993 & 0.99922777 & 1.0000288  \\
3228.1197 & 0.99921973 & 1.0000193  \\
3228.1402 & 0.99924646 & 1.0000444  \\
3228.1606 & 0.99922006 & 1.0000163  \\
3228.1810 & 0.99920835 & 1.0000029  \\
3228.2015 & 0.99924230 & 1.0000351  \\
3228.2423 & 0.99919566 & 0.99998476 \\
3228.2628 & 0.99925061 & 1.0000380  \\
3228.2832 & 0.99919060 & 0.99997593 \\
3228.3036 & 0.99922199 & 1.0000054  \\
3228.3241 & 0.99919549 & 0.99997689 \\
3228.3445 & 0.99926690 & 1.0000462  \\
3228.3649 & 0.99918209 & 0.99995930 \\
3228.3854 & 0.99923777 & 1.0000128  \\
3228.4058 & 0.99921003 & 0.99998297 \\
3228.4262 & 0.99925371 & 1.0000246  \\
3228.4467 & 0.99927418 & 1.0000429  \\
3228.4671 & 0.99920425 & 0.99997074 \\
3228.4875 & 0.99923419 & 0.99999844 \\
3228.5079 & 0.99926153 & 1.0000236  \\
3228.5284 & 0.99923823 & 0.99999813 \\
3228.5488 & 0.99924145 & 0.99999903 \\
3228.5692 & 0.99924528 & 1.0000008  \\
3228.5897 & 0.99924327 & 0.99999661 \\
3228.6101 & 0.99923315 & 0.99998428 \\
3228.6305 & 0.99921157 & 0.99996071 \\
3228.6510 & 0.99924816 & 0.99999506 \\
3228.6714 & 0.99925989 & 1.0000048  \\
3228.6918 & 0.99925258 & 0.99999525 \\
3228.7327 & 0.99923148 & 0.99997014 \\
3228.7531 & 0.99924766 & 0.99998424 \\
3228.7736 & 0.99928509 & 1.0000197  \\
3228.7940 & 0.99921944 & 0.99995213 \\
3228.8144 & 0.99925382 & 0.99998444 \\
3228.8349 & 0.99927105 & 0.99999978 \\
3228.8553 & 0.99922188 & 0.99994861 \\
3228.8757 & 0.99924770 & 0.99997265 \\
3228.8961 & 0.99928791 & 1.0000109  \\
3228.9166 & 0.99928175 & 1.0000029  \\
3228.9370 & 0.99925744 & 0.99997685 \\
3228.9779 & 0.99928078 & 0.99999663 \\
3228.9983 & 0.99929982 & 1.0000140  \\
3229.0187 & 0.99925478 & 0.99996722 \\
3229.0392 & 0.99931805 & 1.0000289  \\
3229.0596 & 0.99927956 & 0.99998861 \\
3229.0800 & 0.99928639 & 0.99999390 \\
3229.1005 & 0.99931073 & 1.0000166  \\
3229.1209 & 0.99933816 & 1.0000424  \\
3229.1413 & 0.99929450 & 0.99999712 \\
3229.1618 & 0.99929490 & 0.99999597 \\
3229.1822 & 0.99930816 & 1.0000079  \\
3229.2026 & 0.99934516 & 1.0000434  \\
3229.2231 & 0.99932298 & 1.0000196  \\
3229.2435 & 0.99932257 & 1.0000179  \\
3229.2639 & 0.99932743 & 1.0000214  \\
3229.2844 & 0.99931917 & 1.0000117  \\
3229.3048 & 0.99934762 & 1.0000389  \\
3229.3252 & 0.99932215 & 1.0000121  \\
3229.3456 & 0.99933569 & 1.0000244  \\
3229.3661 & 0.99932327 & 1.0000107  \\
3229.3865 & 0.99933728 & 1.0000236  \\
3229.4069 & 0.99931102 & 0.99999618 \\
3229.4274 & 0.99930909 & 0.99999299 \\
3229.4682 & 0.99934374 & 1.0000256  \\
3229.4887 & 0.99929626 & 0.99997699 \\
3229.5091 & 0.99927131 & 0.99995113 \\
3229.5295 & 0.99927703 & 0.99995578 \\
3229.5500 & 0.99926802 & 0.99994581 \\
3229.5704 & 0.99934476 & 1.0000215  \\
3229.5908 & 0.99932426 & 1.0000002  \\
3229.6113 & 0.99928611 & 0.99996117 \\
3229.6317 & 0.99932062 & 0.99999462 \\
3229.6521 & 0.99937210 & 1.0000453  \\
3229.6726 & 0.99928991 & 0.99996223 \\
3229.7134 & 0.99934162 & 1.0000122  \\
3229.7338 & 0.99933988 & 1.0000096  \\
3229.7543 & 0.99933518 & 1.0000041  \\
3229.7747 & 0.99933911 & 1.0000072  \\
3229.7951 & 0.99934327 & 1.0000104  \\
3229.8156 & 0.99930810 & 0.99997446 \\
3229.8360 & 0.99927002 & 0.99993552 \\
3229.8564 & 0.99936601 & 1.0000308  \\
3229.8769 & 0.99932611 & 0.99999010 \\
3229.8973 & 0.99930894 & 0.99997209 \\
3229.9177 & 0.99934940 & 1.0000117  \\
3229.9586 & 0.99930143 & 0.99996212 \\
3229.9790 & 0.99934973 & 1.0000096  \\
3229.9995 & 0.99931465 & 0.99997380 \\
3230.0199 & 0.99936002 & 1.0000182  \\
3230.0403 & 0.99937152 & 1.0000288  \\
3230.0608 & 0.99930410 & 0.99996050 \\
3230.0812 & 0.99937241 & 1.0000278  \\
3230.1016 & 0.99935729 & 1.0000119  \\
3230.1221 & 0.99936000 & 1.0000136  \\
3230.1425 & 0.99935589 & 1.0000087  \\
3230.1629 & 0.99936147 & 1.0000133  \\
3230.2038 & 0.99932275 & 0.99997243 \\
3230.2242 & 0.99937353 & 1.0000222  \\
3230.2446 & 0.99937672 & 1.0000245  \\
3230.2651 & 0.99936503 & 1.0000117  \\
3230.2855 & 0.99936638 & 1.0000120  \\
3230.3059 & 0.99939430 & 1.0000388  \\
3230.3264 & 0.99935491 & 0.99999846 \\
3230.3468 & 0.99934896 & 0.99999149 \\
3230.3672 & 0.99937741 & 1.0000188  \\
3230.3877 & 0.99938880 & 1.0000292  \\
3230.4081 & 0.99938321 & 1.0000225  \\
3230.4490 & 0.99941620 & 1.0000535  \\
3230.4694 & 0.99940814 & 1.0000443  \\
3230.4898 & 0.99934678 & 0.99998174 \\
3230.5103 & 0.99937495 & 1.0000089  \\
3230.5307 & 0.99934658 & 0.99997945 \\
3230.5511 & 0.99932981 & 0.99996160 \\
3230.5715 & 0.99930250 & 0.99993319 \\
3230.5920 & 0.99939625 & 1.0000261  \\
3230.6124 & 0.99937108 & 0.99999973 \\
3230.6328 & 0.99936339 & 0.99999114 \\
3230.6533 & 0.99930137 & 0.99992801 \\
3230.6941 & 0.99936245 & 0.99998722 \\
3230.7146 & 0.99933573 & 0.99995959 \\
3230.7350 & 0.99936278 & 0.99998564 \\
3230.7554 & 0.99939816 & 1.0000203  \\
3230.7759 & 0.99935455 & 0.99997562 \\
3230.7963 & 0.99938672 & 1.0000069  \\
3230.8167 & 0.99940135 & 1.0000208  \\
3230.8372 & 0.99933409 & 0.99995258 \\
3230.8576 & 0.99936694 & 0.99998473 \\
3230.8780 & 0.99935074 & 0.99996781 \\
3230.8985 & 0.99936720 & 0.99998356 \\
3230.9393 & 0.99940198 & 1.0000169  \\
3230.9598 & 0.99936472 & 0.99997911 \\
3230.9802 & 0.99936824 & 0.99998186 \\
3231.0006 & 0.99941644 & 1.0000295  \\
3231.0210 & 0.99938622 & 0.99999859 \\
3231.0415 & 0.99940567 & 1.0000175  \\
3231.0619 & 0.99941163 & 1.0000227  \\
3231.0823 & 0.99936465 & 0.99997511 \\
3231.1028 & 0.99939485 & 1.0000048  \\
3231.1232 & 0.99937668 & 0.99998589 \\
3231.1436 & 0.99939490 & 1.0000035  \\
3231.1845 & 0.99938447 & 0.99999190 \\
3231.2049 & 0.99939078 & 0.99999737 \\
3231.2254 & 0.99941019 & 1.0000161  \\
3231.2458 & 0.99941928 & 1.0000245  \\
3231.2662 & 0.99939455 & 0.99999912 \\
3231.2867 & 0.99939634 & 1.0000001  \\
3231.3071 & 0.99950669 & 1.0001097  \\
3231.3275 & 0.99943141 & 1.0000335  \\
3231.3480 & 0.99942785 & 1.0000290  \\
3231.3684 & 0.99943122 & 1.0000316  \\
3231.3888 & 0.99941420 & 1.0000134  \\
3231.4297 & 0.99942575 & 1.0000231  \\
3231.4501 & 0.99940906 & 1.0000051  \\
3231.4705 & 0.99939739 & 0.99999218 \\
3231.5114 & 0.99939345 & 0.99998573 \\
3231.5318 & 0.99943841 & 1.0000293  \\
3231.5523 & 0.99941598 & 1.0000053  \\
3231.5727 & 0.99945655 & 1.0000445  \\
3231.5931 & 0.99941564 & 1.0000017  \\
3231.6136 & 0.99936054 & 0.99994505 \\
3231.6340 & 0.99938105 & 0.99996379 \\
3231.6749 & 0.99941857 & 0.99999745 \\
3231.7157 & 0.99941223 & 0.99998699 \\
3231.7566 & 0.99940371 & 0.99997400 \\
3231.7770 & 0.99945376 & 1.0000218  \\
3231.8383 & 0.99942629 & 0.99998728 \\
3231.8587 & 0.99939281 & 0.99995140 \\
3231.8792 & 0.99945101 & 1.0000071  \\
3231.9200 & 0.99941800 & 0.99996897 \\
3231.9405 & 0.99941601 & 0.99996453 \\
3231.9609 & 0.99940842 & 0.99995431 \\
3231.9813 & 0.99946735 & 1.0000108  \\
3232.0018 & 0.99945932 & 1.0000000  \\
3232.0222 & 0.99943014 & 0.99996835 \\
3232.0426 & 0.99944306 & 0.99997877 \\
3232.0631 & 0.99946007 & 0.99999335 \\
3232.0835 & 0.99948768 & 1.0000185  \\
3232.1039 & 0.99944261 & 0.99997082 \\
3232.1244 & 0.99943803 & 0.99996379 \\
3232.1652 & 0.99946978 & 0.99999084 \\
3232.1857 & 0.99943639 & 0.99995498 \\
3232.2061 & 0.99947441 & 0.99999082 \\
3232.2265 & 0.99958035 & 1.0000945  \\
3232.2470 & 0.99958225 & 1.0000944  \\
3232.2674 & 0.99947301 & 0.99998298 \\
3232.2878 & 0.99949435 & 1.0000023  \\
3232.3082 & 0.99950771 & 1.0000137  \\
3232.3287 & 0.99951182 & 1.0000160  \\
3232.3491 & 0.99949985 & 1.0000021  \\
3232.3695 & 0.99948188 & 0.99998267 \\
3232.4104 & 0.99950596 & 1.0000037  \\
3232.4308 & 0.99955586 & 1.0000521  \\
3232.4513 & 0.99948500 & 0.99998001 \\
3232.4717 & 0.99951786 & 1.0000116  \\
3232.4921 & 0.99951076 & 1.0000033  \\
3232.5126 & 0.99954162 & 1.0000333  \\
3232.5330 & 0.99951846 & 1.0000091  \\
3232.5534 & 0.99950152 & 0.99999128 \\
3232.5739 & 0.99950680 & 0.99999574 \\
3232.5943 & 0.99948593 & 0.99997413 \\
3232.6147 & 0.99952202 & 1.0000097  \\
3232.6556 & 0.99952602 & 1.0000125  \\
3232.6760 & 0.99949441 & 0.99998036 \\
3232.6965 & 0.99943153 & 0.99991697 \\
3232.7169 & 0.99954200 & 1.0000271  \\
3232.7373 & 0.99949830 & 0.99998306 \\
3232.7577 & 0.99956891 & 1.0000534  \\
3232.7782 & 0.99951678 & 1.0000010  \\
3232.7986 & 0.99950714 & 0.99999118 \\
3232.8190 & 0.99953043 & 1.0000143  \\
3232.8395 & 0.99956370 & 1.0000474  \\
3232.8599 & 0.99957106 & 1.0000547  \\
3232.9008 & 0.99951756 & 1.0000011  \\
3232.9212 & 0.99953658 & 1.0000200  \\
3232.9416 & 0.99951561 & 0.99999900 \\
3232.9621 & 0.99949220 & 0.99997546 \\
3232.9825 & 0.99947866 & 0.99996198 \\
3233.0029 & 0.99952055 & 1.0000039  \\
3233.0234 & 0.99950300 & 0.99998638 \\
3233.0438 & 0.99949397 & 0.99997735 \\
3233.0642 & 0.99951112 & 0.99999439 \\
3233.0847 & 0.99954917 & 1.0000325  \\
3233.1051 & 0.99946881 & 0.99995218 \\
3233.1459 & 0.99952167 & 1.0000048  \\
3233.1664 & 0.99950613 & 0.99998934 \\
3233.1868 & 0.99950712 & 0.99999015 \\
3233.2072 & 0.99947511 & 0.99995812 \\
3233.2277 & 0.99951708 & 1.0000000  \\
3233.2481 & 0.99950578 & 0.99998851 \\
3233.2685 & 0.99953209 & 1.0000147  \\
3233.2890 & 0.99948880 & 0.99997117 \\
3233.3094 & 0.99949330 & 0.99997554 \\
3233.3298 & 0.99953407 & 1.0000162  \\
3233.3503 & 0.99947865 & 0.99996048 \\
3233.3911 & 0.99951468 & 0.99999605 \\
3233.4116 & 0.99956541 & 1.0000465  \\
3233.4320 & 0.99955134 & 1.0000322  \\
3233.4524 & 0.99953472 & 1.0000154  \\
3233.4729 & 0.99949673 & 0.99997701 \\
3233.4933 & 0.99949485 & 0.99997483 \\
3233.5137 & 0.99951529 & 0.99999498 \\
3233.5342 & 0.99956956 & 1.0000490  \\
3233.5546 & 0.99955812 & 1.0000371  \\
3233.5750 & 0.99958984 & 1.0000687  \\
3233.5954 & 0.99949629 & 0.99997461 \\
3233.6363 & 0.99951347 & 0.99999102 \\
3233.6567 & 0.99951354 & 0.99999073 \\
3233.6772 & 0.99955729 & 1.0000341  \\
3233.6976 & 0.99954169 & 1.0000181  \\
3233.7180 & 0.99950615 & 0.99998227 \\
3233.7385 & 0.99945481 & 0.99993042 \\
3233.7793 & 0.99955439 & 1.0000292  \\
3233.7998 & 0.99951350 & 0.99998794 \\
3233.8202 & 0.99952417 & 0.99999815 \\
3233.8406 & 0.99957197 & 1.0000455  \\
3233.8815 & 0.99949927 & 0.99997187 \\
3233.9019 & 0.99951518 & 0.99998736 \\
3233.9224 & 0.99954234 & 1.0000139  \\
3233.9428 & 0.99955685 & 1.0000281  \\
3233.9632 & 0.99953023 & 1.0000009  \\
3233.9837 & 0.99954982 & 1.0000200  \\
3234.0041 & 0.99954513 & 1.0000149  \\
3234.0245 & 0.99952892 & 0.99999818 \\
3234.0449 & 0.99950240 & 0.99997112 \\
3234.0654 & 0.99951517 & 0.99998342 \\
3234.0858 & 0.99948275 & 0.99995039 \\
3234.1267 & 0.99951052 & 0.99997691 \\
3234.1471 & 0.99954830 & 1.0000142  \\
3234.1675 & 0.99955064 & 1.0000159  \\
3234.1880 & 0.99951825 & 0.99998286 \\
3234.2084 & 0.99956490 & 1.0000288  \\
3234.2288 & 0.99953514 & 0.99999845 \\
3234.2493 & 0.99953543 & 0.99999796 \\
3234.2697 & 0.99952827 & 0.99999003 \\
3234.2901 & 0.99954087 & 1.0000018  \\
3234.3106 & 0.99954205 & 1.0000022  \\
3234.3310 & 0.99950093 & 0.99996022 \\
3234.3719 & 0.99954464 & 1.0000020  \\
3234.3923 & 0.99956236 & 1.0000188  \\
3234.4127 & 0.99956698 & 1.0000225  \\
3234.4332 & 0.99955808 & 1.0000125  \\
3234.4536 & 0.99954371 & 0.99999700 \\
3234.4740 & 0.99956684 & 1.0000190  \\
3234.4944 & 0.99955230 & 1.0000033  \\
3234.5149 & 0.99953959 & 0.99998936 \\
3234.5353 & 0.99951375 & 0.99996220 \\
3234.5557 & 0.99955413 & 1.0000013  \\
3234.5762 & 0.99954097 & 0.99998675 \\
3234.6170 & 0.99952372 & 0.99996663 \\
3234.6375 & 0.99954317 & 0.99998460 \\
3234.6579 & 0.99953611 & 0.99997586 \\
3234.6783 & 0.99957544 & 1.0000137  \\
3234.6988 & 0.99957407 & 1.0000105  \\
3234.7192 & 0.99950577 & 0.99994044 \\
3234.7396 & 0.99960087 & 1.0000339  \\
3234.7601 & 0.99960892 & 1.0000402  \\
3234.7805 & 0.99954298 & 0.99997230 \\
3234.8009 & 0.99954707 & 0.99997467 \\
3234.8214 & 0.99959004 & 1.0000156  \\
3234.8622 & 0.99957207 & 0.99999407 \\
3234.8826 & 0.99959882 & 1.0000189  \\
3234.9031 & 0.99959224 & 1.0000105  \\
3234.9235 & 0.99964280 & 1.0000591  \\
3234.9439 & 0.99957885 & 0.99999346 \\
3234.9644 & 0.99961548 & 1.0000283  \\
3234.9848 & 0.99960589 & 1.0000169  \\
3235.0052 & 0.99961802 & 1.0000272  \\
3235.0257 & 0.99964181 & 1.0000492  \\
3235.0461 & 0.99961752 & 1.0000234  \\
3235.0665 & 0.99957770 & 0.99998170 \\
3235.1074 & 0.99959247 & 0.99999361 \\
3235.1278 & 0.99960195 & 1.0000016  \\
3235.1483 & 0.99960092 & 0.99999914 \\
3235.1687 & 0.99958230 & 0.99997926 \\
3235.1891 & 0.99963920 & 1.0000350  \\
3235.2096 & 0.99959115 & 0.99998566 \\
3235.2300 & 0.99960957 & 1.0000031  \\
3235.2504 & 0.99957593 & 0.99996859 \\
3235.2709 & 0.99958794 & 0.99997971 \\
3235.2913 & 0.99958347 & 0.99997447 \\
3235.3117 & 0.99961372 & 1.0000042  \\
3235.3526 & 0.99958282 & 0.99997233 \\
3235.3730 & 0.99957987 & 0.99996914 \\
3235.3934 & 0.99957326 & 0.99996234 \\
3235.4139 & 0.99957221 & 0.99996123 \\
3235.4343 & 0.99959573 & 0.99998500 \\
3235.4547 & 0.99958549 & 0.99997499 \\
3235.4752 & 0.99963964 & 1.0000296  \\
3235.4956 & 0.99970798 & 1.0000984  \\
3235.5160 & 0.99966863 & 1.0000597  \\
3235.5365 & 0.99954449 & 0.99993607 \\
3235.5569 & 0.99960741 & 0.99999972 \\
3235.5978 & 0.99958233 & 0.99997631 \\
3235.6182 & 0.99963632 & 1.0000313  \\
3235.6386 & 0.99962370 & 1.0000196  \\
3235.6591 & 0.99956504 & 0.99996199 \\
3235.6795 & 0.99966255 & 1.0000606  \\
3235.6999 & 0.99962718 & 1.0000261  \\
3235.7204 & 0.99959188 & 0.99999183 \\
3235.8634 & 0.99962203 & 1.0000285  \\
3235.8838 & 0.99959361 & 1.0000010  \\
3235.9042 & 0.99958288 & 0.99999087 \\
3235.9247 & 0.99957531 & 0.99998390 \\
3235.9451 & 0.99957958 & 0.99998876 \\
3235.9655 & 0.99952824 & 0.99993776 \\
3235.9860 & 0.99956034 & 0.99997017 \\
3236.0064 & 0.99959055 & 1.0000005  \\
3236.0268 & 0.99960744 & 1.0000176  \\
3236.0473 & 0.99957729 & 0.99998731 \\
3236.0881 & 0.99958073 & 0.99999027 \\
3236.1086 & 0.99955067 & 0.99995960 \\
3236.1290 & 0.99960093 & 1.0000092  \\
3236.1494 & 0.99957490 & 0.99998223 \\
3236.1699 & 0.99962117 & 1.0000275  \\
3236.1903 & 0.99960134 & 1.0000064  \\
3236.2107 & 0.99960200 & 1.0000056  \\
3236.2311 & 0.99965677 & 1.0000587  \\
3236.2516 & 0.99952258 & 0.99992298 \\
3236.2720 & 0.99962467 & 1.0000231  \\
3236.2924 & 0.99966167 & 1.0000582  \\
3236.3333 & 0.99962747 & 1.0000201  \\
3236.3537 & 0.99963920 & 1.0000296  \\
3236.3742 & 0.99957814 & 0.99996628 \\
3236.3946 & 0.99961333 & 0.99999909 \\
3236.4150 & 0.99963573 & 1.0000193  \\
3236.4355 & 0.99960590 & 0.99998701 \\
3236.4559 & 0.99957011 & 0.99994858 \\
3236.4763 & 0.99962046 & 0.99999669 \\
3236.4968 & 0.99964788 & 1.0000217  \\
3236.5172 & 0.99962212 & 0.99999346 \\
3236.5376 & 0.99955553 & 0.99992457 \\
3236.5785 & 0.99965289 & 1.0000174  \\
3236.6194 & 0.99966639 & 1.0000265  \\
3236.6398 & 0.99964662 & 1.0000048  \\
3236.6602 & 0.99967850 & 1.0000347  \\
3236.6806 & 0.99964101 & 0.99999536 \\
3236.7011 & 0.99966656 & 1.0000193  \\
3236.7215 & 0.99970065 & 1.0000519  \\
3236.7419 & 0.99963291 & 0.99998272 \\
3236.7828 & 0.99966381 & 1.0000112  \\
3236.8441 & 0.99966894 & 1.0000143  \\
3236.8645 & 0.99964533 & 0.99999032 \\
3236.8850 & 0.99965516 & 1.0000003  \\
3236.9054 & 0.99967478 & 1.0000202  \\
3236.9258 & 0.99964229 & 0.99998806 \\
3236.9463 & 0.99965160 & 0.99999814 \\
3236.9667 & 0.99961420 & 0.99996156 \\
3236.9871 & 0.99970638 & 1.0000549  \\
3237.0076 & 0.99965290 & 1.0000027  \\
3237.0280 & 0.99964722 & 0.99999865 \\
3237.0689 & 0.99964581 & 1.0000007  \\
3237.0893 & 0.99968807 & 1.0000451  \\
3237.1097 & 0.99967339 & 1.0000325  \\
3237.1301 & 0.99960857 & 0.99997000 \\
3237.1506 & 0.99966208 & 1.0000259  \\
3237.1710 & 0.99956782 & 0.99993407 \\
3237.1914 & 0.99962474 & 0.99999351 \\
3237.2119 & 0.99960036 & 0.99997181 \\
3237.2323 & 0.99961112 & 0.99998526 \\
3237.2527 & 0.99961917 & 0.99999611 \\
3237.2732 & 0.99957150 & 0.99995122 \\
3237.3140 & 0.99958812 & 0.99997363 \\
3237.3345 & 0.99959230 & 0.99998079 \\
3237.3549 & 0.99963001 & 1.0000213  \\
3237.3753 & 0.99961131 & 1.0000055  \\
3237.3958 & 0.99960254 & 0.99999945 \\
3237.4162 & 0.99960806 & 1.0000077  \\
3237.4366 & 0.99956791 & 0.99997041 \\
3237.4571 & 0.99963057 & 1.0000356  \\
3237.4775 & 0.99956578 & 0.99997340 \\
3237.4979 & 0.99959703 & 1.0000072  \\
3237.5184 & 0.99958683 & 0.99999941 \\
3237.5592 & 0.99954440 & 0.99996138 \\
3237.5796 & 0.99956636 & 0.99998531 \\
3237.6001 & 0.99955248 & 0.99997322 \\
3237.6205 & 0.99956912 & 0.99999172 \\
3237.6409 & 0.99953649 & 0.99996044 \\
3237.6614 & 0.99956059 & 0.99998587 \\
3237.6818 & 0.99958809 & 1.0000147  \\
3237.7022 & 0.99958976 & 1.0000172  \\
3237.7227 & 0.99954837 & 0.99997656 \\
3237.7431 & 0.99958995 & 1.0000188  \\
3237.7635 & 0.99958615 & 1.0000154  \\
3237.8044 & 0.99958424 & 1.0000141  \\
3237.8248 & 0.99960662 & 1.0000364  \\
3237.8453 & 0.99961467 & 1.0000445  \\
3237.8657 & 0.99962720 & 1.0000568  \\
3237.8861 & 0.99961972 & 1.0000490  \\
3237.9066 & 0.99955744 & 0.99998623 \\
3237.9270 & 0.99961357 & 1.0000418  \\
3237.9474 & 0.99957114 & 0.99999868 \\
3237.9679 & 0.99953546 & 0.99996233 \\
3237.9883 & 0.99955979 & 0.99998602 \\
3238.0087 & 0.99959141 & 1.0000168  \\
3238.0496 & 0.99959018 & 1.0000137  \\
3238.0700 & 0.99959345 & 1.0000160  \\
3238.1109 & 0.99954439 & 0.99996495 \\
3238.1313 & 0.99959420 & 1.0000135  \\
3238.1517 & 0.99960499 & 1.0000233  \\
3238.1722 & 0.99954358 & 0.99996079 \\
3238.1926 & 0.99956733 & 0.99998349 \\
3238.2130 & 0.99960982 & 1.0000250  \\
3238.2335 & 0.99963443 & 1.0000485  \\
3238.2539 & 0.99963501 & 1.0000482  \\
3238.2948 & 0.99956688 & 0.99997803 \\
3238.3152 & 0.99957290 & 0.99998315 \\
3238.3356 & 0.99959286 & 1.0000022  \\
3238.3561 & 0.99958937 & 0.99999808 \\
3238.3765 & 0.99955316 & 0.99996108 \\
3238.3969 & 0.99958683 & 0.99999423 \\
3238.4174 & 0.99958837 & 0.99999523 \\
3238.4378 & 0.99957535 & 0.99998179 \\
3238.4582 & 0.99954408 & 0.99994996 \\
3238.4786 & 0.99959914 & 1.0000048  \\
3238.4991 & 0.99959616 & 1.0000018  \\
3238.5399 & 0.99954613 & 0.99995142 \\
3238.5604 & 0.99955533 & 0.99996068 \\
3238.5808 & 0.99957112 & 0.99997666 \\
3238.6012 & 0.99954415 & 0.99994980 \\
3238.6217 & 0.99959780 & 1.0000038  \\
3238.6421 & 0.99965718 & 1.0000632  \\
3238.6625 & 0.99958431 & 0.99999105 \\
3238.6830 & 0.99964913 & 1.0000562  \\
3238.7034 & 0.99962686 & 1.0000345  \\
3238.7238 & 0.99960922 & 1.0000172  \\
3238.7443 & 0.99958987 & 0.99999846 \\
3238.8056 & 0.99952807 & 0.99993860 \\
3238.8260 & 0.99956824 & 0.99997950 \\
3238.8464 & 0.99962467 & 1.0000368  \\
3238.8669 & 0.99959231 & 1.0000050  \\
3238.9077 & 0.99960218 & 1.0000167  \\
3238.9281 & 0.99958885 & 1.0000041  \\
3238.9486 & 0.99958925 & 1.0000055  \\
3238.9690 & 0.99957398 & 0.99999115 \\
3238.9894 & 0.99962199 & 1.0000400  \\
3239.0303 & 0.99960897 & 1.0000289  \\
3239.0507 & 0.99961246 & 1.0000333  \\
3239.0712 & 0.99960817 & 1.0000302  \\
3239.0916 & 0.99954693 & 0.99996970 \\
3239.1120 & 0.99956538 & 0.99998922 \\
3239.1325 & 0.99952733 & 0.99995205 \\
3239.1529 & 0.99954326 & 0.99996889 \\
3239.1733 & 0.99958780 & 1.0000145  \\
3239.1938 & 0.99953573 & 0.99996326 \\
3239.2142 & 0.99954723 & 0.99997560 \\
3239.2346 & 0.99956230 & 0.99999163 \\
3239.2755 & 0.99957360 & 1.0000047  \\
3239.2959 & 0.99957001 & 1.0000019  \\
3239.3164 & 0.99958683 & 1.0000196  \\
3239.3368 & 0.99960959 & 1.0000431  \\
3239.3572 & 0.99958813 & 1.0000224  \\
3239.3776 & 0.99954953 & 0.99998458 \\
3239.3981 & 0.99957240 & 1.0000081  \\
3239.4185 & 0.99958693 & 1.0000234  \\
3239.4389 & 0.99958178 & 1.0000189  \\
3239.4594 & 0.99955633 & 0.99999400 \\
3239.4798 & 0.99954248 & 0.99998062 \\
3239.5207 & 0.99952129 & 0.99996050 \\
3239.5411 & 0.99958508 & 1.0000247  \\
3239.5615 & 0.99953850 & 0.99997849 \\
3239.5820 & 0.99952929 & 0.99996969 \\
3239.6024 & 0.99956960 & 1.0000103  \\
3239.6228 & 0.99957873 & 1.0000197  \\
3239.6433 & 0.99954727 & 0.99998840 \\
3239.6637 & 0.99954885 & 0.99999004 \\
3239.6841 & 0.99954063 & 0.99998211 \\
3239.7046 & 0.99954233 & 0.99998363 \\
3239.7250 & 0.99957417 & 1.0000155  \\
3239.7659 & 0.99958850 & 1.0000295  \\
3239.7863 & 0.99956995 & 1.0000108  \\
3239.8067 & 0.99955441 & 0.99999489 \\
3239.8271 & 0.99955086 & 0.99999092 \\
3239.8476 & 0.99951242 & 0.99995204 \\
3239.8680 & 0.99956915 & 1.0000083  \\
3239.8884 & 0.99955809 & 0.99999660 \\
3239.9089 & 0.99956218 & 0.99999986 \\
3239.9293 & 0.99953256 & 0.99996963 \\
3239.9497 & 0.99958431 & 1.0000204  \\
3239.9702 & 0.99961226 & 1.0000476  \\
3240.0110 & 0.99957359 & 1.0000069  \\
3240.0315 & 0.99958191 & 1.0000141  \\
3240.0519 & 0.99957707 & 1.0000081  \\
3240.0723 & 0.99957691 & 1.0000067  \\
3240.0928 & 0.99960418 & 1.0000328  \\
3240.1132 & 0.99956603 & 0.99999339 \\
3240.1336 & 0.99960160 & 1.0000275  \\
3240.1541 & 0.99956321 & 0.99998788 \\
3240.1745 & 0.99956816 & 0.99999141 \\
3240.1949 & 0.99961331 & 1.0000351  \\
3240.2154 & 0.99960272 & 1.0000232  \\
3240.2562 & 0.99961873 & 1.0000361  \\
3240.2766 & 0.99959380 & 1.0000097  \\
3240.2971 & 0.99955485 & 0.99996927 \\
3240.3175 & 0.99962780 & 1.0000408  \\
3240.3379 & 0.99953998 & 0.99995148 \\
3240.3584 & 0.99959748 & 1.0000075  \\
3240.3788 & 0.99954885 & 0.99995742 \\
3240.3992 & 0.99956365 & 0.99997080 \\
3240.4197 & 0.99953382 & 0.99993953 \\
3240.4401 & 0.99960056 & 1.0000049  \\
3240.4605 & 0.99957886 & 0.99998190 \\
3240.5014 & 0.99959860 & 0.99999902 \\
3240.5218 & 0.99960282 & 1.0000021  \\
3240.5423 & 0.99959931 & 0.99999735 \\
3240.5627 & 0.99963264 & 1.0000294  \\
3240.5831 & 0.99957866 & 0.99997443 \\
3240.6036 & 0.99961916 & 1.0000138  \\
3240.6240 & 0.99953951 & 0.99993329 \\
3240.6444 & 0.99955346 & 0.99994630 \\
3240.6649 & 0.99959110 & 0.99998300 \\
3240.6853 & 0.99953404 & 0.99992519 \\
3240.7057 & 0.99959869 & 0.99998921 \\
3240.7466 & 0.99962713 & 1.0000166  \\
3240.7670 & 0.99963623 & 1.0000251  \\
3240.7874 & 0.99964562 & 1.0000341  \\
3240.8079 & 0.99961018 & 0.99999845 \\
3240.8283 & 0.99962667 & 1.0000145  \\
3240.8487 & 0.99963189 & 1.0000193  \\
3240.8692 & 0.99959074 & 0.99997799 \\
3240.8896 & 0.99962358 & 1.0000106  \\
3240.9100 & 0.99963576 & 1.0000227  \\
3240.9305 & 0.99961817 & 1.0000049  \\
3240.9509 & 0.99964566 & 1.0000324  \\
3240.9918 & 0.99971975 & 1.0001064  \\
3241.0122 & 0.99962085 & 1.0000073  \\
3241.0326 & 0.99959084 & 0.99997731 \\
3241.0531 & 0.99962295 & 1.0000094  \\
3241.0735 & 0.99960070 & 0.99998711 \\
3241.0939 & 0.99961853 & 1.0000049  \\
3241.1144 & 0.99959366 & 0.99997989 \\
3241.1348 & 0.99965127 & 1.0000377  \\
3241.1552 & 0.99960754 & 0.99999396 \\
3241.1757 & 0.99960453 & 0.99999088 \\
3241.1961 & 0.99966325 & 1.0000494  \\
3241.2369 & 0.99966540 & 1.0000516  \\
3241.2574 & 0.99962162 & 1.0000075  \\
3241.2778 & 0.99965288 & 1.0000387  \\
3241.2982 & 0.99960519 & 0.99999089 \\
3241.3187 & 0.99961421 & 0.99999962 \\
3241.3391 & 0.99962382 & 1.0000089  \\
3241.3595 & 0.99960908 & 0.99999389 \\
3241.3800 & 0.99960417 & 0.99998855 \\
3241.4004 & 0.99960811 & 0.99999214 \\
3241.4208 & 0.99958102 & 0.99996468 \\
3241.4413 & 0.99955270 & 0.99993575 \\
3241.4617 & 0.99961070 & 0.99999313 \\
3241.4821 & 0.99964891 & 1.0000308  \\
3241.5026 & 0.99964488 & 1.0000260  \\
3241.5230 & 0.99961920 & 0.99999965 \\
3241.5434 & 0.99959107 & 0.99997086 \\
3241.5639 & 0.99962615 & 1.0000050  \\
3241.5843 & 0.99964200 & 1.0000201  \\
3241.6047 & 0.99959057 & 0.99996785 \\
3241.6252 & 0.99961470 & 0.99999110 \\
3241.6456 & 0.99961680 & 0.99999206 \\
3241.6660 & 0.99964910 & 1.0000236  \\
3241.7273 & 0.99961321 & 0.99998478 \\
3241.7477 & 0.99960053 & 0.99997096 \\
3241.7682 & 0.99958972 & 0.99995914 \\
3241.7886 & 0.99957883 & 0.99994729 \\
3241.8090 & 0.99964332 & 1.0000108  \\
3241.8295 & 0.99964716 & 1.0000136  \\
3241.8499 & 0.99964852 & 1.0000140  \\
3241.8703 & 0.99965049 & 1.0000149  \\
3241.8908 & 0.99961579 & 0.99997926 \\
3241.9112 & 0.99965413 & 1.0000165  \\
3241.9316 & 0.99965277 & 1.0000143  \\
3241.9725 & 0.99962399 & 0.99998363 \\
3241.9929 & 0.99965448 & 1.0000131  \\
3242.0134 & 0.99959667 & 0.99995458 \\
3242.0338 & 0.99959754 & 0.99995462 \\
3242.0542 & 0.99963411 & 0.99999030 \\
3242.0951 & 0.99965636 & 1.0000111  \\
3242.1155 & 0.99962573 & 0.99997995 \\
3242.1359 & 0.99960563 & 0.99995919 \\
3242.1564 & 0.99962708 & 0.99998005 \\
3242.1768 & 0.99964827 & 1.0000008  \\
3242.2177 & 0.99963273 & 0.99998439 \\
3242.2381 & 0.99961141 & 0.99996276 \\
3242.2585 & 0.99967752 & 1.0000285  \\
3242.2790 & 0.99962331 & 0.99997419 \\
3242.2994 & 0.99974429 & 1.0000949  \\
3242.3198 & 0.99967206 & 1.0000227  \\
3242.3607 & 0.99972201 & 1.0000725  \\
3242.3811 & 0.99962924 & 0.99997965 \\
3242.4016 & 0.99971118 & 1.0000616  \\
3242.4220 & 0.99965287 & 1.0000035  \\
3242.4629 & 0.99964837 & 0.99999914 \\
3242.4833 & 0.99968994 & 1.0000408  \\
3242.5037 & 0.99964992 & 1.0000011  \\
3242.5242 & 0.99964018 & 0.99999167 \\
3242.5446 & 0.99967239 & 1.0000241  \\
3242.5650 & 0.99963604 & 0.99998806 \\
3242.5855 & 0.99967306 & 1.0000255  \\
3242.6059 & 0.99968322 & 1.0000360  \\
3242.6263 & 0.99968131 & 1.0000344  \\
3242.6467 & 0.99966956 & 1.0000229  \\
3242.6672 & 0.99966661 & 1.0000204  \\
3242.7080 & 0.99962566 & 0.99998060 \\
3242.7285 & 0.99961517 & 0.99997046 \\
3242.7489 & 0.99961848 & 0.99997425 \\
3242.7693 & 0.99963401 & 0.99999032 \\
3242.7898 & 0.99964483 & 1.0000016  \\
3242.8102 & 0.99963006 & 0.99998738 \\
3242.8306 & 0.99966935 & 1.0000273  \\
3242.8715 & 0.99961583 & 0.99997476 \\
3242.8919 & 0.99965086 & 1.0000103  \\
3242.9124 & 0.99957041 & 0.99993045 \\
3242.9532 & 0.99963068 & 0.99999188 \\
3242.9737 & 0.99964158 & 1.0000033  \\
3242.9941 & 0.99964801 & 1.0000101  \\
3243.0145 & 0.99964730 & 1.0000101  \\
3243.0350 & 0.99959819 & 0.99996147 \\
3243.0554 & 0.99962738 & 0.99999114 \\
3243.0758 & 0.99960932 & 0.99997355 \\
3243.0962 & 0.99960119 & 0.99996578 \\
3243.1167 & 0.99962117 & 0.99998618 \\
3243.1371 & 0.99961727 & 0.99998258 \\
3243.1575 & 0.99963029 & 0.99999591 \\
3243.1780 & 0.99962038 & 0.99998623 \\
3243.1984 & 0.99965825 & 1.0000242  \\
3243.2188 & 0.99960199 & 0.99996807 \\
3243.2393 & 0.99966229 & 1.0000285  \\
3243.2597 & 0.99963998 & 1.0000061  \\
3243.2801 & 0.99963452 & 1.0000007  \\
3243.3006 & 0.99963037 & 0.99999611 \\
3243.3210 & 0.99965443 & 1.0000201  \\
3243.3414 & 0.99966443 & 1.0000296  \\
3243.3619 & 0.99966776 & 1.0000326  \\
3243.3823 & 0.99961883 & 0.99998307 \\
3243.4027 & 0.99967215 & 1.0000359  \\
3243.4436 & 0.99962124 & 0.99998340 \\
3243.4640 & 0.99964100 & 1.0000022  \\
3243.4845 & 0.99967414 & 1.0000343  \\
3243.5049 & 0.99960723 & 0.99996621 \\
3243.5253 & 0.99962843 & 0.99998599 \\
3243.5457 & 0.99964292 & 0.99999924 \\
3243.5662 & 0.99967742 & 1.0000321  \\
3243.5866 & 0.99962416 & 0.99997707 \\
3243.6070 & 0.99961851 & 0.99996963 \\
3243.6275 & 0.99963819 & 0.99998735 \\
3243.6479 & 0.99966264 & 1.0000097  \\
3243.6888 & 0.99964627 & 0.99998846 \\
3243.7092 & 0.99967329 & 1.0000130  \\
3243.7296 & 0.99967805 & 1.0000148  \\
3243.7501 & 0.99969117 & 1.0000251  \\
3243.7705 & 0.99967200 & 1.0000030  \\
3243.7909 & 0.99968596 & 1.0000140  \\
3243.8114 & 0.99964595 & 0.99997085 \\
3243.8318 & 0.99970910 & 1.0000309  \\
3243.8522 & 0.99966351 & 0.99998203 \\
3243.8727 & 0.99972397 & 1.0000394  \\
3243.8931 & 0.99968746 & 0.99999991 \\
3243.9340 & 0.99968949 & 0.99999544 \\
3243.9544 & 0.99968622 & 0.99998925 \\
3243.9748 & 0.99967666 & 0.99997670 \\
3243.9953 & 0.99970378 & 1.0000010  \\
3244.0157 & 0.99974316 & 1.0000376  \\
3244.0361 & 0.99963278 & 0.99992458 \\
3244.0565 & 0.99973428 & 1.0000236  \\
3244.0770 & 0.99973997 & 1.0000269  \\
3244.0974 & 0.99968632 & 0.99997105 \\
3244.1178 & 0.99972419 & 1.0000070  \\
3244.1383 & 0.99971796 & 0.99999906 \\
3244.1791 & 0.99969343 & 0.99997172 \\
3244.1996 & 0.99972116 & 0.99999844 \\
3244.2200 & 0.99973759 & 1.0000140  \\
3244.2404 & 0.99971139 & 0.99998747 \\
3244.2609 & 0.99971965 & 0.99999562 \\
3244.2813 & 0.99980711 & 1.0000833  \\
3244.3017 & 0.99968063 & 0.99995737 \\
3244.3222 & 0.99972678 & 1.0000044  \\
3244.3426 & 0.99972075 & 0.99999964 \\
3244.3630 & 0.99970085 & 0.99998146 \\
3244.3835 & 0.99971981 & 1.0000025  \\
3244.4243 & 0.99971669 & 1.0000050  \\
\enddata
\end{deluxetable}
%\tablecomments{}
